Boosting Data Reduction for the Maximum Weight Independent Set Problem Using Increasing Transformations

Given a vertex-weighted graph, the maximum weight independent set problem asks for a pair-wise non-adjacent set of vertices such that the sum of their weights is maximum. The branch-and-reduce paradigm is the de facto standard approach to solve the problem to optimality in practice. In this paradigm, data reduction rules are applied to decrease the problem size. These data reduction rules ensure that given an optimum solution on the new (smaller) input, one can quickly construct an optimum solution on the original input. We introduce new generalized data reduction and transformation rules for the problem. A key feature of our work is that some transformation rules can increase the size of the input. Surprisingly, these so-called increasing transformations can simplify the problem and also open up the reduction space to yield even smaller irreducible graphs later throughout the algorithm. In experiments, our algorithm computes significantly smaller irreducible graphs on all except one instance, solves more instances to optimality than previously possible, is up to two orders of magnitude faster than the best state-of-the-art solver, and finds higher-quality solutions than heuristic solvers DynWVC and HILS on many instances. While the increasing transformations are only efficient enough for preprocessing at this time, we see this as a critical initial step towards a new branch-and-transform paradigm.

==> plots/cactus_plots/fe.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:32:36
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,162.61);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round,fill=fillColor] (  0.00, -0.00) rectangle (216.81,162.61);
\end{scope}
\begin{scope}
\path[clip] ( 24.75, 60.95) rectangle (211.81,157.61);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 24.75, 60.95) rectangle (211.81,157.61);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 24.75, 65.34) --
	(211.81, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 24.75, 94.63) --
	(211.81, 94.63);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 24.75,123.92) --
	(211.81,123.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 24.75,153.21) --
	(211.81,153.21);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 30.32, 60.95) --
	( 30.32,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.57, 60.95) --
	( 73.57,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (116.81, 60.95) --
	(116.81,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (160.06, 60.95) --
	(160.06,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.31, 60.95) --
	(203.31,157.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 33.25, 65.34) --
	( 35.23, 65.34) --
	( 35.23, 94.63) --
	( 53.27, 94.63) --
	( 53.27,123.92) --
	( 70.15,123.92) --
	( 70.15,153.21) --
	(203.31,153.21) --
	(203.31,153.21);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 33.25, 65.34) --
	( 40.11, 65.34) --
	( 40.11, 94.63) --
	( 51.91, 94.63) --
	( 51.91,123.92) --
	( 68.60,123.92) --
	( 68.60,153.21) --
	(203.31,153.21) --
	(203.31,153.21);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 33.25, 65.34) --
	( 59.09, 65.34) --
	( 59.09, 94.63) --
	(203.31, 94.63) --
	(203.31, 94.63);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 33.25, 65.34) --
	(203.31, 65.34) --
	(203.31, 65.34);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 33.25, 65.34) --
	(107.19, 65.34) --
	(107.19, 94.63) --
	(203.31, 94.63) --
	(203.31, 94.63);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (  0.09, 60.95) -- (  0.09, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (  7.71, 60.95) -- (  7.71, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 13.11, 60.95) -- ( 13.11, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 17.30, 60.95) -- ( 17.30, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 20.72, 60.95) -- ( 20.72, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 23.62, 60.95) -- ( 23.62, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 26.13, 60.95) -- ( 26.13, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 28.34, 60.95) -- ( 28.34, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 30.32, 60.95) -- ( 30.32, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 43.34, 60.95) -- ( 43.34, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 50.95, 60.95) -- ( 50.95, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 56.36, 60.95) -- ( 56.36, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 60.55, 60.95) -- ( 60.55, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 63.97, 60.95) -- ( 63.97, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 66.87, 60.95) -- ( 66.87, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 69.37, 60.95) -- ( 69.37, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 71.59, 60.95) -- ( 71.59, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 73.57, 60.95) -- ( 73.57, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 86.58, 60.95) -- ( 86.58, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 94.20, 60.95) -- ( 94.20, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 99.60, 60.95) -- ( 99.60, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (103.79, 60.95) -- (103.79, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (107.22, 60.95) -- (107.22, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (110.11, 60.95) -- (110.11, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (112.62, 60.95) -- (112.62, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (114.83, 60.95) -- (114.83, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (116.81, 60.95) -- (116.81, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (129.83, 60.95) -- (129.83, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (137.45, 60.95) -- (137.45, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (142.85, 60.95) -- (142.85, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (147.04, 60.95) -- (147.04, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (150.47, 60.95) -- (150.47, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (153.36, 60.95) -- (153.36, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (155.87, 60.95) -- (155.87, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (158.08, 60.95) -- (158.08, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (160.06, 60.95) -- (160.06, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (173.08, 60.95) -- (173.08, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (180.69, 60.95) -- (180.69, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (186.10, 60.95) -- (186.10, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (190.29, 60.95) -- (190.29, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (193.71, 60.95) -- (193.71, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (196.61, 60.95) -- (196.61, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (199.12, 60.95) -- (199.12, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (201.33, 60.95) -- (201.33, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (203.31, 60.95) -- (203.31, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (216.33, 60.95) -- (216.33, 62.37);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 24.75, 60.95) rectangle (211.81,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 24.75, 60.95) --
	( 24.75,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 20.25, 62.59) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 20.25, 91.88) {1};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 20.25,121.17) {2};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 20.25,150.46) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 22.25, 65.34) --
	( 24.75, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 22.25, 94.63) --
	( 24.75, 94.63);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 22.25,123.92) --
	( 24.75,123.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 22.25,153.21) --
	( 24.75,153.21);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 24.75, 60.95) --
	(211.81, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 30.32, 58.45) --
	( 30.32, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.57, 58.45) --
	( 73.57, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (116.81, 58.45) --
	(116.81, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (160.06, 58.45) --
	(160.06, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.31, 58.45) --
	(203.31, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.12, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 31.95, 52.84) {-1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 68.28, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 76.11, 52.84) {0};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (111.53, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (119.36, 52.84) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (154.77, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (162.61, 52.84) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (198.02, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (205.85, 52.84) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (118.28, 38.62) {Time [s]};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 11.89,109.28) {Solved instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 50.45, 23.07) -- ( 64.33, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 50.45, 15.84) -- ( 64.33, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 50.45,  8.61) -- ( 64.33,  8.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (129.18, 23.07) -- (143.05, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (129.18, 15.84) -- (143.05, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 71.06, 20.31) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 71.06, 13.09) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 71.06,  5.86) {Non-Increasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (149.79, 20.31) {Basic-Dense};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (149.79, 13.09) {Basic-Sparse};
\end{scope}
\end{tikzpicture}


==> plots/cactus_plots/mesh.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:32:48
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,162.61);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round,fill=fillColor] (  0.00, -0.00) rectangle (216.81,162.61);
\end{scope}
\begin{scope}
\path[clip] ( 28.66, 60.95) rectangle (211.81,157.61);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 28.66, 60.95) rectangle (211.81,157.61);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66, 65.34) --
	(211.81, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66, 94.63) --
	(211.81, 94.63);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66,123.92) --
	(211.81,123.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66,153.21) --
	(211.81,153.21);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.44, 60.95) --
	( 44.44,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 76.25, 60.95) --
	( 76.25,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (108.06, 60.95) --
	(108.06,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (139.87, 60.95) --
	(139.87,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (171.68, 60.95) --
	(171.68,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.49, 60.95) --
	(203.49,157.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 39.58, 65.34) --
	( 39.58, 71.20) --
	( 39.76, 71.20) --
	( 39.76, 77.06) --
	( 40.60, 77.06) --
	( 40.60, 82.92) --
	( 53.41, 82.92) --
	( 53.41, 88.78) --
	( 61.01, 88.78) --
	( 61.01, 94.63) --
	( 61.26, 94.63) --
	( 61.26,100.49) --
	( 62.96,100.49) --
	( 62.96,106.35) --
	( 70.54,106.35) --
	( 70.54,112.21) --
	( 74.70,112.21) --
	( 74.70,118.07) --
	( 82.44,118.07) --
	( 82.44,123.92) --
	( 87.86,123.92) --
	( 87.86,129.78) --
	( 98.15,129.78) --
	( 98.15,135.64) --
	(112.34,135.64) --
	(112.34,141.50) --
	(119.31,141.50) --
	(119.31,147.36) --
	(120.78,147.36) --
	(120.78,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 39.89, 65.34) --
	( 39.89, 71.20) --
	( 40.82, 71.20) --
	( 40.82, 77.06) --
	( 40.96, 77.06) --
	( 40.96, 82.92) --
	( 53.54, 82.92) --
	( 53.54, 88.78) --
	( 60.71, 88.78) --
	( 60.71, 94.63) --
	( 61.70, 94.63) --
	( 61.70,100.49) --
	( 64.08,100.49) --
	( 64.08,106.35) --
	( 70.44,106.35) --
	( 70.44,112.21) --
	( 74.88,112.21) --
	( 74.88,118.07) --
	( 84.24,118.07) --
	( 84.24,123.92) --
	( 88.93,123.92) --
	( 88.93,129.78) --
	( 99.98,129.78) --
	( 99.98,135.64) --
	(111.46,135.64) --
	(111.46,141.50) --
	(120.08,141.50) --
	(120.08,147.36) --
	(121.04,147.36) --
	(121.04,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 38.44, 65.34) --
	( 38.44, 71.20) --
	( 41.08, 71.20) --
	( 41.08, 77.06) --
	( 45.30, 77.06) --
	( 45.30, 82.92) --
	( 58.29, 82.92) --
	( 58.29, 88.78) --
	( 59.31, 88.78) --
	( 59.31, 94.63) --
	( 61.32, 94.63) --
	( 61.32,100.49) --
	( 61.95,100.49) --
	( 61.95,106.35) --
	( 71.43,106.35) --
	( 71.43,112.21) --
	( 74.95,112.21) --
	( 74.95,118.07) --
	( 80.85,118.07) --
	( 80.85,123.92) --
	( 86.23,123.92) --
	( 86.23,129.78) --
	(102.09,129.78) --
	(102.09,135.64) --
	(118.19,135.64) --
	(118.19,141.50) --
	(121.97,141.50) --
	(121.97,147.36) --
	(123.94,147.36) --
	(123.94,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	(136.55, 65.34) --
	(136.55, 71.20) --
	(203.49, 71.20) --
	(203.49, 71.20);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 56.60, 65.34) --
	( 56.60, 71.20) --
	( 70.14, 71.20) --
	( 70.14, 77.06) --
	( 71.17, 77.06) --
	( 71.17, 82.92) --
	( 73.34, 82.92) --
	( 73.34, 88.78) --
	( 78.32, 88.78) --
	( 78.32, 94.63) --
	( 85.50, 94.63) --
	( 85.50,100.49) --
	( 86.49,100.49) --
	( 86.49,106.35) --
	( 94.02,106.35) --
	( 94.02,112.21) --
	( 97.74,112.21) --
	( 97.74,118.07) --
	(106.41,118.07) --
	(106.41,123.92) --
	(126.61,123.92) --
	(126.61,129.78) --
	(130.23,129.78) --
	(130.23,135.64) --
	(132.00,135.64) --
	(132.00,141.50) --
	(143.41,141.50) --
	(143.41,147.36) --
	(166.32,147.36) --
	(166.32,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 12.63, 60.95) -- ( 12.63, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 22.21, 60.95) -- ( 22.21, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 27.81, 60.95) -- ( 27.81, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 31.78, 60.95) -- ( 31.78, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 34.86, 60.95) -- ( 34.86, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 37.38, 60.95) -- ( 37.38, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 39.51, 60.95) -- ( 39.51, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 41.36, 60.95) -- ( 41.36, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 42.98, 60.95) -- ( 42.98, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 44.44, 60.95) -- ( 44.44, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 54.02, 60.95) -- ( 54.02, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 59.62, 60.95) -- ( 59.62, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 63.59, 60.95) -- ( 63.59, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 66.67, 60.95) -- ( 66.67, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 69.19, 60.95) -- ( 69.19, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 71.32, 60.95) -- ( 71.32, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 73.17, 60.95) -- ( 73.17, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 74.79, 60.95) -- ( 74.79, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 76.25, 60.95) -- ( 76.25, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 85.82, 60.95) -- ( 85.82, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 91.43, 60.95) -- ( 91.43, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 95.40, 60.95) -- ( 95.40, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 98.48, 60.95) -- ( 98.48, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (101.00, 60.95) -- (101.00, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (103.13, 60.95) -- (103.13, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (104.98, 60.95) -- (104.98, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (106.60, 60.95) -- (106.60, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (108.06, 60.95) -- (108.06, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (117.63, 60.95) -- (117.63, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (123.23, 60.95) -- (123.23, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (127.21, 60.95) -- (127.21, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (130.29, 60.95) -- (130.29, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (132.81, 60.95) -- (132.81, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (134.94, 60.95) -- (134.94, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (136.78, 60.95) -- (136.78, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (138.41, 60.95) -- (138.41, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (139.87, 60.95) -- (139.87, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (149.44, 60.95) -- (149.44, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (155.04, 60.95) -- (155.04, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (159.02, 60.95) -- (159.02, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (162.10, 60.95) -- (162.10, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (164.62, 60.95) -- (164.62, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (166.75, 60.95) -- (166.75, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (168.59, 60.95) -- (168.59, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (170.22, 60.95) -- (170.22, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (171.68, 60.95) -- (171.68, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (181.25, 60.95) -- (181.25, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (186.85, 60.95) -- (186.85, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (190.83, 60.95) -- (190.83, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (193.91, 60.95) -- (193.91, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (196.43, 60.95) -- (196.43, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (198.56, 60.95) -- (198.56, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (200.40, 60.95) -- (200.40, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (202.03, 60.95) -- (202.03, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (203.49, 60.95) -- (203.49, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (213.06, 60.95) -- (213.06, 62.37);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 28.66, 60.95) rectangle (211.81,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 28.66, 60.95) --
	( 28.66,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16, 62.59) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16, 91.88) {5};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16,121.17) {10};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16,150.46) {15};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16, 65.34) --
	( 28.66, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16, 94.63) --
	( 28.66, 94.63);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16,123.92) --
	( 28.66,123.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16,153.21) --
	( 28.66,153.21);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 28.66, 60.95) --
	(211.81, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.44, 58.45) --
	( 44.44, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 76.25, 58.45) --
	( 76.25, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (108.06, 58.45) --
	(108.06, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (139.87, 58.45) --
	(139.87, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (171.68, 58.45) --
	(171.68, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.49, 58.45) --
	(203.49, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 38.24, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 46.07, 52.84) {-2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 70.05, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 77.88, 52.84) {-1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (102.77, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (110.60, 52.84) {0};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (134.58, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (142.41, 52.84) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (166.39, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (174.22, 52.84) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (198.20, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (206.03, 52.84) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (120.24, 38.62) {Time [s]};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 11.89,109.28) {Solved instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41, 23.07) -- ( 66.29, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41, 15.84) -- ( 66.29, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41,  8.61) -- ( 66.29,  8.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.13, 23.07) -- (145.01, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.13, 15.84) -- (145.01, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02, 20.31) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02, 13.09) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02,  5.86) {Non-Increasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.75, 20.31) {Basic-Dense};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.75, 13.09) {Basic-Sparse};
\end{scope}
\end{tikzpicture}


==> plots/cactus_plots/osm.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:33:01
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,162.61);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round,fill=fillColor] (  0.00, -0.00) rectangle (216.81,162.61);
\end{scope}
\begin{scope}
\path[clip] ( 28.66, 60.95) rectangle (211.81,157.61);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 28.66, 60.95) rectangle (211.81,157.61);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66, 65.34) --
	(211.81, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66, 85.31) --
	(211.81, 85.31);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66,105.28) --
	(211.81,105.28);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66,125.25) --
	(211.81,125.25);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66,145.23) --
	(211.81,145.23);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 52.72, 60.95) --
	( 52.72,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 82.87, 60.95) --
	( 82.87,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (113.02, 60.95) --
	(113.02,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (143.18, 60.95) --
	(143.18,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (173.33, 60.95) --
	(173.33,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.49, 60.95) --
	(203.49,157.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 38.58, 65.34) --
	( 38.58, 69.34) --
	( 54.91, 69.34) --
	( 54.91, 73.33) --
	( 60.37, 73.33) --
	( 60.37, 77.33) --
	( 65.70, 77.33) --
	( 65.70, 81.32) --
	( 75.82, 81.32) --
	( 75.82, 85.31) --
	( 76.97, 85.31) --
	( 76.97, 89.31) --
	( 77.59, 89.31) --
	( 77.59, 93.30) --
	( 78.74, 93.30) --
	( 78.74, 97.30) --
	( 78.95, 97.30) --
	( 78.95,101.29) --
	( 81.44,101.29) --
	( 81.44,105.28) --
	( 81.98,105.28) --
	( 81.98,109.28) --
	( 84.43,109.28) --
	( 84.43,113.27) --
	( 93.83,113.27) --
	( 93.83,117.27) --
	(104.72,117.27) --
	(104.72,121.26) --
	(110.07,121.26) --
	(110.07,125.25) --
	(118.33,125.25) --
	(118.33,129.25) --
	(127.10,129.25) --
	(127.10,133.24) --
	(130.99,133.24) --
	(130.99,137.24) --
	(143.63,137.24) --
	(143.63,141.23) --
	(179.11,141.23) --
	(179.11,145.23) --
	(192.46,145.23) --
	(192.46,149.22) --
	(203.49,149.22) --
	(203.49,149.22);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 38.37, 65.34) --
	( 38.37, 69.34) --
	( 54.67, 69.34) --
	( 54.67, 73.33) --
	( 55.02, 73.33) --
	( 55.02, 77.33) --
	( 68.08, 77.33) --
	( 68.08, 81.32) --
	( 77.38, 81.32) --
	( 77.38, 85.31) --
	( 78.92, 85.31) --
	( 78.92, 89.31) --
	( 81.00, 89.31) --
	( 81.00, 93.30) --
	( 83.29, 93.30) --
	( 83.29, 97.30) --
	( 85.47, 97.30) --
	( 85.47,101.29) --
	( 88.03,101.29) --
	( 88.03,105.28) --
	( 88.94,105.28) --
	( 88.94,109.28) --
	(101.25,109.28) --
	(101.25,113.27) --
	(101.60,113.27) --
	(101.60,117.27) --
	(130.02,117.27) --
	(130.02,121.26) --
	(132.95,121.26) --
	(132.95,125.25) --
	(153.08,125.25) --
	(153.08,129.25) --
	(158.63,129.25) --
	(158.63,133.24) --
	(158.87,133.24) --
	(158.87,137.24) --
	(162.89,137.24) --
	(162.89,141.23) --
	(184.89,141.23) --
	(184.89,145.23) --
	(190.78,145.23) --
	(190.78,149.22) --
	(194.12,149.22) --
	(194.12,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 42.79, 65.34) --
	( 42.79, 69.34) --
	( 53.98, 69.34) --
	( 53.98, 73.33) --
	( 54.71, 73.33) --
	( 54.71, 77.33) --
	( 65.11, 77.33) --
	( 65.11, 81.32) --
	( 78.01, 81.32) --
	( 78.01, 85.31) --
	( 90.08, 85.31) --
	( 90.08, 89.31) --
	( 90.76, 89.31) --
	( 90.76, 93.30) --
	( 91.11, 93.30) --
	( 91.11, 97.30) --
	( 99.96, 97.30) --
	( 99.96,101.29) --
	(100.67,101.29) --
	(100.67,105.28) --
	(100.81,105.28) --
	(100.81,109.28) --
	(110.50,109.28) --
	(110.50,113.27) --
	(111.25,113.27) --
	(111.25,117.27) --
	(118.05,117.27) --
	(118.05,121.26) --
	(130.67,121.26) --
	(130.67,125.25) --
	(155.68,125.25) --
	(155.68,129.25) --
	(161.27,129.25) --
	(161.27,133.24) --
	(179.74,133.24) --
	(179.74,137.24) --
	(184.71,137.24) --
	(184.71,141.23) --
	(203.49,141.23) --
	(203.49,141.23);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 53.43, 65.34) --
	( 53.43, 69.34) --
	( 72.58, 69.34) --
	( 72.58, 73.33) --
	( 97.88, 73.33) --
	( 97.88, 77.33) --
	( 99.82, 77.33) --
	( 99.82, 81.32) --
	(106.46, 81.32) --
	(106.46, 85.31) --
	(132.03, 85.31) --
	(132.03, 89.31) --
	(134.88, 89.31) --
	(134.88, 93.30) --
	(136.90, 93.30) --
	(136.90, 97.30) --
	(137.63, 97.30) --
	(137.63,101.29) --
	(141.03,101.29) --
	(141.03,105.28) --
	(145.40,105.28) --
	(145.40,109.28) --
	(152.71,109.28) --
	(152.71,113.27) --
	(163.11,113.27) --
	(163.11,117.27) --
	(164.75,117.27) --
	(164.75,121.26) --
	(170.45,121.26) --
	(170.45,125.25) --
	(201.99,125.25) --
	(201.99,129.25) --
	(203.49,129.25) --
	(203.49,129.25);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 57.22, 65.34) --
	( 57.22, 69.34) --
	( 73.82, 69.34) --
	( 73.82, 73.33) --
	(105.29, 73.33) --
	(105.29, 77.33) --
	(105.86, 77.33) --
	(105.86, 81.32) --
	(112.91, 81.32) --
	(112.91, 85.31) --
	(141.17, 85.31) --
	(141.17, 89.31) --
	(143.46, 89.31) --
	(143.46, 93.30) --
	(144.10, 93.30) --
	(144.10, 97.30) --
	(149.24, 97.30) --
	(149.24,101.29) --
	(155.29,101.29) --
	(155.29,105.28) --
	(168.14,105.28) --
	(168.14,109.28) --
	(175.03,109.28) --
	(175.03,113.27) --
	(186.64,113.27) --
	(186.64,117.27) --
	(203.38,117.27) --
	(203.38,121.26) --
	(203.49,121.26) --
	(203.49,121.26);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 22.56, 60.95) -- ( 22.56, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 31.64, 60.95) -- ( 31.64, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 36.95, 60.95) -- ( 36.95, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 40.72, 60.95) -- ( 40.72, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 43.64, 60.95) -- ( 43.64, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 46.03, 60.95) -- ( 46.03, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 48.05, 60.95) -- ( 48.05, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 49.80, 60.95) -- ( 49.80, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 51.34, 60.95) -- ( 51.34, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 52.72, 60.95) -- ( 52.72, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 61.79, 60.95) -- ( 61.79, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 67.10, 60.95) -- ( 67.10, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 70.87, 60.95) -- ( 70.87, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 73.79, 60.95) -- ( 73.79, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 76.18, 60.95) -- ( 76.18, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 78.20, 60.95) -- ( 78.20, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 79.95, 60.95) -- ( 79.95, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 81.49, 60.95) -- ( 81.49, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 82.87, 60.95) -- ( 82.87, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 91.95, 60.95) -- ( 91.95, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 97.26, 60.95) -- ( 97.26, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (101.03, 60.95) -- (101.03, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (103.95, 60.95) -- (103.95, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (106.34, 60.95) -- (106.34, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (108.35, 60.95) -- (108.35, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (110.10, 60.95) -- (110.10, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (111.65, 60.95) -- (111.65, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (113.02, 60.95) -- (113.02, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (122.10, 60.95) -- (122.10, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (127.41, 60.95) -- (127.41, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (131.18, 60.95) -- (131.18, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (134.10, 60.95) -- (134.10, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (136.49, 60.95) -- (136.49, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (138.51, 60.95) -- (138.51, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (140.26, 60.95) -- (140.26, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (141.80, 60.95) -- (141.80, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (143.18, 60.95) -- (143.18, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (152.26, 60.95) -- (152.26, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (157.57, 60.95) -- (157.57, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (161.33, 60.95) -- (161.33, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (164.25, 60.95) -- (164.25, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (166.64, 60.95) -- (166.64, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (168.66, 60.95) -- (168.66, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (170.41, 60.95) -- (170.41, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (171.95, 60.95) -- (171.95, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (173.33, 60.95) -- (173.33, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (182.41, 60.95) -- (182.41, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (187.72, 60.95) -- (187.72, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (191.49, 60.95) -- (191.49, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (194.41, 60.95) -- (194.41, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (196.80, 60.95) -- (196.80, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (198.81, 60.95) -- (198.81, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (200.56, 60.95) -- (200.56, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (202.11, 60.95) -- (202.11, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (203.49, 60.95) -- (203.49, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (212.56, 60.95) -- (212.56, 62.37);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 28.66, 60.95) rectangle (211.81,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 28.66, 60.95) --
	( 28.66,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16, 62.59) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16, 82.56) {5};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16,102.53) {10};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16,122.50) {15};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16,142.47) {20};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16, 65.34) --
	( 28.66, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16, 85.31) --
	( 28.66, 85.31);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16,105.28) --
	( 28.66,105.28);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16,125.25) --
	( 28.66,125.25);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16,145.23) --
	( 28.66,145.23);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 28.66, 60.95) --
	(211.81, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 52.72, 58.45) --
	( 52.72, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 82.87, 58.45) --
	( 82.87, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (113.02, 58.45) --
	(113.02, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (143.18, 58.45) --
	(143.18, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (173.33, 58.45) --
	(173.33, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.49, 58.45) --
	(203.49, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 46.52, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 54.35, 52.84) {-2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 76.67, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 84.50, 52.84) {-1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (107.74, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (115.57, 52.84) {0};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (137.89, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (145.72, 52.84) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (168.05, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (175.88, 52.84) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (198.20, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (206.03, 52.84) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (120.24, 38.62) {Time [s]};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 11.89,109.28) {Solved instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41, 23.07) -- ( 66.29, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41, 15.84) -- ( 66.29, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41,  8.61) -- ( 66.29,  8.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.13, 23.07) -- (145.01, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.13, 15.84) -- (145.01, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02, 20.31) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02, 13.09) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02,  5.86) {Non-Increasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.75, 20.31) {Basic-Dense};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.75, 13.09) {Basic-Sparse};
\end{scope}
\end{tikzpicture}


==> plots/cactus_plots/snap.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:33:14
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,162.61);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round,fill=fillColor] (  0.00, -0.00) rectangle (216.81,162.61);
\end{scope}
\begin{scope}
\path[clip] ( 28.66, 60.95) rectangle (211.81,157.61);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 28.66, 60.95) rectangle (211.81,157.61);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66, 65.34) --
	(211.81, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66, 96.73) --
	(211.81, 96.73);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 28.66,128.11) --
	(211.81,128.11);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 56.51, 60.95) --
	( 56.51,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 85.91, 60.95) --
	( 85.91,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (115.30, 60.95) --
	(115.30,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (144.70, 60.95) --
	(144.70,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (174.09, 60.95) --
	(174.09,157.61);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.49, 60.95) --
	(203.49,157.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 38.93, 65.34) --
	( 38.93, 68.48) --
	( 42.21, 68.48) --
	( 42.21, 71.62) --
	( 44.64, 71.62) --
	( 44.64, 74.76) --
	( 50.28, 74.76) --
	( 50.28, 77.90) --
	( 53.88, 77.90) --
	( 53.88, 81.03) --
	( 55.10, 81.03) --
	( 55.10, 84.17) --
	( 57.48, 84.17) --
	( 57.48, 87.31) --
	( 62.07, 87.31) --
	( 62.07, 90.45) --
	( 62.51, 90.45) --
	( 62.51, 93.59) --
	( 62.68, 93.59) --
	( 62.68, 96.73) --
	( 66.08, 96.73) --
	( 66.08, 99.86) --
	( 67.55, 99.86) --
	( 67.55,103.00) --
	( 70.06,103.00) --
	( 70.06,106.14) --
	( 71.59,106.14) --
	( 71.59,109.28) --
	( 73.52,109.28) --
	( 73.52,112.42) --
	( 79.66,112.42) --
	( 79.66,115.55) --
	( 83.82,115.55) --
	( 83.82,118.69) --
	( 84.47,118.69) --
	( 84.47,121.83) --
	( 86.16,121.83) --
	( 86.16,124.97) --
	( 88.83,124.97) --
	( 88.83,128.11) --
	(119.98,128.11) --
	(119.98,131.25) --
	(121.31,131.25) --
	(121.31,134.38) --
	(121.60,134.38) --
	(121.60,137.52) --
	(122.84,137.52) --
	(122.84,140.66) --
	(124.09,140.66) --
	(124.09,143.80) --
	(126.84,143.80) --
	(126.84,146.94) --
	(131.56,146.94) --
	(131.56,150.08) --
	(139.82,150.08) --
	(139.82,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 39.01, 65.34) --
	( 39.01, 68.48) --
	( 46.28, 68.48) --
	( 46.28, 71.62) --
	( 46.61, 71.62) --
	( 46.61, 74.76) --
	( 48.48, 74.76) --
	( 48.48, 77.90) --
	( 51.05, 77.90) --
	( 51.05, 81.03) --
	( 51.71, 81.03) --
	( 51.71, 84.17) --
	( 56.61, 84.17) --
	( 56.61, 87.31) --
	( 57.83, 87.31) --
	( 57.83, 90.45) --
	( 61.46, 90.45) --
	( 61.46, 93.59) --
	( 62.27, 93.59) --
	( 62.27, 96.73) --
	( 62.61, 96.73) --
	( 62.61, 99.86) --
	( 63.80, 99.86) --
	( 63.80,103.00) --
	( 64.69,103.00) --
	( 64.69,106.14) --
	( 70.57,106.14) --
	( 70.57,109.28) --
	( 71.79,109.28) --
	( 71.79,112.42) --
	( 76.55,112.42) --
	( 76.55,115.55) --
	( 81.87,115.55) --
	( 81.87,118.69) --
	( 83.69,118.69) --
	( 83.69,121.83) --
	( 86.03,121.83) --
	( 86.03,124.97) --
	( 88.59,124.97) --
	( 88.59,128.11) --
	(119.63,128.11) --
	(119.63,131.25) --
	(121.69,131.25) --
	(121.69,134.38) --
	(125.82,134.38) --
	(125.82,137.52) --
	(126.37,137.52) --
	(126.37,140.66) --
	(127.35,140.66) --
	(127.35,143.80) --
	(129.60,143.80) --
	(129.60,146.94) --
	(142.24,146.94) --
	(142.24,150.08) --
	(143.68,150.08) --
	(143.68,153.21) --
	(203.49,153.21) --
	(203.49,153.21);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 38.33, 65.34) --
	( 38.33, 68.48) --
	( 42.50, 68.48) --
	( 42.50, 71.62) --
	( 48.53, 71.62) --
	( 48.53, 74.76) --
	( 49.56, 74.76) --
	( 49.56, 77.90) --
	( 53.88, 77.90) --
	( 53.88, 81.03) --
	( 55.68, 81.03) --
	( 55.68, 84.17) --
	( 55.92, 84.17) --
	( 55.92, 87.31) --
	( 57.12, 87.31) --
	( 57.12, 90.45) --
	( 57.35, 90.45) --
	( 57.35, 93.59) --
	( 61.32, 93.59) --
	( 61.32, 96.73) --
	( 62.26, 96.73) --
	( 62.26, 99.86) --
	( 64.66, 99.86) --
	( 64.66,103.00) --
	( 66.14,103.00) --
	( 66.14,106.14) --
	( 69.87,106.14) --
	( 69.87,109.28) --
	( 71.16,109.28) --
	( 71.16,112.42) --
	( 75.38,112.42) --
	( 75.38,115.55) --
	( 83.09,115.55) --
	( 83.09,118.69) --
	( 83.26,118.69) --
	( 83.26,121.83) --
	( 85.90,121.83) --
	( 85.90,124.97) --
	( 86.95,124.97) --
	( 86.95,128.11) --
	(123.07,128.11) --
	(123.07,131.25) --
	(125.57,131.25) --
	(125.57,134.38) --
	(127.01,134.38) --
	(127.01,137.52) --
	(129.09,137.52) --
	(129.09,140.66) --
	(132.95,140.66) --
	(132.95,143.80) --
	(137.52,143.80) --
	(137.52,146.94) --
	(176.42,146.94) --
	(176.42,150.08) --
	(203.49,150.08) --
	(203.49,150.08);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 41.44, 65.34) --
	( 41.44, 68.48) --
	( 46.90, 68.48) --
	( 46.90, 71.62) --
	( 48.76, 71.62) --
	( 48.76, 74.76) --
	( 54.24, 74.76) --
	( 54.24, 77.90) --
	( 57.09, 77.90) --
	( 57.09, 81.03) --
	( 57.95, 81.03) --
	( 57.95, 84.17) --
	( 59.10, 84.17) --
	( 59.10, 87.31) --
	( 62.73, 87.31) --
	( 62.73, 90.45) --
	( 63.38, 90.45) --
	( 63.38, 93.59) --
	( 65.58, 93.59) --
	( 65.58, 96.73) --
	( 66.73, 96.73) --
	( 66.73, 99.86) --
	( 69.80, 99.86) --
	( 69.80,103.00) --
	( 69.83,103.00) --
	( 69.83,106.14) --
	( 69.98,106.14) --
	( 69.98,109.28) --
	( 81.16,109.28) --
	( 81.16,112.42) --
	( 81.46,112.42) --
	( 81.46,115.55) --
	( 85.03,115.55) --
	( 85.03,118.69) --
	( 87.05,118.69) --
	( 87.05,121.83) --
	( 88.44,121.83) --
	( 88.44,124.97) --
	( 92.68,124.97) --
	( 92.68,128.11) --
	(122.16,128.11) --
	(122.16,131.25) --
	(126.47,131.25) --
	(126.47,134.38) --
	(203.49,134.38) --
	(203.49,134.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 36.99, 65.34) --
	( 47.65, 65.34) --
	( 47.65, 68.48) --
	( 47.84, 68.48) --
	( 47.84, 71.62) --
	( 52.04, 71.62) --
	( 52.04, 74.76) --
	( 55.04, 74.76) --
	( 55.04, 77.90) --
	( 56.21, 77.90) --
	( 56.21, 81.03) --
	( 58.02, 81.03) --
	( 58.02, 84.17) --
	( 58.97, 84.17) --
	( 58.97, 87.31) --
	( 63.42, 87.31) --
	( 63.42, 90.45) --
	( 65.64, 90.45) --
	( 65.64, 93.59) --
	( 66.88, 93.59) --
	( 66.88, 96.73) --
	( 68.68, 96.73) --
	( 68.68, 99.86) --
	( 69.53, 99.86) --
	( 69.53,103.00) --
	( 70.53,103.00) --
	( 70.53,106.14) --
	( 71.18,106.14) --
	( 71.18,109.28) --
	( 72.15,109.28) --
	( 72.15,112.42) --
	( 80.81,112.42) --
	( 80.81,115.55) --
	( 82.96,115.55) --
	( 82.96,118.69) --
	( 85.95,118.69) --
	( 85.95,121.83) --
	( 87.48,121.83) --
	( 87.48,124.97) --
	( 91.57,124.97) --
	( 91.57,128.11) --
	(123.88,128.11) --
	(123.88,131.25) --
	(131.87,131.25) --
	(131.87,134.38) --
	(155.80,134.38) --
	(155.80,137.52) --
	(156.03,137.52) --
	(156.03,140.66) --
	(192.94,140.66) --
	(192.94,143.80) --
	(203.49,143.80) --
	(203.49,143.80);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 27.12, 60.95) -- ( 27.12, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 35.97, 60.95) -- ( 35.97, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 41.14, 60.95) -- ( 41.14, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 44.81, 60.95) -- ( 44.81, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 47.66, 60.95) -- ( 47.66, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 49.99, 60.95) -- ( 49.99, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 51.96, 60.95) -- ( 51.96, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 53.66, 60.95) -- ( 53.66, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 55.17, 60.95) -- ( 55.17, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 56.51, 60.95) -- ( 56.51, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 65.36, 60.95) -- ( 65.36, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 70.54, 60.95) -- ( 70.54, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 74.21, 60.95) -- ( 74.21, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 77.06, 60.95) -- ( 77.06, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 79.39, 60.95) -- ( 79.39, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 81.35, 60.95) -- ( 81.35, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 83.06, 60.95) -- ( 83.06, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 84.56, 60.95) -- ( 84.56, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 85.91, 60.95) -- ( 85.91, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 94.76, 60.95) -- ( 94.76, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 99.93, 60.95) -- ( 99.93, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (103.60, 60.95) -- (103.60, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (106.45, 60.95) -- (106.45, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (108.78, 60.95) -- (108.78, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (110.75, 60.95) -- (110.75, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (112.45, 60.95) -- (112.45, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (113.96, 60.95) -- (113.96, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (115.30, 60.95) -- (115.30, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (124.15, 60.95) -- (124.15, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (129.33, 60.95) -- (129.33, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (133.00, 60.95) -- (133.00, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (135.85, 60.95) -- (135.85, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (138.17, 60.95) -- (138.17, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (140.14, 60.95) -- (140.14, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (141.85, 60.95) -- (141.85, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (143.35, 60.95) -- (143.35, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (144.70, 60.95) -- (144.70, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (153.54, 60.95) -- (153.54, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (158.72, 60.95) -- (158.72, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (162.39, 60.95) -- (162.39, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (165.24, 60.95) -- (165.24, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (167.57, 60.95) -- (167.57, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (169.54, 60.95) -- (169.54, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (171.24, 60.95) -- (171.24, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (172.75, 60.95) -- (172.75, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (174.09, 60.95) -- (174.09, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (182.94, 60.95) -- (182.94, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (188.12, 60.95) -- (188.12, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (191.79, 60.95) -- (191.79, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (194.64, 60.95) -- (194.64, 63.79);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (196.96, 60.95) -- (196.96, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (198.93, 60.95) -- (198.93, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (200.64, 60.95) -- (200.64, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (202.14, 60.95) -- (202.14, 62.37);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (203.49, 60.95) -- (203.49, 65.22);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (212.33, 60.95) -- (212.33, 62.37);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 28.66, 60.95) rectangle (211.81,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 28.66, 60.95) --
	( 28.66,157.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16, 62.59) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16, 93.97) {10};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 24.16,125.35) {20};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16, 65.34) --
	( 28.66, 65.34);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16, 96.73) --
	( 28.66, 96.73);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 26.16,128.11) --
	( 28.66,128.11);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 28.66, 60.95) --
	(211.81, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 56.51, 58.45) --
	( 56.51, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 85.91, 58.45) --
	( 85.91, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (115.30, 58.45) --
	(115.30, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (144.70, 58.45) --
	(144.70, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (174.09, 58.45) --
	(174.09, 60.95);

\path[draw=drawColor,line width= 0.5pt,line join=round] (203.49, 58.45) --
	(203.49, 60.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 50.31, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 58.14, 52.84) {-2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 79.71, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at ( 87.54, 52.84) {-1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (110.01, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (117.85, 52.84) {0};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (139.41, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (147.24, 52.84) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (168.80, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (176.64, 52.84) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (198.20, 49.57) {10};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.47] at (206.03, 52.84) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (120.24, 38.62) {Time [s]};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 11.89,109.28) {Solved instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41, 23.07) -- ( 66.29, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41, 15.84) -- ( 66.29, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 52.41,  8.61) -- ( 66.29,  8.61);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.13, 23.07) -- (145.01, 23.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.13, 15.84) -- (145.01, 15.84);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02, 20.31) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02, 13.09) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.02,  5.86) {Non-Increasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.75, 20.31) {Basic-Dense};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,162.61);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.75, 13.09) {Basic-Sparse};
\end{scope}
\end{tikzpicture}


==> plots/graph_size_performance_plots/fe.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:53:25
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,155.38);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 47.21,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 59.84) {0.00};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 80.62) {0.25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,101.40) {0.50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,122.19) {0.75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,142.97) {1.00};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 62.59) --
	( 47.21, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 83.38) --
	( 47.21, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,104.16) --
	( 47.21,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,124.94) --
	( 47.21,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,145.72) --
	( 47.21,145.72);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 24.07,104.16) {Fraction of instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 62.59) --
	( 99.78, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 83.38) --
	( 99.78, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,104.16) --
	( 99.78,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,124.94) --
	( 99.78,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,145.72) --
	( 99.78,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 58.44) --
	( 47.73,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 58.44) --
	( 73.75,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 58.44) --
	( 99.78,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 52.93, 57.19) -- ( 52.93, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 58.14, 57.19) -- ( 58.14, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.34, 57.19) -- ( 63.34, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 68.55, 57.19) -- ( 68.55, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 78.96, 57.19) -- ( 78.96, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 84.16, 57.19) -- ( 84.16, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 89.37, 57.19) -- ( 89.37, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 94.57, 57.19) -- ( 94.57, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73, 74.47) --
	( 47.73, 74.47) --
	( 47.73, 74.47) --
	( 97.80, 74.47) --
	( 97.80, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 98.22) --
	( 99.78, 98.22) --
	( 99.78,110.10) --
	( 99.78,110.10) --
	( 99.78,110.10);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73, 86.34) --
	( 47.73, 86.34) --
	( 47.73, 86.34) --
	( 59.26, 86.34) --
	( 59.26, 98.22) --
	( 99.78, 98.22) --
	( 99.78, 98.22) --
	( 99.78, 98.22) --
	( 99.78,110.10) --
	( 99.78,110.10) --
	( 99.78,121.97) --
	( 99.78,121.97) --
	( 99.78,121.97) --
	( 99.78,121.97) --
	( 99.78,121.97);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,133.85) --
	( 47.73,133.85) --
	( 47.73,133.85) --
	( 99.78,133.85) --
	( 99.78,133.85) --
	( 99.78,133.85) --
	( 99.78,133.85) --
	( 99.78,133.85) --
	( 99.78,133.85);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73, 62.59) --
	( 61.07, 62.59) --
	( 61.07, 74.47) --
	( 99.78, 74.47) --
	( 99.78, 74.47) --
	( 99.78, 74.47) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 86.34) --
	( 99.78, 98.22) --
	( 99.78, 98.22) --
	( 99.78, 98.22);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 99.38, 58.44) rectangle (151.95,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 62.59) --
	(151.95, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 83.38) --
	(151.95, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,104.16) --
	(151.95,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,124.94) --
	(151.95,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 58.44) --
	(122.74,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 58.44) --
	(151.95,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (105.22, 57.19) -- (105.22, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (111.06, 57.19) -- (111.06, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (116.90, 57.19) -- (116.90, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (128.58, 57.19) -- (128.58, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (134.43, 57.19) -- (134.43, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (140.27, 57.19) -- (140.27, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.11, 57.19) -- (146.11, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38, 86.34) --
	(151.95, 86.34) --
	(151.95, 86.34) --
	(151.95, 86.34) --
	(151.95, 98.22) --
	(151.95, 98.22) --
	(151.95,110.10) --
	(151.95,110.10) --
	(151.95,110.10);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38, 98.22) --
	(101.14, 98.22) --
	(101.14,110.10) --
	(118.94,110.10) --
	(118.94,121.97) --
	(151.95,121.97) --
	(151.95,121.97) --
	(151.95,121.97) --
	(151.95,121.97);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,133.85) --
	(151.95,133.85) --
	(151.95,133.85) --
	(151.95,133.85) --
	(151.95,133.85);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38, 74.47) --
	(140.92, 74.47) --
	(140.92, 86.34) --
	(151.95, 86.34) --
	(151.95, 86.34) --
	(151.95, 86.34) --
	(151.95, 98.22) --
	(151.95, 98.22) --
	(151.95, 98.22);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 99.38, 58.44) rectangle (151.95,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (151.55, 58.44) rectangle (204.12,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 62.59) --
	(204.12, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 83.38) --
	(204.12, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,104.16) --
	(204.12,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,124.94) --
	(204.12,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,145.72) --
	(204.12,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 58.44) --
	(165.17,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 58.44) --
	(184.64,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 58.44) --
	(204.12,149.88);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55, 86.34) --
	(153.26, 86.34) --
	(153.26, 98.22) --
	(174.15, 98.22) --
	(174.15,110.10) --
	(204.12,110.10) --
	(204.12,110.10);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,121.97) --
	(204.12,121.97) --
	(204.12,121.97);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,133.85) --
	(204.12,133.85) --
	(204.12,133.85);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55, 86.34) --
	(151.97, 86.34) --
	(151.97, 98.22) --
	(204.12, 98.22) --
	(204.12, 98.22);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (151.55, 58.44) rectangle (204.12,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 55.94) --
	( 47.73, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 55.94) --
	( 73.75, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 55.94) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 47.73, 48.43) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.75, 48.43) {1.05};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 55.94) --
	( 99.38, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 55.94) --
	(122.74, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 55.94) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 99.38, 48.43) {1.1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (122.74, 48.43) {1.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.95, 48.43) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (125.66, 37.27) {Graph size relative to best};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62, 16.30) -- ( 54.49, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62,  8.77) -- ( 54.49,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72, 16.30) -- (131.60, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72,  8.77) -- (131.60,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23, 13.54) {Basic-Sparse};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23,  6.01) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33, 13.54) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33,  6.01) {NonIncreasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 55.94) --
	(151.55, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 55.94) --
	(165.17, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 55.94) --
	(184.64, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 55.94) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (165.17, 48.43) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (184.64, 48.43) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (204.12, 48.43) {1000};
\end{scope}
\end{tikzpicture}


==> plots/graph_size_performance_plots/mesh.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:53:43
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,155.38);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 47.21,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 59.84) {0.00};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 80.62) {0.25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,101.40) {0.50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,122.19) {0.75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,142.97) {1.00};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 62.59) --
	( 47.21, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 83.38) --
	( 47.21, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,104.16) --
	( 47.21,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,124.94) --
	( 47.21,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,145.72) --
	( 47.21,145.72);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 24.07,104.16) {Fraction of instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 62.59) --
	( 99.78, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 83.38) --
	( 99.78, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,104.16) --
	( 99.78,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,124.94) --
	( 99.78,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,145.72) --
	( 99.78,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 58.44) --
	( 47.73,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 58.44) --
	( 73.75,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 58.44) --
	( 99.78,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 52.93, 57.19) -- ( 52.93, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 58.14, 57.19) -- ( 58.14, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.34, 57.19) -- ( 63.34, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 68.55, 57.19) -- ( 68.55, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 78.96, 57.19) -- ( 78.96, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 84.16, 57.19) -- ( 84.16, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 89.37, 57.19) -- ( 89.37, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 94.57, 57.19) -- ( 94.57, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73, 62.59) --
	( 99.78, 62.59) --
	( 99.78, 62.59) --
	( 99.78, 62.59) --
	( 99.78, 62.59) --
	( 99.78, 62.59) --
	( 99.78, 62.59);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,145.72) --
	( 47.73,145.72) --
	( 47.73,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,145.72) --
	( 47.73,145.72) --
	( 47.73,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,118.01) --
	( 47.73,118.01) --
	( 47.73,118.01) --
	( 99.78,118.01) --
	( 99.78,118.01) --
	( 99.78,118.01) --
	( 99.78,118.01) --
	( 99.78,118.01) --
	( 99.78,118.01);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 99.38, 58.44) rectangle (151.95,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 62.59) --
	(151.95, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 83.38) --
	(151.95, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,104.16) --
	(151.95,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,124.94) --
	(151.95,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 58.44) --
	(122.74,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 58.44) --
	(151.95,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (105.22, 57.19) -- (105.22, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (111.06, 57.19) -- (111.06, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (116.90, 57.19) -- (116.90, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (128.58, 57.19) -- (128.58, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (134.43, 57.19) -- (134.43, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (140.27, 57.19) -- (140.27, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.11, 57.19) -- (146.11, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38, 62.59) --
	(151.95, 62.59) --
	(151.95, 62.59) --
	(151.95, 62.59) --
	(151.95, 62.59);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,118.01) --
	(151.95,118.01) --
	(151.95,118.01) --
	(151.95,118.01) --
	(151.95,118.01);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 99.38, 58.44) rectangle (151.95,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (151.55, 58.44) rectangle (204.12,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 62.59) --
	(204.12, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 83.38) --
	(204.12, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,104.16) --
	(204.12,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,124.94) --
	(204.12,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,145.72) --
	(204.12,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 58.44) --
	(165.17,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 58.44) --
	(184.64,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 58.44) --
	(204.12,149.88);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55, 62.59) --
	(204.12, 62.59) --
	(204.12, 62.59);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,145.72) --
	(204.12,145.72) --
	(204.12,145.72);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,145.72) --
	(204.12,145.72) --
	(204.12,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,118.01) --
	(204.12,118.01) --
	(204.12,118.01);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (151.55, 58.44) rectangle (204.12,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 55.94) --
	( 47.73, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 55.94) --
	( 73.75, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 55.94) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 47.73, 48.43) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.75, 48.43) {1.05};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 55.94) --
	( 99.38, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 55.94) --
	(122.74, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 55.94) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 99.38, 48.43) {1.1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (122.74, 48.43) {1.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.95, 48.43) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (125.66, 37.27) {Graph size relative to best};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62, 16.30) -- ( 54.49, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62,  8.77) -- ( 54.49,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72, 16.30) -- (131.60, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72,  8.77) -- (131.60,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23, 13.54) {Basic-Sparse};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23,  6.01) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33, 13.54) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33,  6.01) {NonIncreasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 55.94) --
	(151.55, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 55.94) --
	(165.17, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 55.94) --
	(184.64, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 55.94) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (165.17, 48.43) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (184.64, 48.43) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (204.12, 48.43) {1000};
\end{scope}
\end{tikzpicture}


==> plots/graph_size_performance_plots/osm.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:53:59
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,155.38);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 47.21,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 59.84) {0.00};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 80.62) {0.25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,101.40) {0.50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,122.19) {0.75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,142.97) {1.00};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 62.59) --
	( 47.21, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 83.38) --
	( 47.21, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,104.16) --
	( 47.21,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,124.94) --
	( 47.21,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,145.72) --
	( 47.21,145.72);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 24.07,104.16) {Fraction of instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 62.59) --
	( 99.78, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 83.38) --
	( 99.78, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,104.16) --
	( 99.78,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,124.94) --
	( 99.78,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,145.72) --
	( 99.78,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 58.44) --
	( 47.73,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 58.44) --
	( 73.75,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 58.44) --
	( 99.78,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 52.93, 57.19) -- ( 52.93, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 58.14, 57.19) -- ( 58.14, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.34, 57.19) -- ( 63.34, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 68.55, 57.19) -- ( 68.55, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 78.96, 57.19) -- ( 78.96, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 84.16, 57.19) -- ( 84.16, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 89.37, 57.19) -- ( 89.37, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 94.57, 57.19) -- ( 94.57, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73, 62.59) --
	( 63.28, 62.59) --
	( 63.28, 65.04) --
	( 87.12, 65.04) --
	( 87.12, 67.48) --
	( 99.78, 67.48) --
	( 99.78, 67.48) --
	( 99.78, 67.48) --
	( 99.78, 69.93) --
	( 99.78, 69.93) --
	( 99.78, 72.37) --
	( 99.78, 72.37) --
	( 99.78, 74.82) --
	( 99.78, 74.82) --
	( 99.78, 77.26) --
	( 99.78, 77.26) --
	( 99.78, 79.71) --
	( 99.78, 79.71) --
	( 99.78, 82.15) --
	( 99.78, 82.15) --
	( 99.78, 84.60) --
	( 99.78, 84.60) --
	( 99.78, 87.04) --
	( 99.78, 87.04) --
	( 99.78, 89.49) --
	( 99.78, 89.49) --
	( 99.78, 91.93) --
	( 99.78, 91.93) --
	( 99.78, 94.38) --
	( 99.78, 94.38) --
	( 99.78, 96.82) --
	( 99.78, 96.82) --
	( 99.78, 96.82) --
	( 99.78, 96.82) --
	( 99.78, 99.27) --
	( 99.78, 99.27) --
	( 99.78,101.71) --
	( 99.78,101.71) --
	( 99.78,104.16) --
	( 99.78,104.16) --
	( 99.78,104.16);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,101.71) --
	( 47.73,101.71) --
	( 47.73,101.71) --
	( 49.00,101.71) --
	( 49.00,104.16) --
	( 53.04,104.16) --
	( 53.04,106.60) --
	( 53.83,106.60) --
	( 53.83,109.05) --
	( 56.45,109.05) --
	( 56.45,111.49) --
	( 73.75,111.49) --
	( 73.75,113.94) --
	( 92.64,113.94) --
	( 92.64,116.38) --
	( 94.87,116.38) --
	( 94.87,118.83) --
	( 99.78,118.83) --
	( 99.78,118.83) --
	( 99.78,118.83) --
	( 99.78,121.27) --
	( 99.78,121.27) --
	( 99.78,123.72) --
	( 99.78,123.72) --
	( 99.78,126.16) --
	( 99.78,126.16) --
	( 99.78,128.61) --
	( 99.78,128.61) --
	( 99.78,131.05) --
	( 99.78,131.05) --
	( 99.78,133.50) --
	( 99.78,133.50) --
	( 99.78,135.94) --
	( 99.78,135.94) --
	( 99.78,135.94) --
	( 99.78,135.94) --
	( 99.78,138.39) --
	( 99.78,138.39) --
	( 99.78,138.39);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,145.72) --
	( 47.73,145.72) --
	( 47.73,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73, 72.37) --
	( 47.73, 72.37) --
	( 47.73, 72.37) --
	( 59.29, 72.37) --
	( 59.29, 74.82) --
	( 85.00, 74.82) --
	( 85.00, 77.26) --
	( 99.78, 77.26) --
	( 99.78, 77.26) --
	( 99.78, 77.26) --
	( 99.78, 79.71) --
	( 99.78, 79.71) --
	( 99.78, 82.15) --
	( 99.78, 82.15) --
	( 99.78, 84.60) --
	( 99.78, 84.60) --
	( 99.78, 87.04) --
	( 99.78, 87.04) --
	( 99.78, 89.49) --
	( 99.78, 89.49) --
	( 99.78, 91.93) --
	( 99.78, 91.93) --
	( 99.78, 94.38) --
	( 99.78, 94.38) --
	( 99.78, 96.82) --
	( 99.78, 96.82) --
	( 99.78, 99.27) --
	( 99.78, 99.27) --
	( 99.78,101.71) --
	( 99.78,101.71) --
	( 99.78,104.16) --
	( 99.78,104.16) --
	( 99.78,106.60) --
	( 99.78,106.60) --
	( 99.78,109.05) --
	( 99.78,109.05) --
	( 99.78,109.05) --
	( 99.78,109.05) --
	( 99.78,111.49) --
	( 99.78,111.49) --
	( 99.78,113.94) --
	( 99.78,113.94) --
	( 99.78,113.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 99.38, 58.44) rectangle (151.95,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 62.59) --
	(151.95, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 83.38) --
	(151.95, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,104.16) --
	(151.95,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,124.94) --
	(151.95,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 58.44) --
	(122.74,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 58.44) --
	(151.95,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (105.22, 57.19) -- (105.22, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (111.06, 57.19) -- (111.06, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (116.90, 57.19) -- (116.90, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (128.58, 57.19) -- (128.58, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (134.43, 57.19) -- (134.43, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (140.27, 57.19) -- (140.27, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.11, 57.19) -- (146.11, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38, 67.48) --
	( 99.54, 67.48) --
	( 99.54, 69.93) --
	(100.83, 69.93) --
	(100.83, 72.37) --
	(102.81, 72.37) --
	(102.81, 74.82) --
	(104.09, 74.82) --
	(104.09, 77.26) --
	(106.99, 77.26) --
	(106.99, 79.71) --
	(110.25, 79.71) --
	(110.25, 82.15) --
	(111.28, 82.15) --
	(111.28, 84.60) --
	(112.99, 84.60) --
	(112.99, 87.04) --
	(113.91, 87.04) --
	(113.91, 89.49) --
	(123.81, 89.49) --
	(123.81, 91.93) --
	(133.42, 91.93) --
	(133.42, 94.38) --
	(144.14, 94.38) --
	(144.14, 96.82) --
	(151.95, 96.82) --
	(151.95, 96.82) --
	(151.95, 96.82) --
	(151.95, 99.27) --
	(151.95, 99.27) --
	(151.95,101.71) --
	(151.95,101.71) --
	(151.95,104.16) --
	(151.95,104.16) --
	(151.95,104.16);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,118.83) --
	( 99.96,118.83) --
	( 99.96,121.27) --
	(100.52,121.27) --
	(100.52,123.72) --
	(102.43,123.72) --
	(102.43,126.16) --
	(108.14,126.16) --
	(108.14,128.61) --
	(108.48,128.61) --
	(108.48,131.05) --
	(115.80,131.05) --
	(115.80,133.50) --
	(130.59,133.50) --
	(130.59,135.94) --
	(151.95,135.94) --
	(151.95,135.94) --
	(151.95,135.94) --
	(151.95,138.39) --
	(151.95,138.39) --
	(151.95,138.39);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38, 77.26) --
	( 99.44, 77.26) --
	( 99.44, 79.71) --
	( 99.46, 79.71) --
	( 99.46, 82.15) --
	(100.51, 82.15) --
	(100.51, 84.60) --
	(102.12, 84.60) --
	(102.12, 87.04) --
	(104.13, 87.04) --
	(104.13, 89.49) --
	(104.28, 89.49) --
	(104.28, 91.93) --
	(107.67, 91.93) --
	(107.67, 94.38) --
	(110.55, 94.38) --
	(110.55, 96.82) --
	(112.06, 96.82) --
	(112.06, 99.27) --
	(120.85, 99.27) --
	(120.85,101.71) --
	(130.75,101.71) --
	(130.75,104.16) --
	(140.40,104.16) --
	(140.40,106.60) --
	(144.53,106.60) --
	(144.53,109.05) --
	(151.95,109.05) --
	(151.95,109.05) --
	(151.95,109.05) --
	(151.95,111.49) --
	(151.95,111.49) --
	(151.95,113.94) --
	(151.95,113.94) --
	(151.95,113.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 99.38, 58.44) rectangle (151.95,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (151.55, 58.44) rectangle (204.12,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 62.59) --
	(204.12, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 83.38) --
	(204.12, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,104.16) --
	(204.12,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,124.94) --
	(204.12,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,145.72) --
	(204.12,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 58.44) --
	(165.17,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 58.44) --
	(184.64,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 58.44) --
	(204.12,149.88);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55, 96.82) --
	(151.66, 96.82) --
	(151.66, 99.27) --
	(157.42, 99.27) --
	(157.42,101.71) --
	(158.00,101.71) --
	(158.00,104.16) --
	(204.12,104.16) --
	(204.12,104.16);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,135.94) --
	(153.36,135.94) --
	(153.36,138.39) --
	(204.12,138.39) --
	(204.12,138.39);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,145.72) --
	(204.12,145.72) --
	(204.12,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,109.05) --
	(155.12,109.05) --
	(155.12,111.49) --
	(156.93,111.49) --
	(156.93,113.94) --
	(204.12,113.94) --
	(204.12,113.94);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (151.55, 58.44) rectangle (204.12,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 55.94) --
	( 47.73, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 55.94) --
	( 73.75, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 55.94) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 47.73, 48.43) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.75, 48.43) {1.05};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 55.94) --
	( 99.38, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 55.94) --
	(122.74, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 55.94) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 99.38, 48.43) {1.1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (122.74, 48.43) {1.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.95, 48.43) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (125.66, 37.27) {Graph size relative to best};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62, 16.30) -- ( 54.49, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62,  8.77) -- ( 54.49,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72, 16.30) -- (131.60, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72,  8.77) -- (131.60,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23, 13.54) {Basic-Sparse};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23,  6.01) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33, 13.54) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33,  6.01) {NonIncreasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 55.94) --
	(151.55, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 55.94) --
	(165.17, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 55.94) --
	(184.64, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 55.94) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (165.17, 48.43) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (184.64, 48.43) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (204.12, 48.43) {1000};
\end{scope}
\end{tikzpicture}


==> plots/graph_size_performance_plots/snap.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:54:17
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,155.38);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 47.21,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 59.84) {0.00};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71, 80.62) {0.25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,101.40) {0.50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,122.19) {0.75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 42.71,142.97) {1.00};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 62.59) --
	( 47.21, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71, 83.38) --
	( 47.21, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,104.16) --
	( 47.21,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,124.94) --
	( 47.21,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 44.71,145.72) --
	( 47.21,145.72);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 24.07,104.16) {Fraction of instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 62.59) --
	( 99.78, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21, 83.38) --
	( 99.78, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,104.16) --
	( 99.78,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,124.94) --
	( 99.78,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.21,145.72) --
	( 99.78,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 58.44) --
	( 47.73,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 58.44) --
	( 73.75,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 58.44) --
	( 99.78,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 52.93, 57.19) -- ( 52.93, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 58.14, 57.19) -- ( 58.14, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.34, 57.19) -- ( 63.34, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 68.55, 57.19) -- ( 68.55, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 78.96, 57.19) -- ( 78.96, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 84.16, 57.19) -- ( 84.16, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 89.37, 57.19) -- ( 89.37, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 94.57, 57.19) -- ( 94.57, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,118.91) --
	( 47.73,118.91) --
	( 47.73,118.91) --
	( 99.78,118.91) --
	( 99.78,118.91) --
	( 99.78,118.91) --
	( 99.78,121.59) --
	( 99.78,121.59) --
	( 99.78,121.59) --
	( 99.78,121.59) --
	( 99.78,124.27) --
	( 99.78,124.27) --
	( 99.78,126.95) --
	( 99.78,126.95) --
	( 99.78,129.63) --
	( 99.78,129.63) --
	( 99.78,132.32) --
	( 99.78,132.32) --
	( 99.78,135.00) --
	( 99.78,135.00) --
	( 99.78,135.00);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,135.00) --
	( 47.73,135.00) --
	( 47.73,135.00) --
	( 47.74,135.00) --
	( 47.74,137.68) --
	( 99.78,137.68) --
	( 99.78,137.68) --
	( 99.78,137.68) --
	( 99.78,140.36) --
	( 99.78,140.36) --
	( 99.78,140.36) --
	( 99.78,140.36) --
	( 99.78,143.04) --
	( 99.78,143.04) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,145.72) --
	( 47.73,145.72) --
	( 47.73,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72) --
	( 99.78,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 47.73,118.91) --
	( 47.73,118.91) --
	( 47.73,118.91) --
	( 48.46,118.91) --
	( 48.46,121.59) --
	( 99.78,121.59) --
	( 99.78,121.59) --
	( 99.78,121.59) --
	( 99.78,124.27) --
	( 99.78,124.27) --
	( 99.78,124.27) --
	( 99.78,124.27) --
	( 99.78,126.95) --
	( 99.78,126.95) --
	( 99.78,129.63) --
	( 99.78,129.63) --
	( 99.78,132.32) --
	( 99.78,132.32) --
	( 99.78,135.00) --
	( 99.78,135.00) --
	( 99.78,135.00);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 47.21, 58.44) rectangle ( 99.78,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 99.38, 58.44) rectangle (151.95,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 62.59) --
	(151.95, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 83.38) --
	(151.95, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,104.16) --
	(151.95,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,124.94) --
	(151.95,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 58.44) --
	( 99.38,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 58.44) --
	(122.74,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 58.44) --
	(151.95,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (105.22, 57.19) -- (105.22, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (111.06, 57.19) -- (111.06, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (116.90, 57.19) -- (116.90, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (128.58, 57.19) -- (128.58, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (134.43, 57.19) -- (134.43, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (140.27, 57.19) -- (140.27, 58.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.11, 57.19) -- (146.11, 58.44);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,118.91) --
	(100.15,118.91) --
	(100.15,121.59) --
	(151.95,121.59) --
	(151.95,121.59) --
	(151.95,121.59) --
	(151.95,124.27) --
	(151.95,124.27) --
	(151.95,126.95) --
	(151.95,126.95) --
	(151.95,129.63) --
	(151.95,129.63) --
	(151.95,132.32) --
	(151.95,132.32) --
	(151.95,135.00) --
	(151.95,135.00) --
	(151.95,135.00);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,137.68) --
	(104.48,137.68) --
	(104.48,140.36) --
	(151.95,140.36) --
	(151.95,140.36) --
	(151.95,140.36) --
	(151.95,143.04) --
	(151.95,143.04) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72) --
	(151.95,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 99.38,121.59) --
	(120.54,121.59) --
	(120.54,124.27) --
	(151.95,124.27) --
	(151.95,124.27) --
	(151.95,124.27) --
	(151.95,126.95) --
	(151.95,126.95) --
	(151.95,129.63) --
	(151.95,129.63) --
	(151.95,132.32) --
	(151.95,132.32) --
	(151.95,135.00) --
	(151.95,135.00) --
	(151.95,135.00);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 99.38, 58.44) rectangle (151.95,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (151.55, 58.44) rectangle (204.12,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 62.59) --
	(204.12, 62.59);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 83.38) --
	(204.12, 83.38);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,104.16) --
	(204.12,104.16);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,124.94) --
	(204.12,124.94);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55,145.72) --
	(204.12,145.72);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 58.44) --
	(151.55,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 58.44) --
	(165.17,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 58.44) --
	(184.64,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 58.44) --
	(204.12,149.88);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,121.59) --
	(156.67,121.59) --
	(156.67,124.27) --
	(172.01,124.27) --
	(172.01,126.95) --
	(173.65,126.95) --
	(173.65,129.63) --
	(179.07,129.63) --
	(179.07,132.32) --
	(185.48,132.32) --
	(185.48,135.00) --
	(204.12,135.00) --
	(204.12,135.00);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,140.36) --
	(154.05,140.36) --
	(154.05,143.04) --
	(169.96,143.04) --
	(169.96,145.72) --
	(204.12,145.72) --
	(204.12,145.72);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,145.72) --
	(204.12,145.72) --
	(204.12,145.72);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (151.55,124.27) --
	(155.75,124.27) --
	(155.75,126.95) --
	(163.12,126.95) --
	(163.12,129.63) --
	(167.54,129.63) --
	(167.54,132.32) --
	(171.45,132.32) --
	(171.45,135.00) --
	(204.12,135.00) --
	(204.12,135.00);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (151.55, 58.44) rectangle (204.12,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 47.21, 58.44) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 47.73, 55.94) --
	( 47.73, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 73.75, 55.94) --
	( 73.75, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.78, 55.94) --
	( 99.78, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 47.73, 48.43) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 73.75, 48.43) {1.05};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 99.38, 58.44) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 99.38, 55.94) --
	( 99.38, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.74, 55.94) --
	(122.74, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.95, 55.94) --
	(151.95, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 99.38, 48.43) {1.1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (122.74, 48.43) {1.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (151.95, 48.43) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (125.66, 37.27) {Graph size relative to best};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62, 16.30) -- ( 54.49, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 40.62,  8.77) -- ( 54.49,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72, 16.30) -- (131.60, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (117.72,  8.77) -- (131.60,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23, 13.54) {Basic-Sparse};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 61.23,  6.01) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33, 13.54) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (138.33,  6.01) {NonIncreasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (151.55, 58.44) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (151.55, 55.94) --
	(151.55, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (165.17, 55.94) --
	(165.17, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (184.64, 55.94) --
	(184.64, 58.44);

\path[draw=drawColor,line width= 0.5pt,line join=round] (204.12, 55.94) --
	(204.12, 58.44);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (165.17, 48.43) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (184.64, 48.43) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (204.12, 48.43) {1000};
\end{scope}
\end{tikzpicture}


==> plots/struction_amount/end_mi.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}


==> plots/time_performance_plots/fe.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:53:17
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,155.38);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 53.70, 65.97) --
	( 53.70,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20, 67.03) {0.00};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20, 86.10) {0.25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20,105.17) {0.50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20,124.24) {0.75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20,143.31) {1.00};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20, 69.78) --
	( 53.70, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20, 88.85) --
	( 53.70, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20,107.92) --
	( 53.70,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20,127.00) --
	( 53.70,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20,146.07) --
	( 53.70,146.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 30.57,107.92) {Fraction of instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (101.54, 65.97) --
	(101.54,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (149.39, 65.97) --
	(149.39,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 53.70, 65.97) rectangle (101.94,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70, 69.78) --
	(101.94, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70, 88.85) --
	(101.94, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70,107.92) --
	(101.94,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70,127.00) --
	(101.94,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70,146.07) --
	(101.94,146.07);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 54.18, 65.97) --
	( 54.18,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 78.06, 65.97) --
	( 78.06,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.94, 65.97) --
	(101.94,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 58.95, 64.82) -- ( 58.95, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.73, 64.82) -- ( 63.73, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 68.51, 64.82) -- ( 68.51, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 73.28, 64.82) -- ( 73.28, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 82.84, 64.82) -- ( 82.84, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 87.61, 64.82) -- ( 87.61, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 92.39, 64.82) -- ( 92.39, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 97.17, 64.82) -- ( 97.17, 65.97);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 88.85) --
	( 54.18, 88.85) --
	( 54.18, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 88.85) --
	( 54.18, 88.85) --
	( 54.18, 88.85) --
	( 90.21, 88.85) --
	( 90.21,107.92) --
	( 95.46,107.92) --
	( 95.46,127.00) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18,107.92) --
	( 54.18,107.92) --
	( 54.18,107.92) --
	(101.94,107.92) --
	(101.94,107.92) --
	(101.94,107.92) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00) --
	(101.94,127.00);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85) --
	(101.94, 88.85);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 53.70, 65.97) rectangle (101.94,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (101.54, 65.97) rectangle (149.79,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 69.78) --
	(149.79, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 88.85) --
	(149.79, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54,107.92) --
	(149.79,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54,127.00) --
	(149.79,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54,146.07) --
	(149.79,146.07);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 65.97) --
	(101.54,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.98, 65.97) --
	(122.98,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.79, 65.97) --
	(149.79,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (106.90, 64.82) -- (106.90, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (112.26, 64.82) -- (112.26, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.62, 64.82) -- (117.62, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (128.34, 64.82) -- (128.34, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (133.70, 64.82) -- (133.70, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (139.06, 64.82) -- (139.06, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (144.43, 64.82) -- (144.43, 65.97);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54, 69.78) --
	(149.79, 69.78) --
	(149.79, 69.78) --
	(149.79, 69.78) --
	(149.79, 69.78);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54, 88.85) --
	(149.79, 88.85) --
	(149.79, 88.85) --
	(149.79, 88.85) --
	(149.79, 88.85);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54,127.00) --
	(149.79,127.00) --
	(149.79,127.00) --
	(149.79,127.00) --
	(149.79,127.00);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54,107.92) --
	(112.11,107.92) --
	(112.11,127.00) --
	(149.79,127.00) --
	(149.79,127.00) --
	(149.79,127.00) --
	(149.79,127.00);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54, 69.78) --
	(121.15, 69.78) --
	(121.15, 88.85) --
	(149.79, 88.85) --
	(149.79, 88.85) --
	(149.79, 88.85) --
	(149.79, 88.85);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (101.54, 65.97) rectangle (149.79,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (149.39, 65.97) rectangle (197.63,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 69.78) --
	(197.63, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 88.85) --
	(197.63, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39,107.92) --
	(197.63,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39,127.00) --
	(197.63,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39,146.07) --
	(197.63,146.07);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 65.97) --
	(149.39,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (161.88, 65.97) --
	(161.88,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (179.75, 65.97) --
	(179.75,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (197.63, 65.97) --
	(197.63,149.88);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39, 69.78) --
	(197.63, 69.78) --
	(197.63, 69.78);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39, 88.85) --
	(197.63, 88.85) --
	(197.63, 88.85);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39,127.00) --
	(197.63,127.00) --
	(197.63,127.00);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39,127.00) --
	(197.63,127.00) --
	(197.63,127.00);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39, 88.85) --
	(197.63, 88.85) --
	(197.63, 88.85);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (149.39, 65.97) rectangle (197.63,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 53.70, 65.97) --
	(101.94, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 54.18, 63.47) --
	( 54.18, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 78.06, 63.47) --
	( 78.06, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.94, 63.47) --
	(101.94, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 54.18, 55.96) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 78.06, 55.96) {1.05};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (101.54, 65.97) --
	(149.79, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 63.47) --
	(101.54, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.98, 63.47) --
	(122.98, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.79, 63.47) --
	(149.79, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (101.54, 55.96) {1.1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (122.98, 55.96) {1.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (149.79, 55.96) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (125.66, 44.80) {Solving time relative to best};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.29, 23.83) -- ( 68.16, 23.83);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.29, 16.30) -- ( 68.16, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.29,  8.77) -- ( 68.16,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.39, 23.83) -- (145.27, 23.83);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.39, 16.30) -- (145.27, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 74.90, 21.08) {Basic-Dense};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 74.90, 13.54) {Basic-Sparse};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 74.90,  6.01) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (152.01, 21.08) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (152.01, 13.54) {NonIncreasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (149.39, 65.97) --
	(197.63, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 63.47) --
	(149.39, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (161.88, 63.47) --
	(161.88, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (179.75, 63.47) --
	(179.75, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (197.63, 63.47) --
	(197.63, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (161.88, 55.96) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (179.75, 55.96) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (197.63, 55.96) {1000};
\end{scope}
\end{tikzpicture}


==> plots/time_performance_plots/mesh.tex <==
% Created by tikzDevice version 0.12.3 on 2020-06-29 13:53:34
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,155.38);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 53.70, 65.97) --
	( 53.70,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20, 67.03) {0.00};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20, 86.10) {0.25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20,105.17) {0.50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20,124.24) {0.75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 49.20,143.31) {1.00};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20, 69.78) --
	( 53.70, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20, 88.85) --
	( 53.70, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20,107.92) --
	( 53.70,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20,127.00) --
	( 53.70,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 51.20,146.07) --
	( 53.70,146.07);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 30.57,107.92) {Fraction of instances};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (101.54, 65.97) --
	(101.54,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (149.39, 65.97) --
	(149.39,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 53.70, 65.97) rectangle (101.94,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70, 69.78) --
	(101.94, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70, 88.85) --
	(101.94, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70,107.92) --
	(101.94,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70,127.00) --
	(101.94,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 53.70,146.07) --
	(101.94,146.07);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 54.18, 65.97) --
	( 54.18,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 78.06, 65.97) --
	( 78.06,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.94, 65.97) --
	(101.94,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 58.95, 64.82) -- ( 58.95, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.73, 64.82) -- ( 63.73, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 68.51, 64.82) -- ( 68.51, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 73.28, 64.82) -- ( 73.28, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 82.84, 64.82) -- ( 82.84, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 87.61, 64.82) -- ( 87.61, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 92.39, 64.82) -- ( 92.39, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 97.17, 64.82) -- ( 97.17, 65.97);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 74.87) --
	(101.94, 74.87) --
	(101.94, 74.87);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 69.78) --
	(101.94, 74.87) --
	(101.94, 74.87) --
	(101.94, 74.87) --
	(101.94, 74.87) --
	(101.94, 79.95) --
	(101.94, 79.95) --
	(101.94, 85.04) --
	(101.94, 85.04) --
	(101.94, 90.12) --
	(101.94, 90.12) --
	(101.94, 95.21) --
	(101.94, 95.21) --
	(101.94,100.30) --
	(101.94,100.30) --
	(101.94,105.38) --
	(101.94,105.38) --
	(101.94,110.47) --
	(101.94,110.47) --
	(101.94,115.55) --
	(101.94,115.55) --
	(101.94,120.64) --
	(101.94,120.64) --
	(101.94,125.72) --
	(101.94,125.72) --
	(101.94,130.81) --
	(101.94,130.81) --
	(101.94,135.90) --
	(101.94,135.90) --
	(101.94,140.98) --
	(101.94,140.98) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18,110.47) --
	( 54.18,110.47) --
	( 54.18,110.47) --
	( 57.83,110.47) --
	( 57.83,115.55) --
	( 73.60,115.55) --
	( 73.60,120.64) --
	( 85.45,120.64) --
	( 85.45,125.72) --
	( 95.08,125.72) --
	( 95.08,130.81) --
	(101.94,130.81) --
	(101.94,130.81) --
	(101.94,130.81) --
	(101.94,135.90) --
	(101.94,135.90) --
	(101.94,140.98) --
	(101.94,140.98) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 85.04) --
	( 54.18, 85.04) --
	( 54.18, 85.04) --
	( 58.86, 85.04) --
	( 58.86, 90.12) --
	( 60.62, 90.12) --
	( 60.62, 95.21) --
	( 63.18, 95.21) --
	( 63.18,100.30) --
	( 66.71,100.30) --
	( 66.71,105.38) --
	( 81.51,105.38) --
	( 81.51,110.47) --
	( 92.44,110.47) --
	( 92.44,115.55) --
	(101.94,115.55) --
	(101.94,115.55) --
	(101.94,115.55) --
	(101.94,120.64) --
	(101.94,120.64) --
	(101.94,125.72) --
	(101.94,125.72) --
	(101.94,130.81) --
	(101.94,130.81) --
	(101.94,135.90) --
	(101.94,135.90) --
	(101.94,140.98) --
	(101.94,140.98) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.18, 90.12) --
	( 54.18, 90.12) --
	( 54.18, 90.12) --
	( 63.04, 90.12) --
	( 63.04, 95.21) --
	( 70.94, 95.21) --
	( 70.94,100.30) --
	( 75.77,100.30) --
	( 75.77,105.38) --
	( 88.01,105.38) --
	( 88.01,110.47) --
	( 89.89,110.47) --
	( 89.89,115.55) --
	(101.94,115.55) --
	(101.94,115.55) --
	(101.94,115.55) --
	(101.94,120.64) --
	(101.94,120.64) --
	(101.94,125.72) --
	(101.94,125.72) --
	(101.94,130.81) --
	(101.94,130.81) --
	(101.94,135.90) --
	(101.94,135.90) --
	(101.94,140.98) --
	(101.94,140.98) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07) --
	(101.94,146.07);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] ( 53.70, 65.97) rectangle (101.94,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (101.54, 65.97) rectangle (149.79,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 69.78) --
	(149.79, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 88.85) --
	(149.79, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54,107.92) --
	(149.79,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54,127.00) --
	(149.79,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54,146.07) --
	(149.79,146.07);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 65.97) --
	(101.54,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.98, 65.97) --
	(122.98,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.79, 65.97) --
	(149.79,149.88);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (106.90, 64.82) -- (106.90, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (112.26, 64.82) -- (112.26, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.62, 64.82) -- (117.62, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (128.34, 64.82) -- (128.34, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (133.70, 64.82) -- (133.70, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (139.06, 64.82) -- (139.06, 65.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] (144.43, 64.82) -- (144.43, 65.97);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54, 69.78) --
	(149.79, 69.78) --
	(149.79, 69.78) --
	(149.79, 69.78) --
	(149.79, 74.87) --
	(149.79, 74.87) --
	(149.79, 74.87);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54, 69.78) --
	(137.45, 69.78) --
	(137.45, 74.87) --
	(149.79, 74.87) --
	(149.79, 74.87) --
	(149.79, 74.87) --
	(149.79, 79.95) --
	(149.79, 79.95) --
	(149.79, 85.04) --
	(149.79, 85.04) --
	(149.79, 90.12) --
	(149.79, 90.12) --
	(149.79, 95.21) --
	(149.79, 95.21) --
	(149.79,100.30) --
	(149.79,100.30) --
	(149.79,105.38) --
	(149.79,105.38) --
	(149.79,110.47) --
	(149.79,110.47) --
	(149.79,115.55) --
	(149.79,115.55) --
	(149.79,120.64) --
	(149.79,120.64) --
	(149.79,125.72) --
	(149.79,125.72) --
	(149.79,130.81) --
	(149.79,130.81) --
	(149.79,135.90) --
	(149.79,135.90) --
	(149.79,140.98) --
	(149.79,140.98) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54,130.81) --
	(102.69,130.81) --
	(102.69,135.90) --
	(102.91,135.90) --
	(102.91,140.98) --
	(112.41,140.98) --
	(112.41,146.07) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54,115.55) --
	(102.11,115.55) --
	(102.11,120.64) --
	(103.76,120.64) --
	(103.76,125.72) --
	(106.32,125.72) --
	(106.32,130.81) --
	(107.75,130.81) --
	(107.75,135.90) --
	(109.54,135.90) --
	(109.54,140.98) --
	(111.06,140.98) --
	(111.06,146.07) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (101.54,115.55) --
	(107.55,115.55) --
	(107.55,120.64) --
	(109.94,120.64) --
	(109.94,125.72) --
	(113.83,125.72) --
	(113.83,130.81) --
	(118.89,130.81) --
	(118.89,135.90) --
	(122.60,135.90) --
	(122.60,140.98) --
	(129.83,140.98) --
	(129.83,146.07) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07) --
	(149.79,146.07);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (101.54, 65.97) rectangle (149.79,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] (149.39, 65.97) rectangle (197.63,149.88);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 69.78) --
	(197.63, 69.78);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 88.85) --
	(197.63, 88.85);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39,107.92) --
	(197.63,107.92);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39,127.00) --
	(197.63,127.00);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39,146.07) --
	(197.63,146.07);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 65.97) --
	(149.39,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (161.88, 65.97) --
	(161.88,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (179.75, 65.97) --
	(179.75,149.88);

\path[draw=drawColor,line width= 0.5pt,line join=round] (197.63, 65.97) --
	(197.63,149.88);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39, 69.78) --
	(197.63, 69.78) --
	(197.63, 74.87) --
	(197.63, 74.87) --
	(197.63, 74.87);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39, 74.87) --
	(153.00, 74.87) --
	(153.00, 79.95) --
	(153.99, 79.95) --
	(153.99, 85.04) --
	(155.54, 85.04) --
	(155.54, 90.12) --
	(156.72, 90.12) --
	(156.72, 95.21) --
	(156.95, 95.21) --
	(156.95,100.30) --
	(158.33,100.30) --
	(158.33,105.38) --
	(158.37,105.38) --
	(158.37,110.47) --
	(158.73,110.47) --
	(158.73,115.55) --
	(161.08,115.55) --
	(161.08,120.64) --
	(162.03,120.64) --
	(162.03,125.72) --
	(162.72,125.72) --
	(162.72,130.81) --
	(163.62,130.81) --
	(163.62,135.90) --
	(166.70,135.90) --
	(166.70,140.98) --
	(170.42,140.98) --
	(170.42,146.07) --
	(197.63,146.07) --
	(197.63,146.07);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39,146.07) --
	(197.63,146.07) --
	(197.63,146.07);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39,146.07) --
	(197.63,146.07) --
	(197.63,146.07);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (149.39,146.07) --
	(197.63,146.07) --
	(197.63,146.07);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round,line cap=round] (149.39, 65.97) rectangle (197.63,149.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] ( 53.70, 65.97) --
	(101.94, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 54.18, 63.47) --
	( 54.18, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] ( 78.06, 63.47) --
	( 78.06, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.94, 63.47) --
	(101.94, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 54.18, 55.96) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 78.06, 55.96) {1.05};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (101.54, 65.97) --
	(149.79, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (101.54, 63.47) --
	(101.54, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (122.98, 63.47) --
	(122.98, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.79, 63.47) --
	(149.79, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (101.54, 55.96) {1.1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (122.98, 55.96) {1.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (149.79, 55.96) {2};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (125.66, 44.80) {Solving time relative to best};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{204,121,167}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.29, 23.83) -- ( 68.16, 23.83);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,158,115}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.29, 16.30) -- ( 68.16, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] ( 54.29,  8.77) -- ( 68.16,  8.77);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.39, 23.83) -- (145.27, 23.83);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{86,180,233}

\path[draw=drawColor,line width= 0.9pt,line join=round] (131.39, 16.30) -- (145.27, 16.30);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 74.90, 21.08) {Basic-Dense};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 74.90, 13.54) {Basic-Sparse};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at ( 74.90,  6.01) {Cyclic-Fast};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (152.01, 21.08) {Cyclic-Strong};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.67] at (152.01, 13.54) {NonIncreasing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.2pt,line join=round] (149.39, 65.97) --
	(197.63, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.5pt,line join=round] (149.39, 63.47) --
	(149.39, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (161.88, 63.47) --
	(161.88, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (179.75, 63.47) --
	(179.75, 65.97);

\path[draw=drawColor,line width= 0.5pt,line join=round] (197.63, 63.47) --
	(197.63, 65.97);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,155.38);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (161.88, 55.96) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (179.75, 55.96) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.67] at (197.63, 55.96) {1000};
\end{scope}
\end{tikzpicture}


==> tables/best_weight_tables/best_weight_table_all.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccc}

  \mc{1}{l|}{Graph} & $t_{max}$ & \mc{1}{r|}{$w_{max}$} & $t_{max}$ & \mc{1}{r|}{$w_{max}$} & \mc{1}{r}{$t_{max}$} & \mc{1}{r|}{$w_{max}$} & $t_{max}$ & \mc{1}{r|}{$w_{max}$} & $t_{max}$ & $w_{max}$ \\ 
  \hline  

  \mc{1}{l|}{OSM instances} & \mc{2}{c}{HILS} & \mc{2}{c}{DynWVC1} & \mc{2}{c}{DynWVC2} & \mc{2}{c}{Cyclic-Fast} & \mc{2}{c}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{alabama-AM2} & \mc{1}{r}{0.13} & \mc{1}{r|}{\textbf{174309}} & \mc{1}{r}{0.18} & \mc{1}{r|}{174252} & \mc{1}{r}{0.24} & \mc{1}{r|}{174269} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{174309}} & 0.01 & \mc{1}{r}{\textbf{174309}} \\  

  \mc{1}{l|}{alabama-AM3} & \mc{1}{r}{0.49} & \mc{1}{r|}{\textbf{185744}} & \mc{1}{r}{815.35} & \mc{1}{r|}{185510} & \mc{1}{r}{769.23} & \mc{1}{r|}{185644} & \mc{1}{r}{1.76} & \mc{1}{r|}{\textbf{185744}} & 32.42 & \mc{1}{r}{\textbf{185744}} \\  

  \mc{1}{l|}{district-of-columbia-AM1} & \mc{1}{r}{0.14} & \mc{1}{r|}{\textbf{196475}} & \mc{1}{r}{23.96} & \mc{1}{r|}{\textbf{196475}} & \mc{1}{r}{54.41} & \mc{1}{r|}{\textbf{196475}} & \mc{1}{r}{0.33} & \mc{1}{r|}{\textbf{196475}} & 3.52 & \mc{1}{r}{\textbf{196475}} \\  

  \mc{1}{l|}{district-of-columbia-AM2} & \mc{1}{r}{774.34} & \mc{1}{r|}{\textbf{209132}} & \mc{1}{r}{159.08} & \mc{1}{r|}{208989} & \mc{1}{r}{477.92} & \mc{1}{r|}{208952} & \mc{1}{r}{4.51} & \mc{1}{r|}{\textbf{209132}} & 84.21 & \mc{1}{r}{209131} \\  

  \mc{1}{l|}{district-of-columbia-AM3} & \mc{1}{r}{911.06} & \mc{1}{r|}{\textbf{227567}} & \mc{1}{r}{461.10} & \mc{1}{r|}{224760} & \mc{1}{r}{847.30} & \mc{1}{r|}{223863} & \mc{1}{r}{827.17} & \mc{1}{r|}{142454} & 770.40 & \mc{1}{r}{156967} \\  

  \mc{1}{l|}{florida-AM2} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{230595}} & \mc{1}{r}{0.18} & \mc{1}{r|}{\textbf{230595}} & \mc{1}{r}{0.61} & \mc{1}{r|}{\textbf{230595}} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{230595}} & 0.00 & \mc{1}{r}{\textbf{230595}} \\  

  \mc{1}{l|}{florida-AM3} & \mc{1}{r}{3.15} & \mc{1}{r|}{\textbf{237333}} & \mc{1}{r}{29.98} & \mc{1}{r|}{236992} & \mc{1}{r}{955.26} & \mc{1}{r|}{237065} & \mc{1}{r}{1.57} & \mc{1}{r|}{\textbf{237333}} & 41.04 & \mc{1}{r}{\textbf{237333}} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{222652}} & \mc{1}{r}{1.18} & \mc{1}{r|}{\textbf{222652}} & \mc{1}{r}{1.64} & \mc{1}{r|}{\textbf{222652}} & \mc{1}{r}{0.98} & \mc{1}{r|}{\textbf{222652}} & 12.97 & \mc{1}{r}{\textbf{222652}} \\  

  \mc{1}{l|}{greenland-AM3} & \mc{1}{r}{1.09} & \mc{1}{r|}{\textbf{14011}} & \mc{1}{r}{58.88} & \mc{1}{r|}{14007} & \mc{1}{r}{640.46} & \mc{1}{r|}{14010} & \mc{1}{r}{12.10} & \mc{1}{r|}{\textbf{14011}} & 59.73 & \mc{1}{r}{14007} \\  

  \mc{1}{l|}{hawaii-AM2} & \mc{1}{r}{0.19} & \mc{1}{r|}{\textbf{125284}} & \mc{1}{r}{2.50} & \mc{1}{r|}{125266} & \mc{1}{r}{900.47} & \mc{1}{r|}{125270} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{125284}} & 0.10 & \mc{1}{r}{\textbf{125284}} \\  

  \mc{1}{l|}{hawaii-AM3} & \mc{1}{r}{997.05} & \mc{1}{r|}{\textbf{141034}} & \mc{1}{r}{406.57} & \mc{1}{r|}{140656} & \mc{1}{r}{949.39} & \mc{1}{r|}{140514} & \mc{1}{r}{124.60} & \mc{1}{r|}{116202} & 999.63 & \mc{1}{r}{126851} \\  

  \mc{1}{l|}{idaho-AM3} & \mc{1}{r}{0.82} & \mc{1}{r|}{\textbf{77145}} & \mc{1}{r}{79.67} & \mc{1}{r|}{\textbf{77145}} & \mc{1}{r}{58.83} & \mc{1}{r|}{\textbf{77145}} & \mc{1}{r}{12.77} & \mc{1}{r|}{77086} & 40.71 & \mc{1}{r}{77144} \\  

  \mc{1}{l|}{kansas-AM3} & \mc{1}{r}{1.20} & \mc{1}{r|}{\textbf{87976}} & \mc{1}{r}{403.90} & \mc{1}{r|}{\textbf{87976}} & \mc{1}{r}{276.26} & \mc{1}{r|}{\textbf{87976}} & \mc{1}{r}{2.25} & \mc{1}{r|}{\textbf{87976}} & 110.41 & \mc{1}{r}{\textbf{87976}} \\  

  \mc{1}{l|}{kentucky-AM2} & \mc{1}{r}{0.23} & \mc{1}{r|}{\textbf{97397}} & \mc{1}{r}{3.23} & \mc{1}{r|}{\textbf{97397}} & \mc{1}{r}{9.77} & \mc{1}{r|}{\textbf{97397}} & \mc{1}{r}{0.24} & \mc{1}{r|}{\textbf{97397}} & 0.44 & \mc{1}{r}{\textbf{97397}} \\  

  \mc{1}{l|}{kentucky-AM3} & \mc{1}{r}{778.45} & \mc{1}{r|}{100505} & \mc{1}{r}{951.91} & \mc{1}{r|}{100476} & \mc{1}{r}{96.83} & \mc{1}{r|}{100455} & \mc{1}{r}{412.93} & \mc{1}{r|}{\textbf{100509}} & 808.64 & \mc{1}{r}{100477} \\  

  \mc{1}{l|}{louisiana-AM3} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{60024}} & \mc{1}{r}{8.63} & \mc{1}{r|}{\textbf{60024}} & \mc{1}{r}{0.18} & \mc{1}{r|}{60002} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{60024}} & 0.11 & \mc{1}{r}{\textbf{60024}} \\  

  \mc{1}{l|}{maryland-AM3} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{45496}} & \mc{1}{r}{0.79} & \mc{1}{r|}{\textbf{45496}} & \mc{1}{r}{0.73} & \mc{1}{r|}{\textbf{45496}} & \mc{1}{r}{0.11} & \mc{1}{r|}{\textbf{45496}} & 0.15 & \mc{1}{r}{\textbf{45496}} \\  

  \mc{1}{l|}{massachusetts-AM2} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{140095}} & \mc{1}{r}{0.30} & \mc{1}{r|}{\textbf{140095}} & \mc{1}{r}{0.91} & \mc{1}{r|}{\textbf{140095}} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{140095}} & 0.05 & \mc{1}{r}{\textbf{140095}} \\  

  \mc{1}{l|}{massachusetts-AM3} & \mc{1}{r}{0.67} & \mc{1}{r|}{\textbf{145866}} & \mc{1}{r}{553.21} & \mc{1}{r|}{145844} & \mc{1}{r}{270.28} & \mc{1}{r|}{145862} & \mc{1}{r}{1.39} & \mc{1}{r|}{\textbf{145866}} & 31.04 & \mc{1}{r}{\textbf{145866}} \\  

  \mc{1}{l|}{mexico-AM3} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{97663}} & \mc{1}{r}{3.84} & \mc{1}{r|}{\textbf{97663}} & \mc{1}{r}{275.83} & \mc{1}{r|}{\textbf{97663}} & \mc{1}{r}{0.98} & \mc{1}{r|}{\textbf{97663}} & 21.37 & \mc{1}{r}{\textbf{97663}} \\  

  \mc{1}{l|}{new-hampshire-AM3} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{116060}} & \mc{1}{r}{0.10} & \mc{1}{r|}{116057} & \mc{1}{r}{1.63} & \mc{1}{r|}{\textbf{116060}} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{116060}} & 0.08 & \mc{1}{r}{\textbf{116060}} \\  

  \mc{1}{l|}{north-carolina-AM3} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{49720}} & \mc{1}{r}{3.83} & \mc{1}{r|}{49694} & \mc{1}{r}{114.45} & \mc{1}{r|}{\textbf{49720}} & \mc{1}{r}{0.74} & \mc{1}{r|}{\textbf{49720}} & 45.89 & \mc{1}{r}{\textbf{49720}} \\  

  \mc{1}{l|}{oregon-AM2} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{165047}} & \mc{1}{r}{0.62} & \mc{1}{r|}{\textbf{165047}} & \mc{1}{r}{0.43} & \mc{1}{r|}{\textbf{165047}} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{165047}} & 0.01 & \mc{1}{r}{\textbf{165047}} \\  

  \mc{1}{l|}{oregon-AM3} & \mc{1}{r}{11.50} & \mc{1}{r|}{\textbf{175078}} & \mc{1}{r}{4.82} & \mc{1}{r|}{175042} & \mc{1}{r}{511.10} & \mc{1}{r|}{175067} & \mc{1}{r}{9.80} & \mc{1}{r|}{175074} & 39.78 & \mc{1}{r}{175077} \\  

  \mc{1}{l|}{pennsylvania-AM3} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{143870}} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{143870}} & \mc{1}{r}{0.14} & \mc{1}{r|}{\textbf{143870}} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{143870}} & 0.12 & \mc{1}{r}{\textbf{143870}} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r}{0.22} & \mc{1}{r|}{\textbf{184596}} & \mc{1}{r}{7.75} & \mc{1}{r|}{184537} & \mc{1}{r}{13.90} & \mc{1}{r|}{184576} & \mc{1}{r}{0.41} & \mc{1}{r|}{\textbf{184596}} & 4.37 & \mc{1}{r}{\textbf{184596}} \\  

  \mc{1}{l|}{rhode-island-AM3} & \mc{1}{r}{27.99} & \mc{1}{r|}{\textbf{201758}} & \mc{1}{r}{230.53} & \mc{1}{r|}{201470} & \mc{1}{r}{711.97} & \mc{1}{r|}{201359} & \mc{1}{r}{32.63} & \mc{1}{r|}{167162} & 60.65 & \mc{1}{r}{167162} \\  

  \mc{1}{l|}{utah-AM3} & \mc{1}{r}{0.08} & \mc{1}{r|}{\textbf{98847}} & \mc{1}{r}{143.24} & \mc{1}{r|}{98791} & \mc{1}{r}{7.71} & \mc{1}{r|}{98841} & \mc{1}{r}{0.10} & \mc{1}{r|}{\textbf{98847}} & 0.28 & \mc{1}{r}{\textbf{98847}} \\  

  \mc{1}{l|}{vermont-AM3} & \mc{1}{r}{0.55} & \mc{1}{r|}{63302} & \mc{1}{r}{28.77} & \mc{1}{r|}{63234} & \mc{1}{r}{338.90} & \mc{1}{r|}{63238} & \mc{1}{r}{145.39} & \mc{1}{r|}{\textbf{63312}} & 448.54 & \mc{1}{r}{\textbf{63312}} \\  

  \mc{1}{l|}{virginia-AM2} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{295867}} & \mc{1}{r}{15.96} & \mc{1}{r|}{295643} & \mc{1}{r}{20.50} & \mc{1}{r|}{295638} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{295867}} & 0.02 & \mc{1}{r}{\textbf{295867}} \\  

  \mc{1}{l|}{virginia-AM3} & \mc{1}{r}{2.25} & \mc{1}{r|}{\textbf{308305}} & \mc{1}{r}{971.96} & \mc{1}{r|}{307744} & \mc{1}{r}{809.24} & \mc{1}{r|}{307907} & \mc{1}{r}{34.42} & \mc{1}{r|}{\textbf{308305}} & 200.13 & \mc{1}{r}{\textbf{308305}} \\  

  \mc{1}{l|}{washington-AM2} & \mc{1}{r}{0.32} & \mc{1}{r|}{\textbf{305619}} & \mc{1}{r}{19.08} & \mc{1}{r|}{\textbf{305619}} & \mc{1}{r}{14.39} & \mc{1}{r|}{\textbf{305619}} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{305619}} & 0.07 & \mc{1}{r}{\textbf{305619}} \\  

  \mc{1}{l|}{washington-AM3} & \mc{1}{r}{205.97} & \mc{1}{r|}{\textbf{314288}} & \mc{1}{r}{37.94} & \mc{1}{r|}{313689} & \mc{1}{r}{383.62} & \mc{1}{r|}{313844} & \mc{1}{r}{3.60} & \mc{1}{r|}{284684} & 73.00 & \mc{1}{r}{288116} \\  

  \mc{1}{l|}{west-virginia-AM3} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{47927}} & \mc{1}{r}{2.75} & \mc{1}{r|}{\textbf{47927}} & \mc{1}{r}{2.84} & \mc{1}{r|}{\textbf{47927}} & \mc{1}{r}{2.90} & \mc{1}{r|}{\textbf{47927}} & 41.73 & \mc{1}{r}{\textbf{47927}} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{61.8\% (21/34)} & \mc{2}{c}{64.7\% (22/34)} \\  

  \mc{1}{l|}{Optimal weight} & \mc{2}{r}{100.0\% (22/22)} & \mc{2}{r}{59.1\% (13/22)} & \mc{2}{r}{63.6\% (14/22)} & \mc{2}{r}{} & \mc{2}{c}{} \\ 
  \hline \hline  

  \mc{1}{l|}{SNAP instances} & \mc{2}{c|}{HILS} & \mc{2}{c|}{DynWVC1} & \mc{2}{c|}{DynWVC2} & \mc{2}{c|}{Cyclic-Fast} & \mc{2}{c|}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{as-skitter} & \mc{1}{r}{999.38} & \mc{1}{r|}{122709575} & \mc{1}{r}{872.03} & \mc{1}{r|}{123610385} & \mc{1}{r}{383.97} & \mc{1}{r|}{123273938} & \mc{1}{r}{346.69} & \mc{1}{r|}{124137148} & 354.71 & \mc{1}{r}{\textbf{124137365}} \\  

  \mc{1}{l|}{ca-AstroPh} & \mc{1}{r}{9.47} & \mc{1}{r|}{\textbf{797510}} & \mc{1}{r}{32.46} & \mc{1}{r|}{797475} & \mc{1}{r}{39.35} & \mc{1}{r|}{797470} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{797510}} & 0.02 & \mc{1}{r}{\textbf{797510}} \\  

  \mc{1}{l|}{ca-CondMat} & \mc{1}{r}{41.58} & \mc{1}{r|}{\textbf{1147950}} & \mc{1}{r}{43.50} & \mc{1}{r|}{1147809} & \mc{1}{r}{27.75} & \mc{1}{r|}{1147845} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{1147950}} & 0.01 & \mc{1}{r}{\textbf{1147950}} \\  

  \mc{1}{l|}{ca-GrQc} & \mc{1}{r}{0.32} & \mc{1}{r|}{\textbf{286489}} & \mc{1}{r}{23.64} & \mc{1}{r|}{\textbf{286489}} & \mc{1}{r}{1.93} & \mc{1}{r|}{\textbf{286489}} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{286489}} & 0.00 & \mc{1}{r}{\textbf{286489}} \\  

  \mc{1}{l|}{ca-HepPh} & \mc{1}{r}{6.39} & \mc{1}{r|}{\textbf{581039}} & \mc{1}{r}{13.21} & \mc{1}{r|}{581014} & \mc{1}{r}{17.34} & \mc{1}{r|}{581028} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{581039}} & 0.01 & \mc{1}{r}{\textbf{581039}} \\  

  \mc{1}{l|}{ca-HepTh} & \mc{1}{r}{4.73} & \mc{1}{r|}{\textbf{562004}} & \mc{1}{r}{6.57} & \mc{1}{r|}{561982} & \mc{1}{r}{5.30} & \mc{1}{r|}{561974} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{562004}} & 0.00 & \mc{1}{r}{\textbf{562004}} \\  

  \mc{1}{l|}{email-Enron} & \mc{1}{r}{125.69} & \mc{1}{r|}{2464922} & \mc{1}{r}{794.33} & \mc{1}{r|}{2464887} & \mc{1}{r}{594.93} & \mc{1}{r|}{2464890} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{2464935}} & 0.03 & \mc{1}{r}{\textbf{2464935}} \\  

  \mc{1}{l|}{email-EuAll} & \mc{1}{r}{316.38} & \mc{1}{r|}{\textbf{25286322}} & \mc{1}{r}{136.11} & \mc{1}{r|}{\textbf{25286322}} & \mc{1}{r}{132.62} & \mc{1}{r|}{\textbf{25286322}} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{25286322}} & 0.07 & \mc{1}{r}{\textbf{25286322}} \\  

  \mc{1}{l|}{p2p-Gnutella04} & \mc{1}{r}{130.98} & \mc{1}{r|}{\textbf{679111}} & \mc{1}{r}{1.46} & \mc{1}{r|}{679105} & \mc{1}{r}{1.57} & \mc{1}{r|}{679105} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{679111}} & 0.01 & \mc{1}{r}{\textbf{679111}} \\  

  \mc{1}{l|}{p2p-Gnutella05} & \mc{1}{r}{132.20} & \mc{1}{r|}{\textbf{554943}} & \mc{1}{r}{2.05} & \mc{1}{r|}{554923} & \mc{1}{r}{3.55} & \mc{1}{r|}{554931} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{554943}} & 0.01 & \mc{1}{r}{\textbf{554943}} \\  

  \mc{1}{l|}{p2p-Gnutella06} & \mc{1}{r}{1.39} & \mc{1}{r|}{\textbf{548612}} & \mc{1}{r}{525.35} & \mc{1}{r|}{548611} & \mc{1}{r}{186.97} & \mc{1}{r|}{548611} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{548612}} & 0.01 & \mc{1}{r}{\textbf{548612}} \\  

  \mc{1}{l|}{p2p-Gnutella08} & \mc{1}{r}{0.14} & \mc{1}{r|}{\textbf{434577}} & \mc{1}{r}{0.29} & \mc{1}{r|}{434575} & \mc{1}{r}{0.18} & \mc{1}{r|}{\textbf{434577}} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{434577}} & 0.00 & \mc{1}{r}{\textbf{434577}} \\  

  \mc{1}{l|}{p2p-Gnutella09} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{568439}} & \mc{1}{r}{0.51} & \mc{1}{r|}{\textbf{568439}} & \mc{1}{r}{0.45} & \mc{1}{r|}{\textbf{568439}} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{568439}} & 0.00 & \mc{1}{r}{\textbf{568439}} \\  

  \mc{1}{l|}{p2p-Gnutella24} & \mc{1}{r}{3.50} & \mc{1}{r|}{\textbf{1984567}} & \mc{1}{r}{21.87} & \mc{1}{r|}{\textbf{1984567}} & \mc{1}{r}{5.51} & \mc{1}{r|}{\textbf{1984567}} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{1984567}} & 0.01 & \mc{1}{r}{\textbf{1984567}} \\  

  \mc{1}{l|}{p2p-Gnutella25} & \mc{1}{r}{1.19} & \mc{1}{r|}{\textbf{1701967}} & \mc{1}{r}{2.66} & \mc{1}{r|}{\textbf{1701967}} & \mc{1}{r}{2.20} & \mc{1}{r|}{\textbf{1701967}} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{1701967}} & 0.01 & \mc{1}{r}{\textbf{1701967}} \\  

  \mc{1}{l|}{p2p-Gnutella30} & \mc{1}{r}{8.29} & \mc{1}{r|}{\textbf{2787907}} & \mc{1}{r}{7.33} & \mc{1}{r|}{2787901} & \mc{1}{r}{10.23} & \mc{1}{r|}{2787896} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{2787907}} & 0.01 & \mc{1}{r}{\textbf{2787907}} \\  

  \mc{1}{l|}{p2p-Gnutella31} & \mc{1}{r}{114.57} & \mc{1}{r|}{\textbf{4776986}} & \mc{1}{r}{70.88} & \mc{1}{r|}{4776960} & \mc{1}{r}{47.97} & \mc{1}{r|}{4776961} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{4776986}} & 0.03 & \mc{1}{r}{\textbf{4776986}} \\  

  \mc{1}{l|}{roadNet-CA} & \mc{1}{r}{1239.45} & \mc{1}{r|}{107549493} & \mc{1}{r}{1000.92} & \mc{1}{r|}{109587056} & \mc{1}{r}{999.94} & \mc{1}{r|}{109571608} & \mc{1}{r}{1.94} & \mc{1}{r|}{\textbf{111360828}} & 1.86 & \mc{1}{r}{\textbf{111360828}} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{1000.10} & \mc{1}{r|}{60043107} & \mc{1}{r}{476.71} & \mc{1}{r|}{60986458} & \mc{1}{r}{504.85} & \mc{1}{r|}{60986458} & \mc{1}{r}{0.96} & \mc{1}{r|}{\textbf{61731589}} & 1.07 & \mc{1}{r}{\textbf{61731589}} \\  

  \mc{1}{l|}{roadNet-TX} & \mc{1}{r}{999.87} & \mc{1}{r|}{76340946} & \mc{1}{r}{789.43} & \mc{1}{r|}{77672388} & \mc{1}{r}{694.33} & \mc{1}{r|}{77672388} & \mc{1}{r}{1.34} & \mc{1}{r|}{\textbf{78599946}} & 1.32 & \mc{1}{r}{\textbf{78599946}} \\  

  \mc{1}{l|}{soc-Epinions1} & \mc{1}{r}{237.04} & \mc{1}{r|}{5690874} & \mc{1}{r}{290.84} & \mc{1}{r|}{5690651} & \mc{1}{r}{125.02} & \mc{1}{r|}{5690772} & \mc{1}{r}{0.08} & \mc{1}{r|}{\textbf{5690970}} & 0.08 & \mc{1}{r}{\textbf{5690970}} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r}{1222.69} & \mc{1}{r|}{257654493} & \mc{1}{r}{1000.30} & \mc{1}{r|}{279146154} & \mc{1}{r}{1002.32} & \mc{1}{r|}{279193147} & \mc{1}{r}{44.69} & \mc{1}{r|}{284036216} & 44.57 & \mc{1}{r}{\textbf{284036239}} \\  

  \mc{1}{l|}{soc-Slashdot0811} & \mc{1}{r}{329.62} & \mc{1}{r|}{5660760} & \mc{1}{r}{238.18} & \mc{1}{r|}{5660385} & \mc{1}{r}{880.68} & \mc{1}{r|}{5660555} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{5660899}} & 0.08 & \mc{1}{r}{\textbf{5660899}} \\  

  \mc{1}{l|}{soc-Slashdot0902} & \mc{1}{r}{594.66} & \mc{1}{r|}{5971664} & \mc{1}{r}{270.85} & \mc{1}{r|}{5971308} & \mc{1}{r}{435.90} & \mc{1}{r|}{5971476} & \mc{1}{r}{0.11} & \mc{1}{r|}{\textbf{5971849}} & 0.11 & \mc{1}{r}{\textbf{5971849}} \\  

  \mc{1}{l|}{soc-pokec-relationships} & \mc{1}{r}{1236.28} & \mc{1}{r|}{82159438} & \mc{1}{r}{1000.83} & \mc{1}{r|}{\textbf{83156762}} & \mc{1}{r}{999.13} & \mc{1}{r|}{83155217} & \mc{1}{r}{1165.87} & \mc{1}{r|}{81478217} & 0.00 & \mc{1}{r}{0} \\  

  \mc{1}{l|}{web-BerkStan} & \mc{1}{r}{999.98} & \mc{1}{r|}{43443040} & \mc{1}{r}{144.59} & \mc{1}{r|}{43640083} & \mc{1}{r}{161.66} & \mc{1}{r|}{43634623} & \mc{1}{r}{6.74} & \mc{1}{r|}{\textbf{43907482}} & 8.05 & \mc{1}{r}{\textbf{43907482}} \\  

  \mc{1}{l|}{web-Google} & \mc{1}{r}{999.32} & \mc{1}{r|}{56009070} & \mc{1}{r}{353.69} & \mc{1}{r|}{56208118} & \mc{1}{r}{324.65} & \mc{1}{r|}{56206250} & \mc{1}{r}{1.72} & \mc{1}{r|}{\textbf{56326504}} & 6.44 & \mc{1}{r}{\textbf{56326504}} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{997.37} & \mc{1}{r|}{26004376} & \mc{1}{r}{967.49} & \mc{1}{r|}{26008674} & \mc{1}{r}{968.85} & \mc{1}{r|}{26008856} & \mc{1}{r}{1.60} & \mc{1}{r|}{\textbf{26016941}} & 2.74 & \mc{1}{r}{\textbf{26016941}} \\  

  \mc{1}{l|}{web-Stanford} & \mc{1}{r}{999.55} & \mc{1}{r|}{17716140} & \mc{1}{r}{741.76} & \mc{1}{r|}{17745660} & \mc{1}{r}{671.32} & \mc{1}{r|}{17741043} & \mc{1}{r}{1.74} & \mc{1}{r|}{\textbf{17792930}} & 1.96 & \mc{1}{r}{\textbf{17792930}} \\  

  \mc{1}{l|}{wiki-Talk} & \mc{1}{r}{999.66} & \mc{1}{r|}{235817024} & \mc{1}{r}{964.25} & \mc{1}{r|}{235836778} & \mc{1}{r}{995.65} & \mc{1}{r|}{235836758} & \mc{1}{r}{1.29} & \mc{1}{r|}{\textbf{235837346}} & 1.29 & \mc{1}{r}{\textbf{235837346}} \\  

  \mc{1}{l|}{wiki-Vote} & \mc{1}{r}{21.47} & \mc{1}{r|}{\textbf{500079}} & \mc{1}{r}{15.07} & \mc{1}{r|}{500071} & \mc{1}{r}{0.63} & \mc{1}{r|}{\textbf{500079}} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{500079}} & 0.02 & \mc{1}{r}{\textbf{500079}} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{90.3\% (28/31)} & \mc{2}{c}{90.3\% (28/31)} \\  

  \mc{1}{l|}{Optimal weight} & \mc{2}{r}{57.1\% (16/28)} & \mc{2}{r}{17.9\% (5/28)} & \mc{2}{r}{25.0\% (7/28)} & \mc{2}{r}{} & \mc{2}{c}{} \\ 
  \hline \hline  

  \mc{1}{l|}{mesh instances} & \mc{2}{c|}{HILS} & \mc{2}{c|}{DynWVC1} & \mc{2}{c|}{DynWVC2} & \mc{2}{c|}{Cyclic-Fast} & \mc{2}{c|}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{beethoven} & \mc{1}{r}{481.59} & \mc{1}{r|}{238746} & \mc{1}{r}{7.94} & \mc{1}{r|}{238711} & \mc{1}{r}{8.16} & \mc{1}{r|}{238711} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{238794}} & 0.01 & \mc{1}{r}{\textbf{238794}} \\  

  \mc{1}{l|}{blob} & \mc{1}{r}{350.43} & \mc{1}{r|}{855004} & \mc{1}{r}{39.91} & \mc{1}{r|}{854843} & \mc{1}{r}{40.00} & \mc{1}{r|}{854843} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{855547}} & 0.02 & \mc{1}{r}{\textbf{855547}} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r}{1000.10} & \mc{1}{r|}{55504671} & \mc{1}{r}{879.42} & \mc{1}{r|}{56757052} & \mc{1}{r}{797.35} & \mc{1}{r|}{56757052} & \mc{1}{r}{1.75} & \mc{1}{r|}{\textbf{57555880}} & 1.84 & \mc{1}{r}{\textbf{57555880}} \\  

  \mc{1}{l|}{bunny} & \mc{1}{r}{986.80} & \mc{1}{r|}{3680516} & \mc{1}{r}{826.84} & \mc{1}{r|}{3682827} & \mc{1}{r}{831.80} & \mc{1}{r|}{3682827} & \mc{1}{r}{0.13} & \mc{1}{r|}{\textbf{3686960}} & 0.13 & \mc{1}{r}{\textbf{3686960}} \\  

  \mc{1}{l|}{cow} & \mc{1}{r}{34.53} & \mc{1}{r|}{269453} & \mc{1}{r}{582.61} & \mc{1}{r|}{269319} & \mc{1}{r}{583.91} & \mc{1}{r|}{269319} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{269543}} & 0.01 & \mc{1}{r}{\textbf{269543}} \\  

  \mc{1}{l|}{dragon} & \mc{1}{r}{998.93} & \mc{1}{r|}{7940963} & \mc{1}{r}{970.34} & \mc{1}{r|}{7943911} & \mc{1}{r}{981.51} & \mc{1}{r|}{7944042} & \mc{1}{r}{0.21} & \mc{1}{r|}{\textbf{7956530}} & 0.22 & \mc{1}{r}{\textbf{7956530}} \\  

  \mc{1}{l|}{dragonsub} & \mc{1}{r}{999.92} & \mc{1}{r|}{31331138} & \mc{1}{r}{271.66} & \mc{1}{r|}{31756333} & \mc{1}{r}{275.00} & \mc{1}{r|}{31756333} & \mc{1}{r}{1.10} & \mc{1}{r|}{\textbf{32213898}} & 1.11 & \mc{1}{r}{\textbf{32213898}} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r}{1000.01} & \mc{1}{r|}{35542918} & \mc{1}{r}{506.04} & \mc{1}{r|}{36124409} & \mc{1}{r}{457.18} & \mc{1}{r|}{36124409} & \mc{1}{r}{2.19} & \mc{1}{r|}{\textbf{36650298}} & 2.40 & \mc{1}{r}{\textbf{36650298}} \\  

  \mc{1}{l|}{face} & \mc{1}{r}{215.07} & \mc{1}{r|}{1218565} & \mc{1}{r}{267.71} & \mc{1}{r|}{1218395} & \mc{1}{r}{268.13} & \mc{1}{r|}{1218395} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{1219418}} & 0.03 & \mc{1}{r}{\textbf{1219418}} \\  

  \mc{1}{l|}{fandisk} & \mc{1}{r}{307.45} & \mc{1}{r|}{463046} & \mc{1}{r}{3.09} & \mc{1}{r|}{462871} & \mc{1}{r}{2.91} & \mc{1}{r|}{462871} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{463288}} & 0.01 & \mc{1}{r}{\textbf{463288}} \\  

  \mc{1}{l|}{feline} & \mc{1}{r}{919.67} & \mc{1}{r|}{2204661} & \mc{1}{r}{730.80} & \mc{1}{r|}{2204925} & \mc{1}{r}{734.34} & \mc{1}{r|}{2204925} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{2207219}} & 0.09 & \mc{1}{r}{\textbf{2207219}} \\  

  \mc{1}{l|}{gameguy} & \mc{1}{r}{940.54} & \mc{1}{r|}{2322904} & \mc{1}{r}{930.38} & \mc{1}{r|}{2323663} & \mc{1}{r}{928.76} & \mc{1}{r|}{2323663} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{2325878}} & 0.05 & \mc{1}{r}{\textbf{2325878}} \\  

  \mc{1}{l|}{gargoyle} & \mc{1}{r}{698.13} & \mc{1}{r|}{1058569} & \mc{1}{r}{22.78} & \mc{1}{r|}{1058452} & \mc{1}{r}{22.93} & \mc{1}{r|}{1058452} & \mc{1}{r}{0.04} & \mc{1}{r|}{\textbf{1059559}} & 0.03 & \mc{1}{r}{\textbf{1059559}} \\  

  \mc{1}{l|}{turtle} & \mc{1}{r}{999.90} & \mc{1}{r|}{14166152} & \mc{1}{r}{994.87} & \mc{1}{r|}{14212920} & \mc{1}{r}{976.57} & \mc{1}{r|}{14213516} & \mc{1}{r}{0.42} & \mc{1}{r|}{\textbf{14263005}} & 0.43 & \mc{1}{r}{\textbf{14263005}} \\  

  \mc{1}{l|}{venus} & \mc{1}{r}{413.22} & \mc{1}{r|}{305717} & \mc{1}{r}{559.29} & \mc{1}{r|}{305571} & \mc{1}{r}{556.38} & \mc{1}{r|}{305571} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{305749}} & 0.01 & \mc{1}{r}{\textbf{305749}} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{100.0\% (15/15)} & \mc{2}{c}{100.0\% (15/15)} \\  

  \mc{1}{l|}{Optimal weight} & \mc{2}{r}{0.0\% (0/15)} & \mc{2}{r}{0.0\% (0/15)} & \mc{2}{r}{0.0\% (0/15)} & \mc{2}{r}{} & \mc{2}{c}{} \\ 
  \hline \hline  

  \mc{1}{l|}{FE instances} & \mc{2}{c|}{HILS} & \mc{2}{c|}{DynWVC1} & \mc{2}{c|}{DynWVC2} & \mc{2}{c|}{Cyclic-Fast} & \mc{2}{c|}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{fe\_4elt2} & \mc{1}{r}{771.08} & \mc{1}{r|}{427646} & \mc{1}{r}{910.91} & \mc{1}{r|}{427738} & \mc{1}{r}{906.41} & \mc{1}{r|}{427738} & \mc{1}{r}{0.15} & \mc{1}{r|}{\textbf{428029}} & 0.10 & \mc{1}{r}{\textbf{428029}} \\  

  \mc{1}{l|}{fe\_body} & \mc{1}{r}{610.15} & \mc{1}{r|}{1678532} & \mc{1}{r}{695.46} & \mc{1}{r|}{1678516} & \mc{1}{r}{499.03} & \mc{1}{r|}{1678496} & \mc{1}{r}{0.44} & \mc{1}{r|}{\textbf{1680182}} & 0.83 & \mc{1}{r}{1680117} \\  

  \mc{1}{l|}{fe\_ocean} & \mc{1}{r}{999.60} & \mc{1}{r|}{7077084} & \mc{1}{r}{998.97} & \mc{1}{r|}{\textbf{7220778}} & \mc{1}{r}{379.75} & \mc{1}{r|}{7220128} & \mc{1}{r}{17.55} & \mc{1}{r|}{6594720} & 17.95 & \mc{1}{r}{6598331} \\  

  \mc{1}{l|}{fe\_pwt} & \mc{1}{r}{957.25} & \mc{1}{r|}{1175754} & \mc{1}{r}{814.23} & \mc{1}{r|}{1176721} & \mc{1}{r}{320.05} & \mc{1}{r|}{1176784} & \mc{1}{r}{2.64} & \mc{1}{r|}{1160410} & 5.37 & \mc{1}{r}{\textbf{888959}} \\  

  \mc{1}{l|}{fe\_rotor} & \mc{1}{r}{995.75} & \mc{1}{r|}{2650209} & \mc{1}{r}{961.76} & \mc{1}{r|}{\textbf{2659653}} & \mc{1}{r}{975.98} & \mc{1}{r|}{2658966} & \mc{1}{r}{10.16} & \mc{1}{r|}{2531152} & 16.72 & \mc{1}{r}{2538117} \\  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{846.51} & \mc{1}{r|}{616528} & \mc{1}{r}{442.29} & \mc{1}{r|}{616939} & \mc{1}{r}{441.87} & \mc{1}{r|}{616939} & \mc{1}{r}{0.59} & \mc{1}{r|}{\textbf{617816}} & 0.63 & \mc{1}{r}{\textbf{617816}} \\  

  \mc{1}{l|}{fe\_tooth} & \mc{1}{r}{824.07} & \mc{1}{r|}{3032819} & \mc{1}{r}{353.21} & \mc{1}{r|}{3031269} & \mc{1}{r}{991.48} & \mc{1}{r|}{3031355} & \mc{1}{r}{0.26} & \mc{1}{r|}{\textbf{3033298}} & 0.26 & \mc{1}{r}{\textbf{3033298}} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{} & \mc{2}{r}{42.9\% (3/7)} & \mc{2}{c}{42.9\% (3/7)} \\  

  \mc{1}{l|}{Optimal weight} & \mc{2}{r}{0.0\% (0/3)} & \mc{2}{r}{0.0\% (0/3)} & \mc{2}{r}{0.0\% (0/3)} & \mc{2}{r}{} & \mc{2}{c}{} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/best_weight_tables/fe.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccccccccc}

  \mc{1}{l}{Graph} & \mc{2}{|c}{DynWVC1} & \mc{2}{|c}{DynWVC2} & \mc{2}{|c}{HILS} & \mc{2}{|c}{Cyclic-Fast} & \mc{2}{|c}{Cyclic-Strong} & \mc{2}{|c}{Non-Increasing} & \mc{2}{|c}{Basic-Sparse} & \mc{2}{|c}{Basic-Dense} \\ 
  \hline  

   & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} \\ 
  \hline  

  \mc{1}{l}{\cellcolor{lightgray!50}{fe\_4elt2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{961.12}} & \mc{1}{r}{\cellcolor{lightgray!50}{427755}} & \mc{1}{|r}{\cellcolor{lightgray!50}{974.87}} & \mc{1}{r}{\cellcolor{lightgray!50}{427755}} & \mc{1}{|r}{\cellcolor{lightgray!50}{759.23}} & \mc{1}{r}{\cellcolor{lightgray!50}{427646}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{428029}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{428029}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.18}} & \mc{1}{r}{\cellcolor{lightgray!50}{428016}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.66}} & \mc{1}{r}{\cellcolor{lightgray!50}{420477}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.24}} & \mc{1}{r}{\cellcolor{lightgray!50}{421235}} \\  

  \mc{1}{l}{fe\_body} & \mc{1}{|r}{504.31} & \mc{1}{r}{1678616} & \mc{1}{|r}{499.03} & \mc{1}{r}{1678496} & \mc{1}{|r}{806.46} & \mc{1}{r}{1678708} & \mc{1}{|r}{0.51} & \mc{1}{r}{\textbf{1680182}} & \mc{1}{|r}{0.86} & \mc{1}{r}{1680117} & \mc{1}{|r}{0.27} & \mc{1}{r}{1680133} & \mc{1}{|r}{858.22} & \mc{1}{r}{1194619} & \mc{1}{|r}{26.78} & \mc{1}{r}{1127790} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{fe\_ocean}} & \mc{1}{|r}{\cellcolor{lightgray!50}{983.53}} & \mc{1}{r}{\cellcolor{lightgray!50}{7222521}} & \mc{1}{|r}{\cellcolor{lightgray!50}{379.75}} & \mc{1}{r}{\cellcolor{lightgray!50}{7220128}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.57}} & \mc{1}{r}{\cellcolor{lightgray!50}{7069279}} & \mc{1}{|r}{\cellcolor{lightgray!50}{18.85}} & \mc{1}{r}{\cellcolor{lightgray!50}{6591832}} & \mc{1}{|r}{\cellcolor{lightgray!50}{19.04}} & \mc{1}{r}{\cellcolor{lightgray!50}{6591537}} & \mc{1}{|r}{\cellcolor{lightgray!50}{18.85}} & \mc{1}{r}{\cellcolor{lightgray!50}{6597698}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.91}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{7248581}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.35}} & \mc{1}{r}{\cellcolor{lightgray!50}{6604880}} \\  

  \mc{1}{l}{fe\_pwt} & \mc{1}{|r}{814.23} & \mc{1}{r}{1176721} & \mc{1}{|r}{320.05} & \mc{1}{r}{\textbf{1176784}} & \mc{1}{|r}{932.43} & \mc{1}{r}{1175754} & \mc{1}{|r}{3.03} & \mc{1}{r}{1162232} & \mc{1}{|r}{5.45} & \mc{1}{r}{888959} & \mc{1}{|r}{1.57} & \mc{1}{r}{1151777} & \mc{1}{|r}{3.02} & \mc{1}{r}{1132622} & \mc{1}{|r}{0.79} & \mc{1}{r}{1132622} \\  

  \mc{1}{l}{fe\_rotor} & \mc{1}{|r}{961.76} & \mc{1}{r}{\textbf{2659653}} & \mc{1}{|r}{874.68} & \mc{1}{r}{2659473} & \mc{1}{|r}{973.92} & \mc{1}{r}{2650132} & \mc{1}{|r}{13.95} & \mc{1}{r}{2531152} & \mc{1}{|r}{20.55} & \mc{1}{r}{2538117} & \mc{1}{|r}{13.56} & \mc{1}{r}{2532168} & \mc{1}{|r}{20.76} & \mc{1}{r}{2496992} & \mc{1}{|r}{10.12} & \mc{1}{r}{2496992} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{fe\_sphere}} & \mc{1}{|r}{\cellcolor{lightgray!50}{875.87}} & \mc{1}{r}{\cellcolor{lightgray!50}{616978}} & \mc{1}{|r}{\cellcolor{lightgray!50}{872.36}} & \mc{1}{r}{\cellcolor{lightgray!50}{616978}} & \mc{1}{|r}{\cellcolor{lightgray!50}{843.67}} & \mc{1}{r}{\cellcolor{lightgray!50}{616528}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.63}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{617816}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.67}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{617816}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.46}} & \mc{1}{r}{\cellcolor{lightgray!50}{617585}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.10}} & \mc{1}{r}{\cellcolor{lightgray!50}{600936}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.45}} & \mc{1}{r}{\cellcolor{lightgray!50}{600164}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{fe\_tooth}} & \mc{1}{|r}{\cellcolor{lightgray!50}{353.21}} & \mc{1}{r}{\cellcolor{lightgray!50}{3031269}} & \mc{1}{|r}{\cellcolor{lightgray!50}{619.96}} & \mc{1}{r}{\cellcolor{lightgray!50}{3031385}} & \mc{1}{|r}{\cellcolor{lightgray!50}{994.97}} & \mc{1}{r}{\cellcolor{lightgray!50}{3032819}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.26}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3033298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.26}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3033298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.27}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3033298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{13.02}} & \mc{1}{r}{\cellcolor{lightgray!50}{2694792}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.55}} & \mc{1}{r}{\cellcolor{lightgray!50}{2677851}} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/best_weight_tables/mesh.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccccccccc}

  \mc{1}{l}{Graph} & \mc{2}{|c}{DynWVC1} & \mc{2}{|c}{DynWVC2} & \mc{2}{|c}{HILS} & \mc{2}{|c}{Cyclic-Fast} & \mc{2}{|c}{Cyclic-Strong} & \mc{2}{|c}{Non-Increasing} & \mc{2}{|c}{Basic-Sparse} & \mc{2}{|c}{Basic-Dense} \\ 
  \hline  

   & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} \\ 
  \hline  

  \mc{1}{l}{\cellcolor{lightgray!50}{beethoven}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.86}} & \mc{1}{r}{\cellcolor{lightgray!50}{238726}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.79}} & \mc{1}{r}{\cellcolor{lightgray!50}{238726}} & \mc{1}{|r}{\cellcolor{lightgray!50}{462.31}} & \mc{1}{r}{\cellcolor{lightgray!50}{238746}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{238794}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{238794}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{238794}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{238794}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{5.37}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{238794}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{blob}} & \mc{1}{|r}{\cellcolor{lightgray!50}{39.91}} & \mc{1}{r}{\cellcolor{lightgray!50}{854843}} & \mc{1}{|r}{\cellcolor{lightgray!50}{40.00}} & \mc{1}{r}{\cellcolor{lightgray!50}{854843}} & \mc{1}{|r}{\cellcolor{lightgray!50}{351.91}} & \mc{1}{r}{\cellcolor{lightgray!50}{855004}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{855547}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{855547}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{855547}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.19}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{855547}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.14}} & \mc{1}{r}{\cellcolor{lightgray!50}{616613}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{buddha}} & \mc{1}{|r}{\cellcolor{lightgray!50}{879.42}} & \mc{1}{r}{\cellcolor{lightgray!50}{56757052}} & \mc{1}{|r}{\cellcolor{lightgray!50}{797.35}} & \mc{1}{r}{\cellcolor{lightgray!50}{56757052}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.94}} & \mc{1}{r}{\cellcolor{lightgray!50}{55490134}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.75}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{57555880}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.77}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{57555880}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.24}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{57555880}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{60.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{57555880}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{742.47}} & \mc{1}{r}{\cellcolor{lightgray!50}{41423703}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{bunny}} & \mc{1}{|r}{\cellcolor{lightgray!50}{702.13}} & \mc{1}{r}{\cellcolor{lightgray!50}{3683000}} & \mc{1}{|r}{\cellcolor{lightgray!50}{695.55}} & \mc{1}{r}{\cellcolor{lightgray!50}{3683000}} & \mc{1}{|r}{\cellcolor{lightgray!50}{964.60}} & \mc{1}{r}{\cellcolor{lightgray!50}{3681696}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3686960}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.13}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3686960}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3686960}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.57}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{3686960}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{44.84}} & \mc{1}{r}{\cellcolor{lightgray!50}{3652620}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{cow}} & \mc{1}{|r}{\cellcolor{lightgray!50}{62.04}} & \mc{1}{r}{\cellcolor{lightgray!50}{269340}} & \mc{1}{|r}{\cellcolor{lightgray!50}{61.40}} & \mc{1}{r}{\cellcolor{lightgray!50}{269340}} & \mc{1}{|r}{\cellcolor{lightgray!50}{935.58}} & \mc{1}{r}{\cellcolor{lightgray!50}{269464}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{269543}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{269543}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{269543}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.06}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{269543}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.22}} & \mc{1}{r}{\cellcolor{lightgray!50}{269206}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{dragon}} & \mc{1}{|r}{\cellcolor{lightgray!50}{970.34}} & \mc{1}{r}{\cellcolor{lightgray!50}{7943911}} & \mc{1}{|r}{\cellcolor{lightgray!50}{981.51}} & \mc{1}{r}{\cellcolor{lightgray!50}{7944042}} & \mc{1}{|r}{\cellcolor{lightgray!50}{996.01}} & \mc{1}{r}{\cellcolor{lightgray!50}{7940422}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.21}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{7956530}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.22}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{7956530}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.22}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{7956530}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.82}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{7956530}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{926.01}} & \mc{1}{r}{\cellcolor{lightgray!50}{5951672}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{dragonsub}} & \mc{1}{|r}{\cellcolor{lightgray!50}{323.07}} & \mc{1}{r}{\cellcolor{lightgray!50}{31762035}} & \mc{1}{|r}{\cellcolor{lightgray!50}{379.11}} & \mc{1}{r}{\cellcolor{lightgray!50}{31762035}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.54}} & \mc{1}{r}{\cellcolor{lightgray!50}{31304363}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.10}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{32213898}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{32213898}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.88}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{32213898}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{5.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{32213898}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{936.72}} & \mc{1}{r}{\cellcolor{lightgray!50}{22327211}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{ecat}} & \mc{1}{|r}{\cellcolor{lightgray!50}{565.03}} & \mc{1}{r}{\cellcolor{lightgray!50}{36129804}} & \mc{1}{|r}{\cellcolor{lightgray!50}{542.87}} & \mc{1}{r}{\cellcolor{lightgray!50}{36129804}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.91}} & \mc{1}{r}{\cellcolor{lightgray!50}{35512644}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.19}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{36650298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{36650298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.44}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{36650298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{12.26}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{36650298}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{899.38}} & \mc{1}{r}{\cellcolor{lightgray!50}{25773421}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{face}} & \mc{1}{|r}{\cellcolor{lightgray!50}{87.05}} & \mc{1}{r}{\cellcolor{lightgray!50}{1218510}} & \mc{1}{|r}{\cellcolor{lightgray!50}{86.38}} & \mc{1}{r}{\cellcolor{lightgray!50}{1218510}} & \mc{1}{|r}{\cellcolor{lightgray!50}{228.77}} & \mc{1}{r}{\cellcolor{lightgray!50}{1218565}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1219418}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1219418}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1219418}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.21}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1219418}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{22.99}} & \mc{1}{r}{\cellcolor{lightgray!50}{943327}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{fandisk}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.26}} & \mc{1}{r}{\cellcolor{lightgray!50}{462950}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.42}} & \mc{1}{r}{\cellcolor{lightgray!50}{462950}} & \mc{1}{|r}{\cellcolor{lightgray!50}{232.96}} & \mc{1}{r}{\cellcolor{lightgray!50}{463090}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{463288}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{463288}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{463288}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.04}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{463288}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{5.53}} & \mc{1}{r}{\cellcolor{lightgray!50}{462200}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{feline}} & \mc{1}{|r}{\cellcolor{lightgray!50}{730.80}} & \mc{1}{r}{\cellcolor{lightgray!50}{2204925}} & \mc{1}{|r}{\cellcolor{lightgray!50}{734.34}} & \mc{1}{r}{\cellcolor{lightgray!50}{2204925}} & \mc{1}{|r}{\cellcolor{lightgray!50}{640.98}} & \mc{1}{r}{\cellcolor{lightgray!50}{2204911}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2207219}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2207219}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2207219}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.51}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2207219}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{270.27}} & \mc{1}{r}{\cellcolor{lightgray!50}{1713601}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{gameguy}} & \mc{1}{|r}{\cellcolor{lightgray!50}{519.12}} & \mc{1}{r}{\cellcolor{lightgray!50}{2323941}} & \mc{1}{|r}{\cellcolor{lightgray!50}{525.93}} & \mc{1}{r}{\cellcolor{lightgray!50}{2323941}} & \mc{1}{|r}{\cellcolor{lightgray!50}{736.64}} & \mc{1}{r}{\cellcolor{lightgray!50}{2322824}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2325878}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2325878}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2325878}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2325878}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{177.00}} & \mc{1}{r}{\cellcolor{lightgray!50}{1904924}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{gargoyle}} & \mc{1}{|r}{\cellcolor{lightgray!50}{29.25}} & \mc{1}{r}{\cellcolor{lightgray!50}{1058496}} & \mc{1}{|r}{\cellcolor{lightgray!50}{29.11}} & \mc{1}{r}{\cellcolor{lightgray!50}{1058496}} & \mc{1}{|r}{\cellcolor{lightgray!50}{724.41}} & \mc{1}{r}{\cellcolor{lightgray!50}{1058652}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1059559}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1059559}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1059559}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.28}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1059559}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{229.56}} & \mc{1}{r}{\cellcolor{lightgray!50}{875811}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{turtle}} & \mc{1}{|r}{\cellcolor{lightgray!50}{982.00}} & \mc{1}{r}{\cellcolor{lightgray!50}{14215429}} & \mc{1}{|r}{\cellcolor{lightgray!50}{976.57}} & \mc{1}{r}{\cellcolor{lightgray!50}{14213516}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.68}} & \mc{1}{r}{\cellcolor{lightgray!50}{14151616}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.42}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{14263005}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.43}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{14263005}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.56}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{14263005}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.58}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{14263005}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{407.58}} & \mc{1}{r}{\cellcolor{lightgray!50}{10233723}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{venus}} & \mc{1}{|r}{\cellcolor{lightgray!50}{559.29}} & \mc{1}{r}{\cellcolor{lightgray!50}{305571}} & \mc{1}{|r}{\cellcolor{lightgray!50}{556.38}} & \mc{1}{r}{\cellcolor{lightgray!50}{305571}} & \mc{1}{|r}{\cellcolor{lightgray!50}{130.83}} & \mc{1}{r}{\cellcolor{lightgray!50}{305724}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305749}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305749}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305749}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305749}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\cellcolor{lightgray!50}{304452}} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/best_weight_tables/osm.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccccccccc}

  \mc{1}{l}{Graph} & \mc{2}{|c}{DynWVC1} & \mc{2}{|c}{DynWVC2} & \mc{2}{|c}{HILS} & \mc{2}{|c}{Cyclic-Fast} & \mc{2}{|c}{Cyclic-Strong} & \mc{2}{|c}{Non-Increasing} & \mc{2}{|c}{Basic-Sparse} & \mc{2}{|c}{Basic-Dense} \\ 
  \hline  

   & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} \\ 
  \hline  

  \mc{1}{l}{\cellcolor{lightgray!50}{alabama-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.18}} & \mc{1}{r}{\cellcolor{lightgray!50}{174252}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.24}} & \mc{1}{r}{\cellcolor{lightgray!50}{174269}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{174309}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{174309}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{174309}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{174309}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.28}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{174309}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.28}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{174309}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{alabama-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{725.34}} & \mc{1}{r}{\cellcolor{lightgray!50}{185518}} & \mc{1}{|r}{\cellcolor{lightgray!50}{199.94}} & \mc{1}{r}{\cellcolor{lightgray!50}{185655}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.58}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{185744}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.76}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{185744}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{32.42}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{185744}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.60}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{185744}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{71.87}} & \mc{1}{r}{\cellcolor{lightgray!50}{185707}} & \mc{1}{|r}{\cellcolor{lightgray!50}{22.23}} & \mc{1}{r}{\cellcolor{lightgray!50}{185707}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{district-of-columbia-AM1}} & \mc{1}{|r}{\cellcolor{lightgray!50}{23.96}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{28.42}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.14}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.32}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.52}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.06}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.46}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{196475}}} \\  

  \mc{1}{l}{district-of-columbia-AM2} & \mc{1}{|r}{159.08} & \mc{1}{r}{208989} & \mc{1}{|r}{915.18} & \mc{1}{r}{208977} & \mc{1}{|r}{400.69} & \mc{1}{r}{\textbf{209132}} & \mc{1}{|r}{4.21} & \mc{1}{r}{\textbf{209132}} & \mc{1}{|r}{84.21} & \mc{1}{r}{209131} & \mc{1}{|r}{686.26} & \mc{1}{r}{174114} & \mc{1}{|r}{214.18} & \mc{1}{r}{148513} & \mc{1}{|r}{23.26} & \mc{1}{r}{148513} \\  

  \mc{1}{l}{district-of-columbia-AM3} & \mc{1}{|r}{461.10} & \mc{1}{r}{224760} & \mc{1}{|r}{313.17} & \mc{1}{r}{223955} & \mc{1}{|r}{849.37} & \mc{1}{r}{\textbf{227613}} & \mc{1}{|r}{904.91} & \mc{1}{r}{142454} & \mc{1}{|r}{804.79} & \mc{1}{r}{156967} & \mc{1}{|r}{168.55} & \mc{1}{r}{120366} & \mc{1}{|r}{673.89} & \mc{1}{r}{92804} & \mc{1}{|r}{65.42} & \mc{1}{r}{92804} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{florida-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.18}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.53}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.04}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{230595}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{florida-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{425.87}} & \mc{1}{r}{\cellcolor{lightgray!50}{237229}} & \mc{1}{|r}{\cellcolor{lightgray!50}{862.04}} & \mc{1}{r}{\cellcolor{lightgray!50}{237120}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.98}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{237333}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.57}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{237333}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{40.97}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{237333}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{237333}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{305.20}} & \mc{1}{r}{\cellcolor{lightgray!50}{226767}} & \mc{1}{|r}{\cellcolor{lightgray!50}{42.70}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{237333}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{georgia-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.42}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.31}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.04}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.98}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{12.97}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{14.56}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{861.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{842.78}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{222652}}} \\  

  \mc{1}{l}{greenland-AM3} & \mc{1}{|r}{58.88} & \mc{1}{r}{14007} & \mc{1}{|r}{640.46} & \mc{1}{r}{14010} & \mc{1}{|r}{1.18} & \mc{1}{r}{14011} & \mc{1}{|r}{10.95} & \mc{1}{r}{14011} & \mc{1}{|r}{58.24} & \mc{1}{r}{14008} & \mc{1}{|r}{5.06} & \mc{1}{r}{\textbf{14012}} & \mc{1}{|r}{35.22} & \mc{1}{r}{13829} & \mc{1}{|r}{15.89} & \mc{1}{r}{13829} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{hawaii-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.89}} & \mc{1}{r}{\cellcolor{lightgray!50}{125270}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.63}} & \mc{1}{r}{\cellcolor{lightgray!50}{125270}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.20}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{125284}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{125284}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.10}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{125284}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.13}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{125284}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.44}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{125284}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{125284}}} \\  

  \mc{1}{l}{hawaii-AM3} & \mc{1}{|r}{406.57} & \mc{1}{r}{140656} & \mc{1}{|r}{887.44} & \mc{1}{r}{140595} & \mc{1}{|r}{213.32} & \mc{1}{r}{\textbf{141035}} & \mc{1}{|r}{152.38} & \mc{1}{r}{116202} & \mc{1}{|r}{681.39} & \mc{1}{r}{121222} & \mc{1}{|r}{155.21} & \mc{1}{r}{107879} & \mc{1}{|r}{771.31} & \mc{1}{r}{96774} & \mc{1}{|r}{204.48} & \mc{1}{r}{106251} \\  

  \mc{1}{l}{idaho-AM3} & \mc{1}{|r}{79.67} & \mc{1}{r}{\textbf{77145}} & \mc{1}{|r}{58.83} & \mc{1}{r}{\textbf{77145}} & \mc{1}{|r}{0.78} & \mc{1}{r}{\textbf{77145}} & \mc{1}{|r}{11.95} & \mc{1}{r}{77141} & \mc{1}{|r}{40.71} & \mc{1}{r}{77144} & \mc{1}{|r}{8.89} & \mc{1}{r}{77144} & \mc{1}{|r}{42.51} & \mc{1}{r}{76991} & \mc{1}{|r}{455.18} & \mc{1}{r}{77010} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{kansas-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{333.60}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{87976}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{276.26}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{87976}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.55}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{87976}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.25}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{87976}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{110.41}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{87976}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{337.83}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{87976}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{14.95}} & \mc{1}{r}{\cellcolor{lightgray!50}{87955}} & \mc{1}{|r}{\cellcolor{lightgray!50}{12.67}} & \mc{1}{r}{\cellcolor{lightgray!50}{87955}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{kentucky-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.23}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.92}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.26}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.23}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.44}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.26}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{36.56}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{11.72}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97397}}} \\  

  \mc{1}{l}{kentucky-AM3} & \mc{1}{|r}{951.91} & \mc{1}{r}{100476} & \mc{1}{|r}{96.83} & \mc{1}{r}{100455} & \mc{1}{|r}{515.99} & \mc{1}{r}{100507} & \mc{1}{|r}{354.45} & \mc{1}{r}{\textbf{100510}} & \mc{1}{|r}{776.69} & \mc{1}{r}{\textbf{100510}} & \mc{1}{|r}{305.01} & \mc{1}{r}{100497} & \mc{1}{|r}{0.00} & \mc{1}{r}{0} & \mc{1}{|r}{831.07} & \mc{1}{r}{100311} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{louisiana-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.63}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.18}} & \mc{1}{r}{\cellcolor{lightgray!50}{60002}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.15}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{18.50}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{5.96}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{60024}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{maryland-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.79}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.59}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.15}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.14}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{10.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.46}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{45496}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{massachusetts-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.25}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.74}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.04}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.32}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.31}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{140095}}} \\  

  \mc{1}{l}{massachusetts-AM3} & \mc{1}{|r}{980.11} & \mc{1}{r}{145852} & \mc{1}{|r}{270.28} & \mc{1}{r}{145862} & \mc{1}{|r}{0.77} & \mc{1}{r}{\textbf{145866}} & \mc{1}{|r}{1.39} & \mc{1}{r}{\textbf{145866}} & \mc{1}{|r}{31.04} & \mc{1}{r}{\textbf{145866}} & \mc{1}{|r}{0.76} & \mc{1}{r}{\textbf{145866}} & \mc{1}{|r}{22.52} & \mc{1}{r}{145819} & \mc{1}{|r}{19.32} & \mc{1}{r}{145819} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{mexico-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.71}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.28}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.96}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{21.19}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.67}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{259.31}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{32.63}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{97663}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{new-hampshire-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.63}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.06}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{7.32}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{6.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{116060}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{north-carolina-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.58}} & \mc{1}{r}{\cellcolor{lightgray!50}{49694}} & \mc{1}{|r}{\cellcolor{lightgray!50}{114.45}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{49720}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{49720}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.74}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{49720}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{45.82}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{49720}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.47}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{49720}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{11.20}} & \mc{1}{r}{\cellcolor{lightgray!50}{49563}} & \mc{1}{|r}{\cellcolor{lightgray!50}{10.67}} & \mc{1}{r}{\cellcolor{lightgray!50}{49563}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{oregon-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.62}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.37}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.04}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{165047}}} \\  

  \mc{1}{l}{oregon-AM3} & \mc{1}{|r}{174.64} & \mc{1}{r}{175059} & \mc{1}{|r}{511.10} & \mc{1}{r}{175067} & \mc{1}{|r}{4.65} & \mc{1}{r}{\textbf{175078}} & \mc{1}{|r}{9.50} & \mc{1}{r}{\textbf{175078}} & \mc{1}{|r}{39.78} & \mc{1}{r}{175077} & \mc{1}{|r}{21.29} & \mc{1}{r}{\textbf{175078}} & \mc{1}{|r}{418.10} & \mc{1}{r}{164941} & \mc{1}{|r}{282.50} & \mc{1}{r}{174931} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{pennsylvania-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.06}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.14}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.12}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.16}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{33.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{20.61}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{143870}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{rhode-island-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{7.75}} & \mc{1}{r}{\cellcolor{lightgray!50}{184537}} & \mc{1}{|r}{\cellcolor{lightgray!50}{13.90}} & \mc{1}{r}{\cellcolor{lightgray!50}{184576}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.24}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{184596}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.41}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{184596}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.37}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{184596}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.27}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{184596}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{14.50}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{184596}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{9.87}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{184596}}} \\  

  \mc{1}{l}{rhode-island-AM3} & \mc{1}{|r}{230.53} & \mc{1}{r}{201470} & \mc{1}{|r}{711.97} & \mc{1}{r}{201359} & \mc{1}{|r}{30.15} & \mc{1}{r}{\textbf{201758}} & \mc{1}{|r}{44.88} & \mc{1}{r}{167162} & \mc{1}{|r}{82.02} & \mc{1}{r}{167162} & \mc{1}{|r}{45.46} & \mc{1}{r}{166103} & \mc{1}{|r}{196.07} & \mc{1}{r}{163150} & \mc{1}{|r}{13.44} & \mc{1}{r}{163150} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{utah-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{215.88}} & \mc{1}{r}{\cellcolor{lightgray!50}{98802}} & \mc{1}{|r}{\cellcolor{lightgray!50}{136.90}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.27}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.44}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{29.25}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{49.25}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{98847}}} \\  

  \mc{1}{l}{vermont-AM3} & \mc{1}{|r}{28.77} & \mc{1}{r}{63234} & \mc{1}{|r}{768.43} & \mc{1}{r}{63248} & \mc{1}{|r}{979.14} & \mc{1}{r}{63310} & \mc{1}{|r}{145.39} & \mc{1}{r}{\textbf{63312}} & \mc{1}{|r}{448.54} & \mc{1}{r}{\textbf{63312}} & \mc{1}{|r}{217.67} & \mc{1}{r}{\textbf{63312}} & \mc{1}{|r}{357.47} & \mc{1}{r}{55577} & \mc{1}{|r}{73.99} & \mc{1}{r}{55584} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{virginia-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.53}} & \mc{1}{r}{\cellcolor{lightgray!50}{295758}} & \mc{1}{|r}{\cellcolor{lightgray!50}{20.50}} & \mc{1}{r}{\cellcolor{lightgray!50}{295638}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{295867}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{295867}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{295867}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{295867}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.55}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{295867}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.56}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{295867}}} \\  

  \mc{1}{l}{virginia-AM3} & \mc{1}{|r}{754.86} & \mc{1}{r}{307782} & \mc{1}{|r}{809.24} & \mc{1}{r}{307907} & \mc{1}{|r}{2.52} & \mc{1}{r}{\textbf{308305}} & \mc{1}{|r}{34.42} & \mc{1}{r}{\textbf{308305}} & \mc{1}{|r}{200.13} & \mc{1}{r}{\textbf{308305}} & \mc{1}{|r}{49.42} & \mc{1}{r}{\textbf{308305}} & \mc{1}{|r}{968.54} & \mc{1}{r}{247790} & \mc{1}{|r}{109.05} & \mc{1}{r}{307741} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{washington-AM2}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.24}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{13.35}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.25}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.06}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.53}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.60}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{305619}}} \\  

  \mc{1}{l}{washington-AM3} & \mc{1}{|r}{37.94} & \mc{1}{r}{313689} & \mc{1}{|r}{383.62} & \mc{1}{r}{313844} & \mc{1}{|r}{10.17} & \mc{1}{r}{\textbf{314288}} & \mc{1}{|r}{3.60} & \mc{1}{r}{284684} & \mc{1}{|r}{72.84} & \mc{1}{r}{288116} & \mc{1}{|r}{4.56} & \mc{1}{r}{282020} & \mc{1}{|r}{469.20} & \mc{1}{r}{272404} & \mc{1}{|r}{228.47} & \mc{1}{r}{272404} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{west-virginia-AM3}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.75}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.84}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.88}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{41.73}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.60}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{831.85}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{22.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{47927}}} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/best_weight_tables/snap.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccccccc}

  \mc{1}{l}{Graph} & \mc{2}{|c}{DynWVC1} & \mc{2}{|c}{DynWVC2} & \mc{2}{|c}{HILS} & \mc{2}{|c}{Cyclic-Fast} & \mc{2}{|c}{Cyclic-Strong} & \mc{2}{|c}{Non-Increasing} & \mc{2}{|c}{Basic-Sparse} \\ 
  \hline  

   & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} & \mc{1}{|r}{$t_{max}$} & \mc{1}{r}{$w_{max}$} \\ 
  \hline  

  \mc{1}{l}{as-skitter} & \mc{1}{|r}{989.05} & \mc{1}{r}{123613404} & \mc{1}{|r}{383.97} & \mc{1}{r}{123273938} & \mc{1}{|r}{999.32} & \mc{1}{r}{122658804} & \mc{1}{|r}{346.69} & \mc{1}{r}{124137148} & \mc{1}{|r}{354.71} & \mc{1}{r}{\textbf{124137365}} & \mc{1}{|r}{431.90} & \mc{1}{r}{124136621} & \mc{1}{|r}{801.99} & \mc{1}{r}{124025255} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{ca-AstroPh}} & \mc{1}{|r}{\cellcolor{lightgray!50}{32.46}} & \mc{1}{r}{\cellcolor{lightgray!50}{797475}} & \mc{1}{|r}{\cellcolor{lightgray!50}{125.05}} & \mc{1}{r}{\cellcolor{lightgray!50}{797480}} & \mc{1}{|r}{\cellcolor{lightgray!50}{13.47}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{797510}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{797510}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{797510}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{797510}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{797510}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{ca-CondMat}} & \mc{1}{|r}{\cellcolor{lightgray!50}{114.85}} & \mc{1}{r}{\cellcolor{lightgray!50}{1147814}} & \mc{1}{|r}{\cellcolor{lightgray!50}{27.75}} & \mc{1}{r}{\cellcolor{lightgray!50}{1147845}} & \mc{1}{|r}{\cellcolor{lightgray!50}{50.90}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1147950}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1147950}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1147950}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1147950}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1147950}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{ca-GrQc}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.87}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.93}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.34}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{286489}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{ca-HepPh}} & \mc{1}{|r}{\cellcolor{lightgray!50}{13.21}} & \mc{1}{r}{\cellcolor{lightgray!50}{581014}} & \mc{1}{|r}{\cellcolor{lightgray!50}{17.34}} & \mc{1}{r}{\cellcolor{lightgray!50}{581028}} & \mc{1}{|r}{\cellcolor{lightgray!50}{7.73}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{581039}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{581039}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{581039}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{581039}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{581039}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{ca-HepTh}} & \mc{1}{|r}{\cellcolor{lightgray!50}{6.57}} & \mc{1}{r}{\cellcolor{lightgray!50}{561982}} & \mc{1}{|r}{\cellcolor{lightgray!50}{5.30}} & \mc{1}{r}{\cellcolor{lightgray!50}{561974}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.68}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{562004}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{562004}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{562004}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{562004}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{562004}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{email-Enron}} & \mc{1}{|r}{\cellcolor{lightgray!50}{454.49}} & \mc{1}{r}{\cellcolor{lightgray!50}{2464887}} & \mc{1}{|r}{\cellcolor{lightgray!50}{594.93}} & \mc{1}{r}{\cellcolor{lightgray!50}{2464890}} & \mc{1}{|r}{\cellcolor{lightgray!50}{71.07}} & \mc{1}{r}{\cellcolor{lightgray!50}{2464922}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2464935}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2464935}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2464935}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2464935}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{email-EuAll}} & \mc{1}{|r}{\cellcolor{lightgray!50}{134.83}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{132.62}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{338.14}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.06}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{25286322}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella04}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.46}} & \mc{1}{r}{\cellcolor{lightgray!50}{679105}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.34}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{679111}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{94.12}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{679111}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{679111}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{679111}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{679111}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{679111}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella05}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.15}} & \mc{1}{r}{\cellcolor{lightgray!50}{554926}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.55}} & \mc{1}{r}{\cellcolor{lightgray!50}{554931}} & \mc{1}{|r}{\cellcolor{lightgray!50}{135.17}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{554943}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{554943}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{554943}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{554943}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{554943}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella06}} & \mc{1}{|r}{\cellcolor{lightgray!50}{525.35}} & \mc{1}{r}{\cellcolor{lightgray!50}{548611}} & \mc{1}{|r}{\cellcolor{lightgray!50}{186.97}} & \mc{1}{r}{\cellcolor{lightgray!50}{548611}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{548612}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{548612}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{548612}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{548612}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{548612}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella08}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.15}} & \mc{1}{r}{\cellcolor{lightgray!50}{434575}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.18}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{434577}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.12}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{434577}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{434577}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{434577}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{434577}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{434577}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella09}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.39}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.28}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.00}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{568439}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella24}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{5.51}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.17}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1984567}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella25}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.66}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.20}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.17}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{1701967}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella30}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.83}} & \mc{1}{r}{\cellcolor{lightgray!50}{2787903}} & \mc{1}{|r}{\cellcolor{lightgray!50}{132.71}} & \mc{1}{r}{\cellcolor{lightgray!50}{2787899}} & \mc{1}{|r}{\cellcolor{lightgray!50}{15.14}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2787907}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2787907}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2787907}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2787907}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{2787907}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{p2p-Gnutella31}} & \mc{1}{|r}{\cellcolor{lightgray!50}{70.88}} & \mc{1}{r}{\cellcolor{lightgray!50}{4776960}} & \mc{1}{|r}{\cellcolor{lightgray!50}{47.97}} & \mc{1}{r}{\cellcolor{lightgray!50}{4776961}} & \mc{1}{|r}{\cellcolor{lightgray!50}{115.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{4776986}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{4776986}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{4776986}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{4776986}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.03}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{4776986}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{roadNet-CA}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.98}} & \mc{1}{r}{\cellcolor{lightgray!50}{109586054}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.90}} & \mc{1}{r}{\cellcolor{lightgray!50}{109582579}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1000.00}} & \mc{1}{r}{\cellcolor{lightgray!50}{106584645}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.94}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{111360828}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.86}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{111360828}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{4.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{111360828}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{437.34}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{111360828}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{roadNet-PA}} & \mc{1}{|r}{\cellcolor{lightgray!50}{511.59}} & \mc{1}{r}{\cellcolor{lightgray!50}{60990177}} & \mc{1}{|r}{\cellcolor{lightgray!50}{469.18}} & \mc{1}{r}{\cellcolor{lightgray!50}{60990177}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.94}} & \mc{1}{r}{\cellcolor{lightgray!50}{60037011}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.96}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{61731589}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.04}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{61731589}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.83}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{61731589}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{16.49}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{61731589}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{roadNet-TX}} & \mc{1}{|r}{\cellcolor{lightgray!50}{789.43}} & \mc{1}{r}{\cellcolor{lightgray!50}{77672388}} & \mc{1}{|r}{\cellcolor{lightgray!50}{694.33}} & \mc{1}{r}{\cellcolor{lightgray!50}{77672388}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.97}} & \mc{1}{r}{\cellcolor{lightgray!50}{76347666}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{78599946}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{78599946}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{3.42}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{78599946}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{22.78}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{78599946}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{soc-Epinions1}} & \mc{1}{|r}{\cellcolor{lightgray!50}{290.84}} & \mc{1}{r}{\cellcolor{lightgray!50}{5690651}} & \mc{1}{|r}{\cellcolor{lightgray!50}{272.56}} & \mc{1}{r}{\cellcolor{lightgray!50}{5690773}} & \mc{1}{|r}{\cellcolor{lightgray!50}{253.10}} & \mc{1}{r}{\cellcolor{lightgray!50}{5690874}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5690970}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5690970}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5690970}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.07}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5690970}}} \\  

  \mc{1}{l}{soc-LiveJournal1} & \mc{1}{|r}{999.99} & \mc{1}{r}{279150686} & \mc{1}{|r}{999.99} & \mc{1}{r}{279231875} & \mc{1}{|r}{1000.00} & \mc{1}{r}{255079926} & \mc{1}{|r}{51.33} & \mc{1}{r}{284036222} & \mc{1}{|r}{44.19} & \mc{1}{r}{\textbf{284036239}} & \mc{1}{|r}{39.36} & \mc{1}{r}{283970295} & \mc{1}{|r}{231.80} & \mc{1}{r}{284010263} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{soc-Slashdot0811}} & \mc{1}{|r}{\cellcolor{lightgray!50}{238.18}} & \mc{1}{r}{\cellcolor{lightgray!50}{5660385}} & \mc{1}{|r}{\cellcolor{lightgray!50}{880.68}} & \mc{1}{r}{\cellcolor{lightgray!50}{5660555}} & \mc{1}{|r}{\cellcolor{lightgray!50}{446.95}} & \mc{1}{r}{\cellcolor{lightgray!50}{5660787}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.09}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5660899}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5660899}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5660899}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.08}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5660899}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{soc-Slashdot0902}} & \mc{1}{|r}{\cellcolor{lightgray!50}{270.85}} & \mc{1}{r}{\cellcolor{lightgray!50}{5971308}} & \mc{1}{|r}{\cellcolor{lightgray!50}{435.90}} & \mc{1}{r}{\cellcolor{lightgray!50}{5971476}} & \mc{1}{|r}{\cellcolor{lightgray!50}{604.07}} & \mc{1}{r}{\cellcolor{lightgray!50}{5971664}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5971849}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5971849}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.12}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5971849}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.11}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{5971849}}} \\  

  \mc{1}{l}{soc-pokec-relationships} & \mc{1}{|r}{999.85} & \mc{1}{r}{\textbf{83223668}} & \mc{1}{|r}{999.13} & \mc{1}{r}{83155217} & \mc{1}{|r}{1000.00} & \mc{1}{r}{82021946} & \mc{1}{|r}{254.59} & \mc{1}{r}{76075111} & \mc{1}{|r}{488.31} & \mc{1}{r}{76075700} & \mc{1}{|r}{228.07} & \mc{1}{r}{76063476} & \mc{1}{|r}{0.00} & \mc{1}{r}{0} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{web-BerkStan}} & \mc{1}{|r}{\cellcolor{lightgray!50}{194.20}} & \mc{1}{r}{\cellcolor{lightgray!50}{43640833}} & \mc{1}{|r}{\cellcolor{lightgray!50}{164.10}} & \mc{1}{r}{\cellcolor{lightgray!50}{43637382}} & \mc{1}{|r}{\cellcolor{lightgray!50}{998.73}} & \mc{1}{r}{\cellcolor{lightgray!50}{43424373}} & \mc{1}{|r}{\cellcolor{lightgray!50}{6.74}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{43907482}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{8.05}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{43907482}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{16.01}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{43907482}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{50.88}} & \mc{1}{r}{\cellcolor{lightgray!50}{43742339}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{web-Google}} & \mc{1}{|r}{\cellcolor{lightgray!50}{349.08}} & \mc{1}{r}{\cellcolor{lightgray!50}{56209005}} & \mc{1}{|r}{\cellcolor{lightgray!50}{324.65}} & \mc{1}{r}{\cellcolor{lightgray!50}{56206250}} & \mc{1}{|r}{\cellcolor{lightgray!50}{995.92}} & \mc{1}{r}{\cellcolor{lightgray!50}{56008278}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.72}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{56326504}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{6.44}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{56326504}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.17}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{56326504}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.86}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{56326504}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{web-NotreDame}} & \mc{1}{|r}{\cellcolor{lightgray!50}{949.84}} & \mc{1}{r}{\cellcolor{lightgray!50}{26010791}} & \mc{1}{|r}{\cellcolor{lightgray!50}{905.72}} & \mc{1}{r}{\cellcolor{lightgray!50}{26009287}} & \mc{1}{|r}{\cellcolor{lightgray!50}{997.00}} & \mc{1}{r}{\cellcolor{lightgray!50}{26002793}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.60}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{26016941}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.74}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{26016941}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.36}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{26016941}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{99.49}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{26016941}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{web-Stanford}} & \mc{1}{|r}{\cellcolor{lightgray!50}{943.85}} & \mc{1}{r}{\cellcolor{lightgray!50}{17748798}} & \mc{1}{|r}{\cellcolor{lightgray!50}{671.32}} & \mc{1}{r}{\cellcolor{lightgray!50}{17741043}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.50}} & \mc{1}{r}{\cellcolor{lightgray!50}{17709827}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.68}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{17792930}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.86}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{17792930}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.71}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{17792930}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{2.51}} & \mc{1}{r}{\cellcolor{lightgray!50}{17792824}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{wiki-Talk}} & \mc{1}{|r}{\cellcolor{lightgray!50}{951.51}} & \mc{1}{r}{\cellcolor{lightgray!50}{235836837}} & \mc{1}{|r}{\cellcolor{lightgray!50}{972.93}} & \mc{1}{r}{\cellcolor{lightgray!50}{235836913}} & \mc{1}{|r}{\cellcolor{lightgray!50}{999.69}} & \mc{1}{r}{\cellcolor{lightgray!50}{235818823}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{235837346}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.29}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{235837346}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.31}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{235837346}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{1.30}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{235837346}}} \\  

  \mc{1}{l}{\cellcolor{lightgray!50}{wiki-Vote}} & \mc{1}{|r}{\cellcolor{lightgray!50}{188.76}} & \mc{1}{r}{\cellcolor{lightgray!50}{500075}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.32}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{500079}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{10.34}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{500079}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{500079}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{500079}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{500079}}} & \mc{1}{|r}{\cellcolor{lightgray!50}{0.02}} & \mc{1}{r}{\textbf{\cellcolor{lightgray!50}{500079}}} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_size_tables/bnr_time_table_fe.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}
  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  
  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  
  \mc{1}{l|}{fe\_4elt2} & \mc{1}{r}{8580} & \mc{1}{r}{0.29} & \mc{1}{r|}{-} & \mc{1}{r}{8578} & \mc{1}{r}{0.87} & \mc{1}{r|}{-} & \mc{1}{r}{562} & \mc{1}{r}{0.10} & \mc{1}{r|}{-} & \mc{1}{r}{0} & \mc{1}{r}{0.12} & \mc{1}{r|}{\textbf{0.13}} & \mc{1}{r}{0} & \mc{1}{r}{0.16} & \mc{1}{r}{0.17} \\  
  \mc{1}{l|}{fe\_body} & \mc{1}{r}{16107} & \mc{1}{r}{0.69} & \mc{1}{r|}{-} & \mc{1}{r}{15992} & \mc{1}{r}{3.40} & \mc{1}{r|}{-} & \mc{1}{r}{1162} & \mc{1}{r}{0.16} & \mc{1}{r|}{-} & \mc{1}{r}{625} & \mc{1}{r}{0.44} & \mc{1}{r|}{-} & \mc{1}{r}{553} & \mc{1}{r}{0.94} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_ocean} & \mc{1}{r}{141283} & \mc{1}{r}{1.05} & \mc{1}{r|}{-} & \mc{1}{r}{0} & \mc{1}{r}{5.94} & \mc{1}{r|}{\textbf{5.99}} & \mc{1}{r}{138338} & \mc{1}{r}{8.90} & \mc{1}{r|}{-} & \mc{1}{r}{138134} & \mc{1}{r}{9.61} & \mc{1}{r|}{-} & \mc{1}{r}{138049} & \mc{1}{r}{10.78} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_pwt} & \mc{1}{r}{34521} & \mc{1}{r}{0.46} & \mc{1}{r|}{-} & \mc{1}{r}{34521} & \mc{1}{r}{2.70} & \mc{1}{r|}{-} & \mc{1}{r}{25550} & \mc{1}{r}{0.78} & \mc{1}{r|}{-} & \mc{1}{r}{20241} & \mc{1}{r}{1.80} & \mc{1}{r|}{-} & \mc{1}{r}{14107} & \mc{1}{r}{5.65} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_rotor} & \mc{1}{r}{98271} & \mc{1}{r}{9.80} & \mc{1}{r|}{-} & \mc{1}{r}{98271} & \mc{1}{r}{24.47} & \mc{1}{r|}{-} & \mc{1}{r}{91946} & \mc{1}{r}{4.80} & \mc{1}{r|}{-} & \mc{1}{r}{91634} & \mc{1}{r}{4.82} & \mc{1}{r|}{-} & \mc{1}{r}{89647} & \mc{1}{r}{11.11} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{15269} & \mc{1}{r}{0.21} & \mc{1}{r|}{-} & \mc{1}{r}{15269} & \mc{1}{r}{1.47} & \mc{1}{r|}{-} & \mc{1}{r}{2961} & \mc{1}{r}{0.34} & \mc{1}{r|}{-} & \mc{1}{r}{147} & \mc{1}{r}{0.62} & \mc{1}{r|}{\textbf{0.83}} & \mc{1}{r}{0} & \mc{1}{r}{0.75} & \mc{1}{r}{0.77} \\  
  \mc{1}{l|}{fe\_tooth} & \mc{1}{r}{10922} & \mc{1}{r}{1.69} & \mc{1}{r|}{-} & \mc{1}{r}{10801} & \mc{1}{r}{3.79} & \mc{1}{r|}{-} & \mc{1}{r}{15} & \mc{1}{r}{0.41} & \mc{1}{r|}{0.46} & \mc{1}{r}{0} & \mc{1}{r}{0.30} & \mc{1}{r|}{\textbf{0.34}} & \mc{1}{r}{0} & \mc{1}{r}{0.28} & \mc{1}{r}{0.32} \\  
\end{tabu}
\end{ThreePartTable}

==> tables/bnr_size_tables/bnr_time_table_mesh.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{beethoven} & \mc{1}{r}{1254} & \mc{1}{r}{0.02} & \mc{1}{r|}{7.86} & \mc{1}{r}{427} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.08} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{blob} & \mc{1}{r}{5746} & \mc{1}{r}{0.08} & \mc{1}{r|}{-} & \mc{1}{r}{1464} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.20} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r}{380315} & \mc{1}{r}{5.56} & \mc{1}{r|}{-} & \mc{1}{r}{107265} & \mc{1}{r}{26.19} & \mc{1}{r|}{67.85} & \mc{1}{r}{86} & \mc{1}{r}{1.83} & \mc{1}{r|}{2.74} & \mc{1}{r}{0} & \mc{1}{r}{1.87} & \mc{1}{r|}{\textbf{2.26}} & \mc{1}{r}{0} & \mc{1}{r}{1.91} & \mc{1}{r}{2.39} \\  

  \mc{1}{l|}{bunny} & \mc{1}{r}{24580} & \mc{1}{r}{0.34} & \mc{1}{r|}{-} & \mc{1}{r}{3290} & \mc{1}{r}{0.56} & \mc{1}{r|}{0.89} & \mc{1}{r}{0} & \mc{1}{r}{0.12} & \mc{1}{r|}{\textbf{0.14}} & \mc{1}{r}{0} & \mc{1}{r}{0.13} & \mc{1}{r|}{0.16} & \mc{1}{r}{0} & \mc{1}{r}{0.15} & \mc{1}{r}{0.18} \\  

  \mc{1}{l|}{cow} & \mc{1}{r}{1916} & \mc{1}{r}{0.02} & \mc{1}{r|}{-} & \mc{1}{r}{513} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.06} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{dragon} & \mc{1}{r}{51885} & \mc{1}{r}{0.89} & \mc{1}{r|}{-} & \mc{1}{r}{12893} & \mc{1}{r}{1.34} & \mc{1}{r|}{3.83} & \mc{1}{r}{0} & \mc{1}{r}{0.18} & \mc{1}{r|}{\textbf{0.21}} & \mc{1}{r}{0} & \mc{1}{r}{0.19} & \mc{1}{r|}{0.23} & \mc{1}{r}{0} & \mc{1}{r}{0.21} & \mc{1}{r}{0.25} \\  

  \mc{1}{l|}{dragonsub} & \mc{1}{r}{218779} & \mc{1}{r}{2.60} & \mc{1}{r|}{-} & \mc{1}{r}{19470} & \mc{1}{r}{4.15} & \mc{1}{r|}{5.66} & \mc{1}{r}{506} & \mc{1}{r}{1.03} & \mc{1}{r|}{2.08} & \mc{1}{r}{0} & \mc{1}{r}{1.13} & \mc{1}{r|}{\textbf{1.36}} & \mc{1}{r}{0} & \mc{1}{r}{1.07} & \mc{1}{r}{1.28} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r}{239787} & \mc{1}{r}{4.07} & \mc{1}{r|}{-} & \mc{1}{r}{26270} & \mc{1}{r}{10.09} & \mc{1}{r|}{12.93} & \mc{1}{r}{274} & \mc{1}{r}{2.12} & \mc{1}{r|}{3.16} & \mc{1}{r}{0} & \mc{1}{r}{2.12} & \mc{1}{r|}{\textbf{2.51}} & \mc{1}{r}{0} & \mc{1}{r}{2.14} & \mc{1}{r}{2.56} \\  

  \mc{1}{l|}{face} & \mc{1}{r}{7588} & \mc{1}{r}{0.09} & \mc{1}{r|}{-} & \mc{1}{r}{1540} & \mc{1}{r}{0.10} & \mc{1}{r|}{0.21} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.04} \\  

  \mc{1}{l|}{fandisk} & \mc{1}{r}{2851} & \mc{1}{r}{0.05} & \mc{1}{r|}{-} & \mc{1}{r}{336} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.07} & \mc{1}{r}{51} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{feline} & \mc{1}{r}{14817} & \mc{1}{r}{0.20} & \mc{1}{r|}{-} & \mc{1}{r}{2743} & \mc{1}{r}{0.25} & \mc{1}{r|}{0.47} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.09} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r}{0.09} \\  

  \mc{1}{l|}{gameguy} & \mc{1}{r}{13959} & \mc{1}{r}{0.17} & \mc{1}{r|}{-} & \mc{1}{r}{312} & \mc{1}{r}{0.10} & \mc{1}{r|}{0.12} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{gargoyle} & \mc{1}{r}{6512} & \mc{1}{r}{0.15} & \mc{1}{r|}{-} & \mc{1}{r}{1819} & \mc{1}{r}{0.14} & \mc{1}{r|}{0.36} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{turtle} & \mc{1}{r}{91624} & \mc{1}{r}{1.17} & \mc{1}{r|}{-} & \mc{1}{r}{16095} & \mc{1}{r}{1.92} & \mc{1}{r|}{4.98} & \mc{1}{r}{186} & \mc{1}{r}{0.42} & \mc{1}{r|}{0.65} & \mc{1}{r}{0} & \mc{1}{r}{0.41} & \mc{1}{r|}{\textbf{0.49}} & \mc{1}{r}{0} & \mc{1}{r}{0.47} & \mc{1}{r}{0.56} \\  

  \mc{1}{l|}{venus} & \mc{1}{r}{1898} & \mc{1}{r}{0.02} & \mc{1}{r|}{-} & \mc{1}{r}{175} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_size_tables/bnr_time_table_osm.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{alabama-AM2} & \mc{1}{r}{173} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.31} & \mc{1}{r}{173} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.55} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{alabama-AM3} & \mc{1}{r}{1614} & \mc{1}{r}{12.05} & \mc{1}{r|}{-} & \mc{1}{r}{1614} & \mc{1}{r}{14.37} & \mc{1}{r|}{-} & \mc{1}{r}{1288} & \mc{1}{r}{0.34} & \mc{1}{r|}{-} & \mc{1}{r}{456} & \mc{1}{r}{1.45} & \mc{1}{r|}{\textbf{3.94}} & \mc{1}{r}{0} & \mc{1}{r}{33.11} & \mc{1}{r}{33.16} \\  

  \mc{1}{l|}{district-of-columbia-AM1} & \mc{1}{r}{800} & \mc{1}{r}{1.22} & \mc{1}{r|}{-} & \mc{1}{r}{800} & \mc{1}{r}{1.28} & \mc{1}{r|}{-} & \mc{1}{r}{367} & \mc{1}{r}{0.03} & \mc{1}{r|}{39.81} & \mc{1}{r}{185} & \mc{1}{r}{0.41} & \mc{1}{r|}{\textbf{0.80}} & \mc{1}{r}{0} & \mc{1}{r}{3.65} & \mc{1}{r}{3.66} \\  

  \mc{1}{l|}{district-of-columbia-AM2} & \mc{1}{r}{6360} & \mc{1}{r}{11.86} & \mc{1}{r|}{-} & \mc{1}{r}{6360} & \mc{1}{r}{14.39} & \mc{1}{r|}{-} & \mc{1}{r}{5606} & \mc{1}{r}{0.85} & \mc{1}{r|}{-} & \mc{1}{r}{1855} & \mc{1}{r}{2.51} & \mc{1}{r|}{-} & \mc{1}{r}{1484} & \mc{1}{r}{84.91} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{district-of-columbia-AM3} & \mc{1}{r}{33367} & \mc{1}{r}{63.23} & \mc{1}{r|}{-} & \mc{1}{r}{33367} & \mc{1}{r}{358.14} & \mc{1}{r|}{-} & \mc{1}{r}{32320} & \mc{1}{r}{33.68} & \mc{1}{r|}{-} & \mc{1}{r}{28842} & \mc{1}{r}{66.67} & \mc{1}{r|}{-} & \mc{1}{r}{25031} & \mc{1}{r}{441.44} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{florida-AM2} & \mc{1}{r}{41} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{41} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{florida-AM3} & \mc{1}{r}{1069} & \mc{1}{r}{31.52} & \mc{1}{r|}{45.81} & \mc{1}{r}{1069} & \mc{1}{r}{35.20} & \mc{1}{r|}{-} & \mc{1}{r}{814} & \mc{1}{r}{0.13} & \mc{1}{r|}{3.85} & \mc{1}{r}{661} & \mc{1}{r}{0.44} & \mc{1}{r|}{\textbf{2.93}} & \mc{1}{r}{267} & \mc{1}{r}{42.26} & \mc{1}{r}{45.05} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{861} & \mc{1}{r}{8.99} & \mc{1}{r|}{892.17} & \mc{1}{r}{861} & \mc{1}{r}{10.14} & \mc{1}{r|}{-} & \mc{1}{r}{796} & \mc{1}{r}{0.08} & \mc{1}{r|}{25.97} & \mc{1}{r}{587} & \mc{1}{r}{0.69} & \mc{1}{r|}{\textbf{10.35}} & \mc{1}{r}{425} & \mc{1}{r}{12.84} & \mc{1}{r}{32.53} \\  

  \mc{1}{l|}{greenland-AM3} & \mc{1}{r}{3942} & \mc{1}{r}{3.81} & \mc{1}{r|}{-} & \mc{1}{r}{3942} & \mc{1}{r}{24.77} & \mc{1}{r|}{-} & \mc{1}{r}{3953} & \mc{1}{r}{3.94} & \mc{1}{r|}{-} & \mc{1}{r}{3339} & \mc{1}{r}{10.27} & \mc{1}{r|}{-} & \mc{1}{r}{3339} & \mc{1}{r}{54.44} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{hawaii-AM2} & \mc{1}{r}{428} & \mc{1}{r}{2.08} & \mc{1}{r|}{4.27} & \mc{1}{r}{428} & \mc{1}{r}{2.15} & \mc{1}{r|}{10.22} & \mc{1}{r}{262} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.18} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.10} & \mc{1}{r}{0.10} \\  

  \mc{1}{l|}{hawaii-AM3} & \mc{1}{r}{24436} & \mc{1}{r}{70.38} & \mc{1}{r|}{-} & \mc{1}{r}{24436} & \mc{1}{r}{743.04} & \mc{1}{r|}{-} & \mc{1}{r}{24184} & \mc{1}{r}{98.22} & \mc{1}{r|}{-} & \mc{1}{r}{22997} & \mc{1}{r}{118.52} & \mc{1}{r|}{-} & \mc{1}{r}{21087} & \mc{1}{r}{632.02} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{idaho-AM3} & \mc{1}{r}{3208} & \mc{1}{r}{3.17} & \mc{1}{r|}{-} & \mc{1}{r}{3208} & \mc{1}{r}{29.91} & \mc{1}{r|}{-} & \mc{1}{r}{3204} & \mc{1}{r}{6.96} & \mc{1}{r|}{-} & \mc{1}{r}{3160} & \mc{1}{r}{8.74} & \mc{1}{r|}{-} & \mc{1}{r}{2909} & \mc{1}{r}{33.77} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{kansas-AM3} & \mc{1}{r}{1605} & \mc{1}{r}{2.46} & \mc{1}{r|}{-} & \mc{1}{r}{1605} & \mc{1}{r}{4.81} & \mc{1}{r|}{-} & \mc{1}{r}{1550} & \mc{1}{r}{0.49} & \mc{1}{r|}{-} & \mc{1}{r}{903} & \mc{1}{r}{2.46} & \mc{1}{r|}{\textbf{430.93}} & \mc{1}{r}{860} & \mc{1}{r}{41.61} & \mc{1}{r}{489.15} \\  

  \mc{1}{l|}{kentucky-AM2} & \mc{1}{r}{442} & \mc{1}{r}{2.05} & \mc{1}{r|}{11.85} & \mc{1}{r}{442} & \mc{1}{r}{2.19} & \mc{1}{r|}{67.28} & \mc{1}{r}{183} & \mc{1}{r}{0.20} & \mc{1}{r|}{0.39} & \mc{1}{r}{0} & \mc{1}{r}{0.22} & \mc{1}{r|}{\textbf{0.23}} & \mc{1}{r}{0} & \mc{1}{r}{0.41} & \mc{1}{r}{0.42} \\  

  \mc{1}{l|}{kentucky-AM3} & \mc{1}{r}{16871} & \mc{1}{r}{109.47} & \mc{1}{r|}{-} & \mc{1}{r}{16871} & \mc{1}{r}{3344.67} & \mc{1}{r|}{-} & \mc{1}{r}{16807} & \mc{1}{r}{237.86} & \mc{1}{r|}{-} & \mc{1}{r}{15947} & \mc{1}{r}{298.49} & \mc{1}{r|}{-} & \mc{1}{r}{15684} & \mc{1}{r}{705.46} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{louisiana-AM3} & \mc{1}{r}{382} & \mc{1}{r}{4.56} & \mc{1}{r|}{6.55} & \mc{1}{r}{382} & \mc{1}{r}{5.04} & \mc{1}{r|}{25.22} & \mc{1}{r}{349} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.82} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.16} & \mc{1}{r}{0.16} \\  

  \mc{1}{l|}{maryland-AM3} & \mc{1}{r}{187} & \mc{1}{r}{7.59} & \mc{1}{r|}{8.49} & \mc{1}{r}{187} & \mc{1}{r}{8.65} & \mc{1}{r|}{10.73} & \mc{1}{r}{335} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.19} & \mc{1}{r}{0} & \mc{1}{r}{0.11} & \mc{1}{r|}{\textbf{0.11}} & \mc{1}{r}{0} & \mc{1}{r}{0.15} & \mc{1}{r}{0.15} \\  

  \mc{1}{l|}{massachusetts-AM2} & \mc{1}{r}{196} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.36} & \mc{1}{r}{196} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.58} & \mc{1}{r}{193} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.06}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{massachusetts-AM3} & \mc{1}{r}{2008} & \mc{1}{r}{9.42} & \mc{1}{r|}{-} & \mc{1}{r}{2008} & \mc{1}{r}{12.62} & \mc{1}{r|}{-} & \mc{1}{r}{1928} & \mc{1}{r}{0.36} & \mc{1}{r|}{-} & \mc{1}{r}{1636} & \mc{1}{r}{1.08} & \mc{1}{r|}{-} & \mc{1}{r}{1632} & \mc{1}{r}{31.83} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{mexico-AM3} & \mc{1}{r}{620} & \mc{1}{r}{25.29} & \mc{1}{r|}{80.23} & \mc{1}{r}{620} & \mc{1}{r}{27.52} & \mc{1}{r|}{991.99} & \mc{1}{r}{514} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{1.47}} & \mc{1}{r}{483} & \mc{1}{r}{0.28} & \mc{1}{r|}{1.50} & \mc{1}{r}{0} & \mc{1}{r}{21.03} & \mc{1}{r}{21.30} \\  

  \mc{1}{l|}{new-hampshire-AM3} & \mc{1}{r}{247} & \mc{1}{r}{4.99} & \mc{1}{r|}{6.19} & \mc{1}{r}{247} & \mc{1}{r}{5.69} & \mc{1}{r|}{15.89} & \mc{1}{r}{164} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.17} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r}{0.09} \\  

  \mc{1}{l|}{north-carolina-AM3} & \mc{1}{r}{1178} & \mc{1}{r}{0.69} & \mc{1}{r|}{-} & \mc{1}{r}{1178} & \mc{1}{r}{1.22} & \mc{1}{r|}{-} & \mc{1}{r}{1146} & \mc{1}{r}{0.25} & \mc{1}{r|}{-} & \mc{1}{r}{1144} & \mc{1}{r}{0.43} & \mc{1}{r|}{-} & \mc{1}{r}{700} & \mc{1}{r}{47.38} & \mc{1}{r}{379.088} \\  

  \mc{1}{l|}{oregon-AM2} & \mc{1}{r}{35} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.05} & \mc{1}{r}{35} & \mc{1}{r}{0.05} & \mc{1}{r|}{0.05} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{oregon-AM3} & \mc{1}{r}{3670} & \mc{1}{r}{9.95} & \mc{1}{r|}{-} & \mc{1}{r}{3670} & \mc{1}{r}{34.95} & \mc{1}{r|}{-} & \mc{1}{r}{3584} & \mc{1}{r}{3.92} & \mc{1}{r|}{-} & \mc{1}{r}{3417} & \mc{1}{r}{6.21} & \mc{1}{r|}{-} & \mc{1}{r}{2721} & \mc{1}{r}{38.72} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{pennsylvania-AM3} & \mc{1}{r}{315} & \mc{1}{r}{16.69} & \mc{1}{r|}{20.71} & \mc{1}{r}{315} & \mc{1}{r}{19.39} & \mc{1}{r|}{113.87} & \mc{1}{r}{317} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.39} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.12} & \mc{1}{r}{0.12} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r}{1103} & \mc{1}{r}{0.55} & \mc{1}{r|}{-} & \mc{1}{r}{1103} & \mc{1}{r}{0.68} & \mc{1}{r|}{-} & \mc{1}{r}{845} & \mc{1}{r}{0.17} & \mc{1}{r|}{163.07} & \mc{1}{r}{0} & \mc{1}{r}{0.53} & \mc{1}{r|}{\textbf{0.53}} & \mc{1}{r}{0} & \mc{1}{r}{4.57} & \mc{1}{r}{4.58} \\  

  \mc{1}{l|}{rhode-island-AM3} & \mc{1}{r}{13031} & \mc{1}{r}{7.75} & \mc{1}{r|}{-} & \mc{1}{r}{13031} & \mc{1}{r}{193.76} & \mc{1}{r|}{-} & \mc{1}{r}{12934} & \mc{1}{r}{26.54} & \mc{1}{r|}{-} & \mc{1}{r}{12653} & \mc{1}{r}{29.75} & \mc{1}{r|}{-} & \mc{1}{r}{12653} & \mc{1}{r}{59.69} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{utah-AM3} & \mc{1}{r}{568} & \mc{1}{r}{8.21} & \mc{1}{r|}{51.91} & \mc{1}{r}{568} & \mc{1}{r}{8.97} & \mc{1}{r|}{276.27} & \mc{1}{r}{396} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.87} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.40} & \mc{1}{r}{0.41} \\  

  \mc{1}{l|}{vermont-AM3} & \mc{1}{r}{2630} & \mc{1}{r}{4.79} & \mc{1}{r|}{-} & \mc{1}{r}{2630} & \mc{1}{r}{9.82} & \mc{1}{r|}{-} & \mc{1}{r}{2289} & \mc{1}{r}{0.97} & \mc{1}{r|}{-} & \mc{1}{r}{2069} & \mc{1}{r}{1.37} & \mc{1}{r|}{-} & \mc{1}{r}{2045} & \mc{1}{r}{55.28} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{virginia-AM2} & \mc{1}{r}{237} & \mc{1}{r}{0.13} & \mc{1}{r|}{0.61} & \mc{1}{r}{237} & \mc{1}{r}{0.12} & \mc{1}{r|}{0.99} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{virginia-AM3} & \mc{1}{r}{3867} & \mc{1}{r}{34.13} & \mc{1}{r|}{-} & \mc{1}{r}{3867} & \mc{1}{r}{39.74} & \mc{1}{r|}{-} & \mc{1}{r}{3738} & \mc{1}{r}{0.40} & \mc{1}{r|}{-} & \mc{1}{r}{2827} & \mc{1}{r}{1.28} & \mc{1}{r|}{-} & \mc{1}{r}{2547} & \mc{1}{r}{81.67} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{washington-AM2} & \mc{1}{r}{382} & \mc{1}{r}{0.24} & \mc{1}{r|}{5.31} & \mc{1}{r}{382} & \mc{1}{r}{0.18} & \mc{1}{r|}{8.58} & \mc{1}{r}{171} & \mc{1}{r}{0.05} & \mc{1}{r|}{0.37} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.06}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{washington-AM3} & \mc{1}{r}{8030} & \mc{1}{r}{50.21} & \mc{1}{r|}{-} & \mc{1}{r}{8030} & \mc{1}{r}{67.00} & \mc{1}{r|}{-} & \mc{1}{r}{7649} & \mc{1}{r}{2.19} & \mc{1}{r|}{-} & \mc{1}{r}{6895} & \mc{1}{r}{3.12} & \mc{1}{r|}{-} & \mc{1}{r}{6159} & \mc{1}{r}{73.52} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{west-virginia-AM3} & \mc{1}{r}{991} & \mc{1}{r}{10.69} & \mc{1}{r|}{-} & \mc{1}{r}{991} & \mc{1}{r}{12.13} & \mc{1}{r|}{-} & \mc{1}{r}{970} & \mc{1}{r}{0.08} & \mc{1}{r|}{238.39} & \mc{1}{r}{890} & \mc{1}{r}{0.33} & \mc{1}{r|}{\textbf{155.49}} & \mc{1}{r}{881} & \mc{1}{r}{38.73} & \mc{1}{r}{241.68} \\  

\end{tabu}
\end{ThreePartTable}


==> tables/bnr_size_tables/bnr_time_table_snap.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{as-skitter} & \mc{1}{r}{26584} & \mc{1}{r}{25.82} & \mc{1}{r|}{-} & \mc{1}{r}{8585} & \mc{1}{r}{36.69} & \mc{1}{r|}{-} & \mc{1}{r}{3426} & \mc{1}{r}{4.75} & \mc{1}{r|}{-} & \mc{1}{r}{2782} & \mc{1}{r}{5.50} & \mc{1}{r|}{-} & \mc{1}{r}{2343} & \mc{1}{r}{6.80} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{ca-AstroPh} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{ca-CondMat} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{ca-GrQc} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{ca-HepPh} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{ca-HepTh} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{email-Enron} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{email-EuAll} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.17} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{0.16} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.08}} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{0.13} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.10} \\  

  \mc{1}{l|}{p2p-Gnutella04} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella05} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella06} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella08} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{p2p-Gnutella09} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella24} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella25} & \mc{1}{r}{10} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{p2p-Gnutella30} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{p2p-Gnutella31} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.05} & \mc{1}{r|}{0.06} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r}{0.05} \\  

  \mc{1}{l|}{roadNet-CA} & \mc{1}{r}{234433} & \mc{1}{r}{3.96} & \mc{1}{r|}{-} & \mc{1}{r}{66406} & \mc{1}{r}{20.51} & \mc{1}{r|}{437.62} & \mc{1}{r}{478} & \mc{1}{r}{2.14} & \mc{1}{r|}{5.70} & \mc{1}{r}{0} & \mc{1}{r}{2.42} & \mc{1}{r|}{\textbf{3.57}} & \mc{1}{r}{0} & \mc{1}{r}{2.59} & \mc{1}{r}{3.07} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{133814} & \mc{1}{r}{2.43} & \mc{1}{r|}{-} & \mc{1}{r}{35442} & \mc{1}{r}{7.73} & \mc{1}{r|}{23.86} & \mc{1}{r}{300} & \mc{1}{r}{1.05} & \mc{1}{r|}{2.24} & \mc{1}{r}{0} & \mc{1}{r}{1.19} & \mc{1}{r|}{\textbf{1.44}} & \mc{1}{r}{0} & \mc{1}{r}{1.14} & \mc{1}{r}{1.40} \\  

  \mc{1}{l|}{roadNet-TX} & \mc{1}{r}{153985} & \mc{1}{r}{2.65} & \mc{1}{r|}{-} & \mc{1}{r}{40350} & \mc{1}{r}{10.49} & \mc{1}{r|}{24.30} & \mc{1}{r}{882} & \mc{1}{r}{1.23} & \mc{1}{r|}{3.98} & \mc{1}{r}{0} & \mc{1}{r}{1.32} & \mc{1}{r|}{\textbf{1.64}} & \mc{1}{r}{0} & \mc{1}{r}{1.34} & \mc{1}{r}{1.65} \\  

  \mc{1}{l|}{soc-Epinions1} & \mc{1}{r}{7} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.08} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.10} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.08} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.08} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r}{60041} & \mc{1}{r}{236.88} & \mc{1}{r|}{-} & \mc{1}{r}{29508} & \mc{1}{r}{213.74} & \mc{1}{r|}{-} & \mc{1}{r}{4319} & \mc{1}{r}{22.27} & \mc{1}{r|}{-} & \mc{1}{r}{3530} & \mc{1}{r}{24.13} & \mc{1}{r|}{-} & \mc{1}{r}{1314} & \mc{1}{r}{37.77} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{soc-Slashdot0811} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.11} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.11} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.08}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.09} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{soc-Slashdot0902} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.10} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{0.11} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.10} & \mc{1}{r}{0} & \mc{1}{r}{0.10} & \mc{1}{r}{0.12} \\  

  \mc{1}{l|}{soc-pokec-relationships} & \mc{1}{r}{926346} & \mc{1}{r}{299.11} & \mc{1}{r|}{-} & \mc{1}{r}{898779} & \mc{1}{r}{1013.39} & \mc{1}{r|}{-} & \mc{1}{r}{808542} & \mc{1}{r}{188.57} & \mc{1}{r|}{-} & \mc{1}{r}{807412} & \mc{1}{r}{217.83} & \mc{1}{r|}{-} & \mc{1}{r}{807395} & \mc{1}{r}{388.57} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{web-BerkStan} & \mc{1}{r}{36637} & \mc{1}{r}{6.58} & \mc{1}{r|}{-} & \mc{1}{r}{16661} & \mc{1}{r}{8.70} & \mc{1}{r|}{-} & \mc{1}{r}{1999} & \mc{1}{r}{6.86} & \mc{1}{r|}{120.05} & \mc{1}{r}{151} & \mc{1}{r}{6.46} & \mc{1}{r|}{\textbf{6.83}} & \mc{1}{r}{151} & \mc{1}{r}{7.89} & \mc{1}{r}{8.25} \\  

  \mc{1}{l|}{web-Google} & \mc{1}{r}{2810} & \mc{1}{r}{1.57} & \mc{1}{r|}{\textbf{2.40}} & \mc{1}{r}{1254} & \mc{1}{r}{2.42} & \mc{1}{r|}{3.66} & \mc{1}{r}{361} & \mc{1}{r}{1.75} & \mc{1}{r|}{2.95} & \mc{1}{r}{46} & \mc{1}{r}{1.88} & \mc{1}{r|}{2.47} & \mc{1}{r}{46} & \mc{1}{r}{7.97} & \mc{1}{r}{9.24} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{13464} & \mc{1}{r}{1.03} & \mc{1}{r|}{-} & \mc{1}{r}{6052} & \mc{1}{r}{2.03} & \mc{1}{r|}{-} & \mc{1}{r}{2460} & \mc{1}{r}{0.40} & \mc{1}{r|}{-} & \mc{1}{r}{2061} & \mc{1}{r}{0.56} & \mc{1}{r|}{\textbf{1.60}} & \mc{1}{r}{117} & \mc{1}{r}{2.44} & \mc{1}{r}{2.57} \\  

  \mc{1}{l|}{web-Stanford} & \mc{1}{r}{14153} & \mc{1}{r}{1.81} & \mc{1}{r|}{-} & \mc{1}{r}{3325} & \mc{1}{r}{2.45} & \mc{1}{r|}{-} & \mc{1}{r}{112} & \mc{1}{r}{2.25} & \mc{1}{r|}{2.50} & \mc{1}{r}{0} & \mc{1}{r}{1.80} & \mc{1}{r|}{\textbf{1.99}} & \mc{1}{r}{0} & \mc{1}{r}{2.17} & \mc{1}{r}{2.38} \\  

  \mc{1}{l|}{wiki-Talk} & \mc{1}{r}{0} & \mc{1}{r}{1.00} & \mc{1}{r|}{\textbf{1.71}} & \mc{1}{r}{0} & \mc{1}{r}{1.32} & \mc{1}{r|}{1.96} & \mc{1}{r}{0} & \mc{1}{r}{1.26} & \mc{1}{r|}{1.84} & \mc{1}{r}{0} & \mc{1}{r}{1.24} & \mc{1}{r|}{1.80} & \mc{1}{r}{0} & \mc{1}{r}{1.67} & \mc{1}{r}{2.28} \\  

  \mc{1}{l|}{wiki-Vote} & \mc{1}{r}{477} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.12} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r}{0.02} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_graph_tables/bnr_time_table_fe.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}
  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  
  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  
  \mc{1}{l|}{fe\_4elt2} & \mc{1}{r}{8580} & \mc{1}{r}{0.29} & \mc{1}{r|}{-} & \mc{1}{r}{8578} & \mc{1}{r}{0.87} & \mc{1}{r|}{-} & \mc{1}{r}{562} & \mc{1}{r}{0.10} & \mc{1}{r|}{-} & \mc{1}{r}{0} & \mc{1}{r}{0.12} & \mc{1}{r|}{\textbf{0.13}} & \mc{1}{r}{0} & \mc{1}{r}{0.16} & \mc{1}{r}{0.17} \\  
  \mc{1}{l|}{fe\_body} & \mc{1}{r}{16107} & \mc{1}{r}{0.69} & \mc{1}{r|}{-} & \mc{1}{r}{15992} & \mc{1}{r}{3.40} & \mc{1}{r|}{-} & \mc{1}{r}{1162} & \mc{1}{r}{0.16} & \mc{1}{r|}{-} & \mc{1}{r}{625} & \mc{1}{r}{0.44} & \mc{1}{r|}{-} & \mc{1}{r}{553} & \mc{1}{r}{0.94} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_ocean} & \mc{1}{r}{141283} & \mc{1}{r}{1.05} & \mc{1}{r|}{-} & \mc{1}{r}{0} & \mc{1}{r}{5.94} & \mc{1}{r|}{\textbf{5.99}} & \mc{1}{r}{138338} & \mc{1}{r}{8.90} & \mc{1}{r|}{-} & \mc{1}{r}{138134} & \mc{1}{r}{9.61} & \mc{1}{r|}{-} & \mc{1}{r}{138049} & \mc{1}{r}{10.78} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_pwt} & \mc{1}{r}{34521} & \mc{1}{r}{0.46} & \mc{1}{r|}{-} & \mc{1}{r}{34521} & \mc{1}{r}{2.70} & \mc{1}{r|}{-} & \mc{1}{r}{25550} & \mc{1}{r}{0.78} & \mc{1}{r|}{-} & \mc{1}{r}{20241} & \mc{1}{r}{1.80} & \mc{1}{r|}{-} & \mc{1}{r}{14107} & \mc{1}{r}{5.65} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_rotor} & \mc{1}{r}{98271} & \mc{1}{r}{9.80} & \mc{1}{r|}{-} & \mc{1}{r}{98271} & \mc{1}{r}{24.47} & \mc{1}{r|}{-} & \mc{1}{r}{91946} & \mc{1}{r}{4.80} & \mc{1}{r|}{-} & \mc{1}{r}{91634} & \mc{1}{r}{4.82} & \mc{1}{r|}{-} & \mc{1}{r}{89647} & \mc{1}{r}{11.11} & \mc{1}{r}{-} \\  
  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{15269} & \mc{1}{r}{0.21} & \mc{1}{r|}{-} & \mc{1}{r}{15269} & \mc{1}{r}{1.47} & \mc{1}{r|}{-} & \mc{1}{r}{2961} & \mc{1}{r}{0.34} & \mc{1}{r|}{-} & \mc{1}{r}{147} & \mc{1}{r}{0.62} & \mc{1}{r|}{\textbf{0.83}} & \mc{1}{r}{0} & \mc{1}{r}{0.75} & \mc{1}{r}{0.77} \\  
  \mc{1}{l|}{fe\_tooth} & \mc{1}{r}{10922} & \mc{1}{r}{1.69} & \mc{1}{r|}{-} & \mc{1}{r}{10801} & \mc{1}{r}{3.79} & \mc{1}{r|}{-} & \mc{1}{r}{15} & \mc{1}{r}{0.41} & \mc{1}{r|}{0.46} & \mc{1}{r}{0} & \mc{1}{r}{0.30} & \mc{1}{r|}{\textbf{0.34}} & \mc{1}{r}{0} & \mc{1}{r}{0.28} & \mc{1}{r}{0.32} \\  
\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_graph_tables/bnr_time_table_mesh.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{beethoven} & \mc{1}{r}{1254} & \mc{1}{r}{0.02} & \mc{1}{r|}{7.86} & \mc{1}{r}{427} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.08} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{blob} & \mc{1}{r}{5746} & \mc{1}{r}{0.08} & \mc{1}{r|}{-} & \mc{1}{r}{1464} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.20} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r}{380315} & \mc{1}{r}{5.56} & \mc{1}{r|}{-} & \mc{1}{r}{107265} & \mc{1}{r}{26.19} & \mc{1}{r|}{67.85} & \mc{1}{r}{86} & \mc{1}{r}{1.83} & \mc{1}{r|}{2.74} & \mc{1}{r}{0} & \mc{1}{r}{1.87} & \mc{1}{r|}{\textbf{2.26}} & \mc{1}{r}{0} & \mc{1}{r}{1.91} & \mc{1}{r}{2.39} \\  

  \mc{1}{l|}{bunny} & \mc{1}{r}{24580} & \mc{1}{r}{0.34} & \mc{1}{r|}{-} & \mc{1}{r}{3290} & \mc{1}{r}{0.56} & \mc{1}{r|}{0.89} & \mc{1}{r}{0} & \mc{1}{r}{0.12} & \mc{1}{r|}{\textbf{0.14}} & \mc{1}{r}{0} & \mc{1}{r}{0.13} & \mc{1}{r|}{0.16} & \mc{1}{r}{0} & \mc{1}{r}{0.15} & \mc{1}{r}{0.18} \\  

  \mc{1}{l|}{cow} & \mc{1}{r}{1916} & \mc{1}{r}{0.02} & \mc{1}{r|}{-} & \mc{1}{r}{513} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.06} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{dragon} & \mc{1}{r}{51885} & \mc{1}{r}{0.89} & \mc{1}{r|}{-} & \mc{1}{r}{12893} & \mc{1}{r}{1.34} & \mc{1}{r|}{3.83} & \mc{1}{r}{0} & \mc{1}{r}{0.18} & \mc{1}{r|}{\textbf{0.21}} & \mc{1}{r}{0} & \mc{1}{r}{0.19} & \mc{1}{r|}{0.23} & \mc{1}{r}{0} & \mc{1}{r}{0.21} & \mc{1}{r}{0.25} \\  

  \mc{1}{l|}{dragonsub} & \mc{1}{r}{218779} & \mc{1}{r}{2.60} & \mc{1}{r|}{-} & \mc{1}{r}{19470} & \mc{1}{r}{4.15} & \mc{1}{r|}{5.66} & \mc{1}{r}{506} & \mc{1}{r}{1.03} & \mc{1}{r|}{2.08} & \mc{1}{r}{0} & \mc{1}{r}{1.13} & \mc{1}{r|}{\textbf{1.36}} & \mc{1}{r}{0} & \mc{1}{r}{1.07} & \mc{1}{r}{1.28} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r}{239787} & \mc{1}{r}{4.07} & \mc{1}{r|}{-} & \mc{1}{r}{26270} & \mc{1}{r}{10.09} & \mc{1}{r|}{12.93} & \mc{1}{r}{274} & \mc{1}{r}{2.12} & \mc{1}{r|}{3.16} & \mc{1}{r}{0} & \mc{1}{r}{2.12} & \mc{1}{r|}{\textbf{2.51}} & \mc{1}{r}{0} & \mc{1}{r}{2.14} & \mc{1}{r}{2.56} \\  

  \mc{1}{l|}{face} & \mc{1}{r}{7588} & \mc{1}{r}{0.09} & \mc{1}{r|}{-} & \mc{1}{r}{1540} & \mc{1}{r}{0.10} & \mc{1}{r|}{0.21} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.04} \\  

  \mc{1}{l|}{fandisk} & \mc{1}{r}{2851} & \mc{1}{r}{0.05} & \mc{1}{r|}{-} & \mc{1}{r}{336} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.07} & \mc{1}{r}{51} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{feline} & \mc{1}{r}{14817} & \mc{1}{r}{0.20} & \mc{1}{r|}{-} & \mc{1}{r}{2743} & \mc{1}{r}{0.25} & \mc{1}{r|}{0.47} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.09} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r}{0.09} \\  

  \mc{1}{l|}{gameguy} & \mc{1}{r}{13959} & \mc{1}{r}{0.17} & \mc{1}{r|}{-} & \mc{1}{r}{312} & \mc{1}{r}{0.10} & \mc{1}{r|}{0.12} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{gargoyle} & \mc{1}{r}{6512} & \mc{1}{r}{0.15} & \mc{1}{r|}{-} & \mc{1}{r}{1819} & \mc{1}{r}{0.14} & \mc{1}{r|}{0.36} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{turtle} & \mc{1}{r}{91624} & \mc{1}{r}{1.17} & \mc{1}{r|}{-} & \mc{1}{r}{16095} & \mc{1}{r}{1.92} & \mc{1}{r|}{4.98} & \mc{1}{r}{186} & \mc{1}{r}{0.42} & \mc{1}{r|}{0.65} & \mc{1}{r}{0} & \mc{1}{r}{0.41} & \mc{1}{r|}{\textbf{0.49}} & \mc{1}{r}{0} & \mc{1}{r}{0.47} & \mc{1}{r}{0.56} \\  

  \mc{1}{l|}{venus} & \mc{1}{r}{1898} & \mc{1}{r}{0.02} & \mc{1}{r|}{-} & \mc{1}{r}{175} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_graph_tables/bnr_time_table_osm.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{alabama-AM2} & \mc{1}{r}{173} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.31} & \mc{1}{r}{173} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.55} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{alabama-AM3} & \mc{1}{r}{1614} & \mc{1}{r}{12.05} & \mc{1}{r|}{-} & \mc{1}{r}{1614} & \mc{1}{r}{14.37} & \mc{1}{r|}{-} & \mc{1}{r}{1288} & \mc{1}{r}{0.34} & \mc{1}{r|}{-} & \mc{1}{r}{456} & \mc{1}{r}{1.45} & \mc{1}{r|}{\textbf{3.94}} & \mc{1}{r}{0} & \mc{1}{r}{33.11} & \mc{1}{r}{33.16} \\  

  \mc{1}{l|}{district-of-columbia-AM1} & \mc{1}{r}{800} & \mc{1}{r}{1.22} & \mc{1}{r|}{-} & \mc{1}{r}{800} & \mc{1}{r}{1.28} & \mc{1}{r|}{-} & \mc{1}{r}{367} & \mc{1}{r}{0.03} & \mc{1}{r|}{39.81} & \mc{1}{r}{185} & \mc{1}{r}{0.41} & \mc{1}{r|}{\textbf{0.80}} & \mc{1}{r}{0} & \mc{1}{r}{3.65} & \mc{1}{r}{3.66} \\  

  \mc{1}{l|}{district-of-columbia-AM2} & \mc{1}{r}{6360} & \mc{1}{r}{11.86} & \mc{1}{r|}{-} & \mc{1}{r}{6360} & \mc{1}{r}{14.39} & \mc{1}{r|}{-} & \mc{1}{r}{5606} & \mc{1}{r}{0.85} & \mc{1}{r|}{-} & \mc{1}{r}{1855} & \mc{1}{r}{2.51} & \mc{1}{r|}{-} & \mc{1}{r}{1484} & \mc{1}{r}{84.91} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{district-of-columbia-AM3} & \mc{1}{r}{33367} & \mc{1}{r}{63.23} & \mc{1}{r|}{-} & \mc{1}{r}{33367} & \mc{1}{r}{358.14} & \mc{1}{r|}{-} & \mc{1}{r}{32320} & \mc{1}{r}{33.68} & \mc{1}{r|}{-} & \mc{1}{r}{28842} & \mc{1}{r}{66.67} & \mc{1}{r|}{-} & \mc{1}{r}{25031} & \mc{1}{r}{441.44} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{florida-AM2} & \mc{1}{r}{41} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{41} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{florida-AM3} & \mc{1}{r}{1069} & \mc{1}{r}{31.52} & \mc{1}{r|}{45.81} & \mc{1}{r}{1069} & \mc{1}{r}{35.20} & \mc{1}{r|}{-} & \mc{1}{r}{814} & \mc{1}{r}{0.13} & \mc{1}{r|}{3.85} & \mc{1}{r}{661} & \mc{1}{r}{0.44} & \mc{1}{r|}{\textbf{2.93}} & \mc{1}{r}{267} & \mc{1}{r}{42.26} & \mc{1}{r}{45.05} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{861} & \mc{1}{r}{8.99} & \mc{1}{r|}{892.17} & \mc{1}{r}{861} & \mc{1}{r}{10.14} & \mc{1}{r|}{-} & \mc{1}{r}{796} & \mc{1}{r}{0.08} & \mc{1}{r|}{25.97} & \mc{1}{r}{587} & \mc{1}{r}{0.69} & \mc{1}{r|}{\textbf{10.35}} & \mc{1}{r}{425} & \mc{1}{r}{12.84} & \mc{1}{r}{32.53} \\  

  \mc{1}{l|}{greenland-AM3} & \mc{1}{r}{3942} & \mc{1}{r}{3.81} & \mc{1}{r|}{-} & \mc{1}{r}{3942} & \mc{1}{r}{24.77} & \mc{1}{r|}{-} & \mc{1}{r}{3953} & \mc{1}{r}{3.94} & \mc{1}{r|}{-} & \mc{1}{r}{3339} & \mc{1}{r}{10.27} & \mc{1}{r|}{-} & \mc{1}{r}{3339} & \mc{1}{r}{54.44} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{hawaii-AM2} & \mc{1}{r}{428} & \mc{1}{r}{2.08} & \mc{1}{r|}{4.27} & \mc{1}{r}{428} & \mc{1}{r}{2.15} & \mc{1}{r|}{10.22} & \mc{1}{r}{262} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.18} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.10} & \mc{1}{r}{0.10} \\  

  \mc{1}{l|}{hawaii-AM3} & \mc{1}{r}{24436} & \mc{1}{r}{70.38} & \mc{1}{r|}{-} & \mc{1}{r}{24436} & \mc{1}{r}{743.04} & \mc{1}{r|}{-} & \mc{1}{r}{24184} & \mc{1}{r}{98.22} & \mc{1}{r|}{-} & \mc{1}{r}{22997} & \mc{1}{r}{118.52} & \mc{1}{r|}{-} & \mc{1}{r}{21087} & \mc{1}{r}{632.02} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{idaho-AM3} & \mc{1}{r}{3208} & \mc{1}{r}{3.17} & \mc{1}{r|}{-} & \mc{1}{r}{3208} & \mc{1}{r}{29.91} & \mc{1}{r|}{-} & \mc{1}{r}{3204} & \mc{1}{r}{6.96} & \mc{1}{r|}{-} & \mc{1}{r}{3160} & \mc{1}{r}{8.74} & \mc{1}{r|}{-} & \mc{1}{r}{2909} & \mc{1}{r}{33.77} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{kansas-AM3} & \mc{1}{r}{1605} & \mc{1}{r}{2.46} & \mc{1}{r|}{-} & \mc{1}{r}{1605} & \mc{1}{r}{4.81} & \mc{1}{r|}{-} & \mc{1}{r}{1550} & \mc{1}{r}{0.49} & \mc{1}{r|}{-} & \mc{1}{r}{903} & \mc{1}{r}{2.46} & \mc{1}{r|}{\textbf{430.93}} & \mc{1}{r}{860} & \mc{1}{r}{41.61} & \mc{1}{r}{489.15} \\  

  \mc{1}{l|}{kentucky-AM2} & \mc{1}{r}{442} & \mc{1}{r}{2.05} & \mc{1}{r|}{11.85} & \mc{1}{r}{442} & \mc{1}{r}{2.19} & \mc{1}{r|}{67.28} & \mc{1}{r}{183} & \mc{1}{r}{0.20} & \mc{1}{r|}{0.39} & \mc{1}{r}{0} & \mc{1}{r}{0.22} & \mc{1}{r|}{\textbf{0.23}} & \mc{1}{r}{0} & \mc{1}{r}{0.41} & \mc{1}{r}{0.42} \\  

  \mc{1}{l|}{kentucky-AM3} & \mc{1}{r}{16871} & \mc{1}{r}{109.47} & \mc{1}{r|}{-} & \mc{1}{r}{16871} & \mc{1}{r}{3344.67} & \mc{1}{r|}{-} & \mc{1}{r}{16807} & \mc{1}{r}{237.86} & \mc{1}{r|}{-} & \mc{1}{r}{15947} & \mc{1}{r}{298.49} & \mc{1}{r|}{-} & \mc{1}{r}{15684} & \mc{1}{r}{705.46} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{louisiana-AM3} & \mc{1}{r}{382} & \mc{1}{r}{4.56} & \mc{1}{r|}{6.55} & \mc{1}{r}{382} & \mc{1}{r}{5.04} & \mc{1}{r|}{25.22} & \mc{1}{r}{349} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.82} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.16} & \mc{1}{r}{0.16} \\  

  \mc{1}{l|}{maryland-AM3} & \mc{1}{r}{187} & \mc{1}{r}{7.59} & \mc{1}{r|}{8.49} & \mc{1}{r}{187} & \mc{1}{r}{8.65} & \mc{1}{r|}{10.73} & \mc{1}{r}{335} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.19} & \mc{1}{r}{0} & \mc{1}{r}{0.11} & \mc{1}{r|}{\textbf{0.11}} & \mc{1}{r}{0} & \mc{1}{r}{0.15} & \mc{1}{r}{0.15} \\  

  \mc{1}{l|}{massachusetts-AM2} & \mc{1}{r}{196} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.36} & \mc{1}{r}{196} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.58} & \mc{1}{r}{193} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.06}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{massachusetts-AM3} & \mc{1}{r}{2008} & \mc{1}{r}{9.42} & \mc{1}{r|}{-} & \mc{1}{r}{2008} & \mc{1}{r}{12.62} & \mc{1}{r|}{-} & \mc{1}{r}{1928} & \mc{1}{r}{0.36} & \mc{1}{r|}{-} & \mc{1}{r}{1636} & \mc{1}{r}{1.08} & \mc{1}{r|}{-} & \mc{1}{r}{1632} & \mc{1}{r}{31.83} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{mexico-AM3} & \mc{1}{r}{620} & \mc{1}{r}{25.29} & \mc{1}{r|}{80.23} & \mc{1}{r}{620} & \mc{1}{r}{27.52} & \mc{1}{r|}{991.99} & \mc{1}{r}{514} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{1.47}} & \mc{1}{r}{483} & \mc{1}{r}{0.28} & \mc{1}{r|}{1.50} & \mc{1}{r}{0} & \mc{1}{r}{21.03} & \mc{1}{r}{21.30} \\  

  \mc{1}{l|}{new-hampshire-AM3} & \mc{1}{r}{247} & \mc{1}{r}{4.99} & \mc{1}{r|}{6.19} & \mc{1}{r}{247} & \mc{1}{r}{5.69} & \mc{1}{r|}{15.89} & \mc{1}{r}{164} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.17} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r}{0.09} \\  

  \mc{1}{l|}{north-carolina-AM3} & \mc{1}{r}{1178} & \mc{1}{r}{0.69} & \mc{1}{r|}{-} & \mc{1}{r}{1178} & \mc{1}{r}{1.22} & \mc{1}{r|}{-} & \mc{1}{r}{1146} & \mc{1}{r}{0.25} & \mc{1}{r|}{-} & \mc{1}{r}{1144} & \mc{1}{r}{0.43} & \mc{1}{r|}{-} & \mc{1}{r}{700} & \mc{1}{r}{47.38} & \mc{1}{r}{379.088} \\  

  \mc{1}{l|}{oregon-AM2} & \mc{1}{r}{35} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.05} & \mc{1}{r}{35} & \mc{1}{r}{0.05} & \mc{1}{r|}{0.05} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{oregon-AM3} & \mc{1}{r}{3670} & \mc{1}{r}{9.95} & \mc{1}{r|}{-} & \mc{1}{r}{3670} & \mc{1}{r}{34.95} & \mc{1}{r|}{-} & \mc{1}{r}{3584} & \mc{1}{r}{3.92} & \mc{1}{r|}{-} & \mc{1}{r}{3417} & \mc{1}{r}{6.21} & \mc{1}{r|}{-} & \mc{1}{r}{2721} & \mc{1}{r}{38.72} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{pennsylvania-AM3} & \mc{1}{r}{315} & \mc{1}{r}{16.69} & \mc{1}{r|}{20.71} & \mc{1}{r}{315} & \mc{1}{r}{19.39} & \mc{1}{r|}{113.87} & \mc{1}{r}{317} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.39} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.12} & \mc{1}{r}{0.12} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r}{1103} & \mc{1}{r}{0.55} & \mc{1}{r|}{-} & \mc{1}{r}{1103} & \mc{1}{r}{0.68} & \mc{1}{r|}{-} & \mc{1}{r}{845} & \mc{1}{r}{0.17} & \mc{1}{r|}{163.07} & \mc{1}{r}{0} & \mc{1}{r}{0.53} & \mc{1}{r|}{\textbf{0.53}} & \mc{1}{r}{0} & \mc{1}{r}{4.57} & \mc{1}{r}{4.58} \\  

  \mc{1}{l|}{rhode-island-AM3} & \mc{1}{r}{13031} & \mc{1}{r}{7.75} & \mc{1}{r|}{-} & \mc{1}{r}{13031} & \mc{1}{r}{193.76} & \mc{1}{r|}{-} & \mc{1}{r}{12934} & \mc{1}{r}{26.54} & \mc{1}{r|}{-} & \mc{1}{r}{12653} & \mc{1}{r}{29.75} & \mc{1}{r|}{-} & \mc{1}{r}{12653} & \mc{1}{r}{59.69} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{utah-AM3} & \mc{1}{r}{568} & \mc{1}{r}{8.21} & \mc{1}{r|}{51.91} & \mc{1}{r}{568} & \mc{1}{r}{8.97} & \mc{1}{r|}{276.27} & \mc{1}{r}{396} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.87} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.40} & \mc{1}{r}{0.41} \\  

  \mc{1}{l|}{vermont-AM3} & \mc{1}{r}{2630} & \mc{1}{r}{4.79} & \mc{1}{r|}{-} & \mc{1}{r}{2630} & \mc{1}{r}{9.82} & \mc{1}{r|}{-} & \mc{1}{r}{2289} & \mc{1}{r}{0.97} & \mc{1}{r|}{-} & \mc{1}{r}{2069} & \mc{1}{r}{1.37} & \mc{1}{r|}{-} & \mc{1}{r}{2045} & \mc{1}{r}{55.28} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{virginia-AM2} & \mc{1}{r}{237} & \mc{1}{r}{0.13} & \mc{1}{r|}{0.61} & \mc{1}{r}{237} & \mc{1}{r}{0.12} & \mc{1}{r|}{0.99} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{virginia-AM3} & \mc{1}{r}{3867} & \mc{1}{r}{34.13} & \mc{1}{r|}{-} & \mc{1}{r}{3867} & \mc{1}{r}{39.74} & \mc{1}{r|}{-} & \mc{1}{r}{3738} & \mc{1}{r}{0.40} & \mc{1}{r|}{-} & \mc{1}{r}{2827} & \mc{1}{r}{1.28} & \mc{1}{r|}{-} & \mc{1}{r}{2547} & \mc{1}{r}{81.67} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{washington-AM2} & \mc{1}{r}{382} & \mc{1}{r}{0.24} & \mc{1}{r|}{5.31} & \mc{1}{r}{382} & \mc{1}{r}{0.18} & \mc{1}{r|}{8.58} & \mc{1}{r}{171} & \mc{1}{r}{0.05} & \mc{1}{r|}{0.37} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.06}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{washington-AM3} & \mc{1}{r}{8030} & \mc{1}{r}{50.21} & \mc{1}{r|}{-} & \mc{1}{r}{8030} & \mc{1}{r}{67.00} & \mc{1}{r|}{-} & \mc{1}{r}{7649} & \mc{1}{r}{2.19} & \mc{1}{r|}{-} & \mc{1}{r}{6895} & \mc{1}{r}{3.12} & \mc{1}{r|}{-} & \mc{1}{r}{6159} & \mc{1}{r}{73.52} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{west-virginia-AM3} & \mc{1}{r}{991} & \mc{1}{r}{10.69} & \mc{1}{r|}{-} & \mc{1}{r}{991} & \mc{1}{r}{12.13} & \mc{1}{r|}{-} & \mc{1}{r}{970} & \mc{1}{r}{0.08} & \mc{1}{r|}{238.39} & \mc{1}{r}{890} & \mc{1}{r}{0.33} & \mc{1}{r|}{\textbf{155.49}} & \mc{1}{r}{881} & \mc{1}{r}{38.73} & \mc{1}{r}{241.68} \\  

\end{tabu}
\end{ThreePartTable}


==> tables/bnr_time_graph_tables/bnr_time_table_snap.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\basicDense} & \mc{3}{c}{\basicSparse} & \mc{3}{c}{\nonIncreasing} & \mc{3}{c}{\cyclicFast} & \mc{3}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{as-skitter} & \mc{1}{r}{26584} & \mc{1}{r}{25.82} & \mc{1}{r|}{-} & \mc{1}{r}{8585} & \mc{1}{r}{36.69} & \mc{1}{r|}{-} & \mc{1}{r}{3426} & \mc{1}{r}{4.75} & \mc{1}{r|}{-} & \mc{1}{r}{2782} & \mc{1}{r}{5.50} & \mc{1}{r|}{-} & \mc{1}{r}{2343} & \mc{1}{r}{6.80} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{ca-AstroPh} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{ca-CondMat} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{ca-GrQc} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{ca-HepPh} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{ca-HepTh} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{email-Enron} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.04} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{email-EuAll} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.17} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{0.16} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{\textbf{0.08}} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{0.13} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.10} \\  

  \mc{1}{l|}{p2p-Gnutella04} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella05} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella06} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella08} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{p2p-Gnutella09} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0} & \mc{1}{r}{0.00} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella24} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella25} & \mc{1}{r}{10} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{p2p-Gnutella30} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.01} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{p2p-Gnutella31} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r|}{0.07} & \mc{1}{r}{0} & \mc{1}{r}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0} & \mc{1}{r}{0.05} & \mc{1}{r|}{0.06} & \mc{1}{r}{0} & \mc{1}{r}{0.04} & \mc{1}{r}{0.05} \\  

  \mc{1}{l|}{roadNet-CA} & \mc{1}{r}{234433} & \mc{1}{r}{3.96} & \mc{1}{r|}{-} & \mc{1}{r}{66406} & \mc{1}{r}{20.51} & \mc{1}{r|}{437.62} & \mc{1}{r}{478} & \mc{1}{r}{2.14} & \mc{1}{r|}{5.70} & \mc{1}{r}{0} & \mc{1}{r}{2.42} & \mc{1}{r|}{\textbf{3.57}} & \mc{1}{r}{0} & \mc{1}{r}{2.59} & \mc{1}{r}{3.07} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{133814} & \mc{1}{r}{2.43} & \mc{1}{r|}{-} & \mc{1}{r}{35442} & \mc{1}{r}{7.73} & \mc{1}{r|}{23.86} & \mc{1}{r}{300} & \mc{1}{r}{1.05} & \mc{1}{r|}{2.24} & \mc{1}{r}{0} & \mc{1}{r}{1.19} & \mc{1}{r|}{\textbf{1.44}} & \mc{1}{r}{0} & \mc{1}{r}{1.14} & \mc{1}{r}{1.40} \\  

  \mc{1}{l|}{roadNet-TX} & \mc{1}{r}{153985} & \mc{1}{r}{2.65} & \mc{1}{r|}{-} & \mc{1}{r}{40350} & \mc{1}{r}{10.49} & \mc{1}{r|}{24.30} & \mc{1}{r}{882} & \mc{1}{r}{1.23} & \mc{1}{r|}{3.98} & \mc{1}{r}{0} & \mc{1}{r}{1.32} & \mc{1}{r|}{\textbf{1.64}} & \mc{1}{r}{0} & \mc{1}{r}{1.34} & \mc{1}{r}{1.65} \\  

  \mc{1}{l|}{soc-Epinions1} & \mc{1}{r}{7} & \mc{1}{r}{0.05} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r|}{0.08} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.10} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.08} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r}{0.08} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r}{60041} & \mc{1}{r}{236.88} & \mc{1}{r|}{-} & \mc{1}{r}{29508} & \mc{1}{r}{213.74} & \mc{1}{r|}{-} & \mc{1}{r}{4319} & \mc{1}{r}{22.27} & \mc{1}{r|}{-} & \mc{1}{r}{3530} & \mc{1}{r}{24.13} & \mc{1}{r|}{-} & \mc{1}{r}{1314} & \mc{1}{r}{37.77} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{soc-Slashdot0811} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.11} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.11} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.08}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.09} & \mc{1}{r}{0} & \mc{1}{r}{0.06} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{soc-Slashdot0902} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0} & \mc{1}{r}{0.07} & \mc{1}{r|}{0.10} & \mc{1}{r}{0} & \mc{1}{r}{0.09} & \mc{1}{r|}{0.11} & \mc{1}{r}{0} & \mc{1}{r}{0.08} & \mc{1}{r|}{0.10} & \mc{1}{r}{0} & \mc{1}{r}{0.10} & \mc{1}{r}{0.12} \\  

  \mc{1}{l|}{soc-pokec-relationships} & \mc{1}{r}{926346} & \mc{1}{r}{299.11} & \mc{1}{r|}{-} & \mc{1}{r}{898779} & \mc{1}{r}{1013.39} & \mc{1}{r|}{-} & \mc{1}{r}{808542} & \mc{1}{r}{188.57} & \mc{1}{r|}{-} & \mc{1}{r}{807412} & \mc{1}{r}{217.83} & \mc{1}{r|}{-} & \mc{1}{r}{807395} & \mc{1}{r}{388.57} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{web-BerkStan} & \mc{1}{r}{36637} & \mc{1}{r}{6.58} & \mc{1}{r|}{-} & \mc{1}{r}{16661} & \mc{1}{r}{8.70} & \mc{1}{r|}{-} & \mc{1}{r}{1999} & \mc{1}{r}{6.86} & \mc{1}{r|}{120.05} & \mc{1}{r}{151} & \mc{1}{r}{6.46} & \mc{1}{r|}{\textbf{6.83}} & \mc{1}{r}{151} & \mc{1}{r}{7.89} & \mc{1}{r}{8.25} \\  

  \mc{1}{l|}{web-Google} & \mc{1}{r}{2810} & \mc{1}{r}{1.57} & \mc{1}{r|}{\textbf{2.40}} & \mc{1}{r}{1254} & \mc{1}{r}{2.42} & \mc{1}{r|}{3.66} & \mc{1}{r}{361} & \mc{1}{r}{1.75} & \mc{1}{r|}{2.95} & \mc{1}{r}{46} & \mc{1}{r}{1.88} & \mc{1}{r|}{2.47} & \mc{1}{r}{46} & \mc{1}{r}{7.97} & \mc{1}{r}{9.24} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{13464} & \mc{1}{r}{1.03} & \mc{1}{r|}{-} & \mc{1}{r}{6052} & \mc{1}{r}{2.03} & \mc{1}{r|}{-} & \mc{1}{r}{2460} & \mc{1}{r}{0.40} & \mc{1}{r|}{-} & \mc{1}{r}{2061} & \mc{1}{r}{0.56} & \mc{1}{r|}{\textbf{1.60}} & \mc{1}{r}{117} & \mc{1}{r}{2.44} & \mc{1}{r}{2.57} \\  

  \mc{1}{l|}{web-Stanford} & \mc{1}{r}{14153} & \mc{1}{r}{1.81} & \mc{1}{r|}{-} & \mc{1}{r}{3325} & \mc{1}{r}{2.45} & \mc{1}{r|}{-} & \mc{1}{r}{112} & \mc{1}{r}{2.25} & \mc{1}{r|}{2.50} & \mc{1}{r}{0} & \mc{1}{r}{1.80} & \mc{1}{r|}{\textbf{1.99}} & \mc{1}{r}{0} & \mc{1}{r}{2.17} & \mc{1}{r}{2.38} \\  

  \mc{1}{l|}{wiki-Talk} & \mc{1}{r}{0} & \mc{1}{r}{1.00} & \mc{1}{r|}{\textbf{1.71}} & \mc{1}{r}{0} & \mc{1}{r}{1.32} & \mc{1}{r|}{1.96} & \mc{1}{r}{0} & \mc{1}{r}{1.26} & \mc{1}{r|}{1.84} & \mc{1}{r}{0} & \mc{1}{r}{1.24} & \mc{1}{r|}{1.80} & \mc{1}{r}{0} & \mc{1}{r}{1.67} & \mc{1}{r}{2.28} \\  

  \mc{1}{l|}{wiki-Vote} & \mc{1}{r}{477} & \mc{1}{r}{0.03} & \mc{1}{r|}{0.12} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r}{0} & \mc{1}{r}{0.02} & \mc{1}{r}{0.02} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_tables/bnr_time_table.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccc}

  \mc{1}{l|}{Graph} & \mc{1}{r|}{$t_s$} & \mc{1}{r|}{$t_s$} & \mc{1}{r|}{$t_s$} & \mc{1}{r}{$t_s$} \\ 
  \hline  

  \mc{1}{l|}{OSM instances} & \mc{1}{c|}{Basic-Dense} & \mc{1}{c|}{NonIncreasing} & \mc{1}{c|}{Cyclic-Fast} & \mc{1}{c}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{district-of-columbia-AM1} & \mc{1}{r|}{-} & \mc{1}{r|}{39.81} & \mc{1}{r|}{\textbf{0.80}} & \mc{1}{r}{3.66} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r|}{892.17} & \mc{1}{r|}{25.97} & \mc{1}{r|}{\textbf{10.35}} & \mc{1}{r}{32.53} \\  

  \mc{1}{l|}{north-carolina-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{\textbf{379.09}} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r|}{-} & \mc{1}{r|}{163.07} & \mc{1}{r|}{\textbf{0.53}} & \mc{1}{r}{4.58} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{1}{r|}{47.1\% (16/34)} & \mc{1}{r|}{55.9\% (19/34)} & \mc{1}{r|}{61.8\% (21/34)} & \mc{1}{r}{64.7\% (22/34)} \\ 
  \hline \hline  

  \mc{1}{l|}{SNAP instances} & \mc{1}{r|}{Basic-Sparse} & \mc{1}{r|}{NonIncreasing} & \mc{1}{r|}{Cyclic-Fast} & \mc{1}{r}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{roadNet-TX} & \mc{1}{r|}{24.30} & \mc{1}{r|}{3.98} & \mc{1}{r|}{\textbf{1.64}} & \mc{1}{r}{1.65} \\  

  \mc{1}{l|}{web-BerkStan} & \mc{1}{r|}{-} & \mc{1}{r|}{120.05} & \mc{1}{r|}{\textbf{6.83}} & \mc{1}{r}{8.25} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{1.60}} & \mc{1}{r}{2.57} \\  

  \mc{1}{l|}{web-Stanford} & \mc{1}{r|}{-} & \mc{1}{r|}{2.50} & \mc{1}{r|}{\textbf{1.99}} & \mc{1}{r}{2.38} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{1}{r|}{80.6\% (25/31)} & \mc{1}{r|}{87.1\% (27/31)} & \mc{1}{r|}{90.3\% (28/31)} & \mc{1}{r}{90.3\% (28/31)} \\ 
  \hline \hline  

  \mc{1}{l|}{mesh instances} & \mc{1}{r|}{Basic-Sparse} & \mc{1}{r|}{NonIncreasing} & \mc{1}{r|}{Cyclic-Fast} & \mc{1}{r}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{buddha} & \mc{1}{r|}{67.85} & \mc{1}{r|}{2.74} & \mc{1}{r|}{\textbf{2.26}} & \mc{1}{r}{2.39} \\  

  \mc{1}{l|}{dragon} & \mc{1}{r|}{3.83} & \mc{1}{r|}{\textbf{0.21}} & \mc{1}{r|}{0.23} & \mc{1}{r}{0.25} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r|}{12.93} & \mc{1}{r|}{3.16} & \mc{1}{r|}{\textbf{2.51}} & \mc{1}{r}{2.56} \\  

  \mc{1}{l|}{turtle} & \mc{1}{r|}{4.98} & \mc{1}{r|}{0.65} & \mc{1}{r|}{\textbf{0.49}} & \mc{1}{r}{0.56} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{1}{r|}{100.0\% (15/15)} & \mc{1}{r|}{100.0\% (15/15)} & \mc{1}{r|}{100.0\% (15/15)} & \mc{1}{r}{100.0\% (15/15)} \\ 
  \hline \hline  

  \mc{1}{l|}{FE instances} & \mc{1}{r|}{Basic-Sparse} & \mc{1}{r|}{NonIncreasing} & \mc{1}{r|}{Cyclic-Fast} & \mc{1}{r}{Cyclic-Strong} \\ 
  \hline  

  \mc{1}{l|}{fe\_4elt2} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{0.13}} & \mc{1}{r}{0.17} \\  

  \mc{1}{l|}{fe\_ocean} & \mc{1}{r|}{\textbf{5.99}} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{0.83} & \mc{1}{r}{\textbf{0.77}} \\  

  \mc{1}{l|}{fe\_tooth} & \mc{1}{r|}{-} & \mc{1}{r|}{0.46} & \mc{1}{r|}{0.34} & \mc{1}{r}{\textbf{0.32}} \\ 
  \hline  

  \mc{1}{l|}{Solved instances} & \mc{1}{r|}{14.3\% (1/7)} & \mc{1}{r|}{14.3\% (1/7)} & \mc{1}{r|}{42.9\% (3/7)} & \mc{1}{r}{42.9\% (3/7)} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_tables/bnr_time_table_fe.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccc}

  \mc{1}{l|}{Graph} & \mc{1}{c}{\basicDense} & \mc{1}{c}{\basicSparse} & \mc{1}{c}{\nonIncreasing} & \mc{1}{c}{\cyclicFast} & \mc{1}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{fe\_4elt2} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{0.13}} & \mc{1}{r}{0.17} \\  

  \mc{1}{l|}{fe\_body} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{fe\_ocean} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{5.99}} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{fe\_pwt} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{fe\_rotor} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{0.83}} & \mc{1}{r}{0.77} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_tables/bnr_time_table_mesh.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccc}

  \mc{1}{l|}{Graph} & \mc{1}{c}{\basicDense} & \mc{1}{c}{\basicSparse} & \mc{1}{c}{\nonIncreasing} & \mc{1}{c}{\cyclicFast} & \mc{1}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{beethoven} & \mc{1}{r|}{7.86} & \mc{1}{r|}{0.08} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{blob} & \mc{1}{r|}{-} & \mc{1}{r|}{0.20} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r|}{0.04} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r|}{-} & \mc{1}{r|}{67.85} & \mc{1}{r|}{2.74} & \mc{1}{r|}{\textbf{2.26}} & \mc{1}{r}{2.39} \\  

  \mc{1}{l|}{bunny} & \mc{1}{r|}{-} & \mc{1}{r|}{0.89} & \mc{1}{r|}{\textbf{0.14}} & \mc{1}{r|}{0.16} & \mc{1}{r}{0.18} \\  

  \mc{1}{l|}{cow} & \mc{1}{r|}{-} & \mc{1}{r|}{0.06} & \mc{1}{r|}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{dragon} & \mc{1}{r|}{-} & \mc{1}{r|}{3.83} & \mc{1}{r|}{\textbf{0.21}} & \mc{1}{r|}{0.23} & \mc{1}{r}{0.25} \\  

  \mc{1}{l|}{dragonsub} & \mc{1}{r|}{-} & \mc{1}{r|}{5.66} & \mc{1}{r|}{2.08} & \mc{1}{r|}{\textbf{1.36}} & \mc{1}{r}{1.28} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r|}{-} & \mc{1}{r|}{12.93} & \mc{1}{r|}{3.16} & \mc{1}{r|}{\textbf{2.51}} & \mc{1}{r}{2.56} \\  

  \mc{1}{l|}{face} & \mc{1}{r|}{-} & \mc{1}{r|}{0.21} & \mc{1}{r|}{0.04} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0.04} \\  

  \mc{1}{l|}{fandisk} & \mc{1}{r|}{-} & \mc{1}{r|}{0.07} & \mc{1}{r|}{0.03} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{feline} & \mc{1}{r|}{-} & \mc{1}{r|}{0.47} & \mc{1}{r|}{0.09} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0.09} \\  

  \mc{1}{l|}{gameguy} & \mc{1}{r|}{-} & \mc{1}{r|}{0.12} & \mc{1}{r|}{0.07} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{gargoyle} & \mc{1}{r|}{-} & \mc{1}{r|}{0.36} & \mc{1}{r|}{0.03} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{turtle} & \mc{1}{r|}{-} & \mc{1}{r|}{4.98} & \mc{1}{r|}{0.65} & \mc{1}{r|}{\textbf{0.49}} & \mc{1}{r}{0.56} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_tables/bnr_time_table_osm.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccc}

  \mc{1}{l|}{Graph} & \mc{1}{c}{\basicDense} & \mc{1}{c}{\basicSparse} & \mc{1}{c}{\nonIncreasing} & \mc{1}{c}{\cyclicFast} & \mc{1}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{alabama-AM2} & \mc{1}{r|}{0.31} & \mc{1}{r|}{0.55} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{alabama-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{3.94}} & \mc{1}{r}{33.16} \\  

  \mc{1}{l|}{district-of-columbia-AM1} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{39.81} & \mc{1}{r|}{\textbf{0.80}} & \mc{1}{r}{3.66} \\  

  \mc{1}{l|}{district-of-columbia-AM2} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{district-of-columbia-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{florida-AM2} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{florida-AM3} & \mc{1}{r|}{45.81} & \mc{1}{r|}{-} & \mc{1}{r|}{3.85} & \mc{1}{r|}{\textbf{2.93}} & \mc{1}{r}{45.05} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r|}{892.17} & \mc{1}{r|}{-} & \mc{1}{r|}{25.97} & \mc{1}{r|}{\textbf{10.35}} & \mc{1}{r}{32.53} \\  

  \mc{1}{l|}{greenland-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{hawaii-AM2} & \mc{1}{r|}{4.27} & \mc{1}{r|}{10.22} & \mc{1}{r|}{0.18} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0.10} \\  

  \mc{1}{l|}{hawaii-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{idaho-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{kansas-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{430.93}} & \mc{1}{r}{489.15} \\  

  \mc{1}{l|}{kentucky-AM2} & \mc{1}{r|}{11.85} & \mc{1}{r|}{67.28} & \mc{1}{r|}{0.39} & \mc{1}{r|}{\textbf{0.23}} & \mc{1}{r}{0.42} \\  

  \mc{1}{l|}{kentucky-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{louisiana-AM3} & \mc{1}{r|}{6.55} & \mc{1}{r|}{25.22} & \mc{1}{r|}{0.82} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0.16} \\  

  \mc{1}{l|}{maryland-AM3} & \mc{1}{r|}{8.49} & \mc{1}{r|}{10.73} & \mc{1}{r|}{0.19} & \mc{1}{r|}{\textbf{0.11}} & \mc{1}{r}{0.15} \\  

  \mc{1}{l|}{massachusetts-AM2} & \mc{1}{r|}{0.36} & \mc{1}{r|}{0.58} & \mc{1}{r|}{0.07} & \mc{1}{r|}{\textbf{0.06}} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{massachusetts-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{mexico-AM3} & \mc{1}{r|}{80.23} & \mc{1}{r|}{991.99} & \mc{1}{r|}{\textbf{1.47}} & \mc{1}{r|}{1.50} & \mc{1}{r}{21.30} \\  

  \mc{1}{l|}{new-hampshire-AM3} & \mc{1}{r|}{6.19} & \mc{1}{r|}{15.89} & \mc{1}{r|}{0.17} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0.09} \\  

  \mc{1}{l|}{north-carolina-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{379.088} \\  

  \mc{1}{l|}{oregon-AM2} & \mc{1}{r|}{0.05} & \mc{1}{r|}{0.05} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.02} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{oregon-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{pennsylvania-AM3} & \mc{1}{r|}{20.71} & \mc{1}{r|}{113.87} & \mc{1}{r|}{0.39} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r}{0.12} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{163.07} & \mc{1}{r|}{\textbf{0.53}} & \mc{1}{r}{4.58} \\  

  \mc{1}{l|}{rhode-island-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{utah-AM3} & \mc{1}{r|}{51.91} & \mc{1}{r|}{276.27} & \mc{1}{r|}{0.87} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r}{0.41} \\  

  \mc{1}{l|}{vermont-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{virginia-AM2} & \mc{1}{r|}{0.61} & \mc{1}{r|}{0.99} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r|}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{virginia-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{washington-AM2} & \mc{1}{r|}{5.31} & \mc{1}{r|}{8.58} & \mc{1}{r|}{0.37} & \mc{1}{r|}{\textbf{0.06}} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{washington-AM3} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/bnr_time_tables/bnr_time_table_snap.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccc}

  \mc{1}{l|}{Graph} & \mc{1}{c}{\basicDense} & \mc{1}{c}{\basicSparse} & \mc{1}{c}{\nonIncreasing} & \mc{1}{c}{\cyclicFast} & \mc{1}{c}{\cyclicStrong} \\  

  \mc{1}{l|}{} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{as-skitter} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{ca-AstroPh} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r|}{0.03} & \mc{1}{r|}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{ca-CondMat} & \mc{1}{r|}{0.03} & \mc{1}{r|}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r|}{0.03} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{ca-GrQc} & \mc{1}{r|}{0.00} & \mc{1}{r|}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r|}{0.00} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{ca-HepPh} & \mc{1}{r|}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.02} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{ca-HepTh} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.01} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{email-Enron} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r|}{0.03} & \mc{1}{r|}{0.04} & \mc{1}{r|}{0.03} & \mc{1}{r}{0.03} \\  

  \mc{1}{l|}{email-EuAll} & \mc{1}{r|}{0.17} & \mc{1}{r|}{0.16} & \mc{1}{r|}{\textbf{0.08}} & \mc{1}{r|}{0.13} & \mc{1}{r}{0.10} \\  

  \mc{1}{l|}{p2p-Gnutella04} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella05} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella06} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.01} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella08} & \mc{1}{r|}{0.00} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.00} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0.00} \\  

  \mc{1}{l|}{p2p-Gnutella09} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{0.01} & \mc{1}{r|}{\textbf{0.00}} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella24} & \mc{1}{r|}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.02} & \mc{1}{r}{0.01} \\  

  \mc{1}{l|}{p2p-Gnutella25} & \mc{1}{r|}{0.02} & \mc{1}{r|}{0.02} & \mc{1}{r|}{\textbf{0.01}} & \mc{1}{r|}{0.02} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{p2p-Gnutella30} & \mc{1}{r|}{0.02} & \mc{1}{r|}{0.03} & \mc{1}{r|}{0.02} & \mc{1}{r|}{\textbf{0.02}} & \mc{1}{r}{0.02} \\  

  \mc{1}{l|}{p2p-Gnutella31} & \mc{1}{r|}{0.07} & \mc{1}{r|}{0.07} & \mc{1}{r|}{\textbf{0.03}} & \mc{1}{r|}{0.06} & \mc{1}{r}{0.05} \\  

  \mc{1}{l|}{roadNet-CA} & \mc{1}{r|}{-} & \mc{1}{r|}{437.62} & \mc{1}{r|}{5.70} & \mc{1}{r|}{\textbf{3.57}} & \mc{1}{r}{3.07} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r|}{-} & \mc{1}{r|}{23.86} & \mc{1}{r|}{2.24} & \mc{1}{r|}{\textbf{1.44}} & \mc{1}{r}{1.40} \\  

  \mc{1}{l|}{roadNet-TX} & \mc{1}{r|}{-} & \mc{1}{r|}{24.30} & \mc{1}{r|}{3.98} & \mc{1}{r|}{\textbf{1.64}} & \mc{1}{r}{1.65} \\  

  \mc{1}{l|}{soc-Epinions1} & \mc{1}{r|}{\textbf{0.07}} & \mc{1}{r|}{0.08} & \mc{1}{r|}{0.10} & \mc{1}{r|}{0.08} & \mc{1}{r}{0.08} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{soc-Slashdot0811} & \mc{1}{r|}{0.11} & \mc{1}{r|}{0.11} & \mc{1}{r|}{\textbf{0.08}} & \mc{1}{r|}{0.09} & \mc{1}{r}{0.07} \\  

  \mc{1}{l|}{soc-Slashdot0902} & \mc{1}{r|}{\textbf{0.09}} & \mc{1}{r|}{0.10} & \mc{1}{r|}{0.11} & \mc{1}{r|}{0.10} & \mc{1}{r}{0.12} \\  

  \mc{1}{l|}{soc-pokec-relationships} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{web-BerkStan} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{120.05} & \mc{1}{r|}{\textbf{6.83}} & \mc{1}{r}{8.25} \\  

  \mc{1}{l|}{web-Google} & \mc{1}{r|}{\textbf{2.40}} & \mc{1}{r|}{3.66} & \mc{1}{r|}{2.95} & \mc{1}{r|}{2.47} & \mc{1}{r}{9.24} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r|}{-} & \mc{1}{r|}{561.62} & \mc{1}{r|}{-} & \mc{1}{r|}{\textbf{1.60}} & \mc{1}{r}{2.57} \\  

  \mc{1}{l|}{web-Stanford} & \mc{1}{r|}{-} & \mc{1}{r|}{-} & \mc{1}{r|}{2.50} & \mc{1}{r|}{\textbf{1.99}} & \mc{1}{r}{2.38} \\  

  \mc{1}{l|}{wiki-Talk} & \mc{1}{r|}{\textbf{1.71}} & \mc{1}{r|}{1.96} & \mc{1}{r|}{1.84} & \mc{1}{r|}{1.80} & \mc{1}{r}{2.28} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/configuration_time_table.tex <==
\begin{ThreePartTable}
\begin{tabu}{cccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{3}{c}{\conFast} & \mc{3}{c}{\conStrong} & \mc{3}{c}{\conFull} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r|}{$t_{t}$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t_{r}$} & \mc{1}{r}{$t_{t}$} \\ 
  \hline  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{147} & \mc{1}{r}{0.71} & \mc{1}{r|}{0.92} & \mc{1}{r}{0} & \mc{1}{r}{0.70} & \mc{1}{r|}{\textbf{0.72}} & \mc{1}{r}{0} & \mc{1}{r}{0.69} & \mc{1}{r}{0.71} \\  

  \mc{1}{l|}{alabama-AM3} & \mc{1}{r}{456} & \mc{1}{r}{1.51} & \mc{1}{r|}{\textbf{4.03}} & \mc{1}{r}{0} & \mc{1}{r}{32.27} & \mc{1}{r|}{32.31} & \mc{1}{r}{0} & \mc{1}{r}{33.81} & \mc{1}{r}{33.85} \\  

  \mc{1}{l|}{florida-AM3} & \mc{1}{r}{661} & \mc{1}{r}{0.44} & \mc{1}{r|}{\textbf{2.85}} & \mc{1}{r}{267} & \mc{1}{r}{42.65} & \mc{1}{r|}{45.46} & \mc{1}{r}{267} & \mc{1}{r}{1057.72} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{587} & \mc{1}{r}{0.47} & \mc{1}{r|}{\textbf{10.49}} & \mc{1}{r}{425} & \mc{1}{r}{12.63} & \mc{1}{r|}{31.83} & \mc{1}{r}{425} & \mc{1}{r}{1054.47} & \mc{1}{r}{-} \\  

  \mc{1}{l|}{mexico-AM3} & \mc{1}{r}{483} & \mc{1}{r}{0.39} & \mc{1}{r|}{\textbf{1.75}} & \mc{1}{r}{0} & \mc{1}{r}{20.83} & \mc{1}{r|}{21.10} & \mc{1}{r}{0} & \mc{1}{r}{22.62} & \mc{1}{r}{22.89} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{0} & \mc{1}{r}{1.03} & \mc{1}{r|}{\textbf{1.27}} & \mc{1}{r}{0} & \mc{1}{r}{1.42} & \mc{1}{r|}{1.92} & \mc{1}{r}{0} & \mc{1}{r}{1.07} & \mc{1}{r}{1.33} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{2061} & \mc{1}{r}{0.58} & \mc{1}{r|}{\textbf{1.71}} & \mc{1}{r}{117} & \mc{1}{r}{2.44} & \mc{1}{r|}{2.59} & \mc{1}{r}{101} & \mc{1}{r}{1056.04} & \mc{1}{r}{-} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/integrated_struction_table.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccc}

  \mc{1}{l|}{\mr{3}{*}{Graph}} & \mc{2}{c}{NonIncreasing} & \mc{2}{c}{NonIncreasing} & \mc{2}{c}{NonIncreasing} & \mc{2}{c}{NonIncreasing} & \mc{2}{c}{NonIncreasing} \\  

  \mc{1}{l|}{} & \mc{2}{c}{[no struction]} & \mc{2}{c}{[orig. struction]} & \mc{2}{c}{[mod. struction]} & \mc{2}{c}{[ext. struction]} & \mc{2}{c}{[ext. red. struction]} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{fe\_body} & \mc{1}{r}{15992} & \mc{1}{r|}{0.88} & \mc{1}{r}{14018} & \mc{1}{r|}{0.86} & \mc{1}{r}{15333} & \mc{1}{r|}{1.51} & \mc{1}{r}{\textbf{1167}} & \mc{1}{r|}{0.82} & \mc{1}{r}{1206} & \mc{1}{r}{0.82} \\  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{15269} & \mc{1}{r|}{0.41} & \mc{1}{r}{15269} & \mc{1}{r|}{0.41} & \mc{1}{r}{15269} & \mc{1}{r|}{0.45} & \mc{1}{r}{\textbf{3540}} & \mc{1}{r|}{1.26} & \mc{1}{r}{3578} & \mc{1}{r}{1.38} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r}{107265} & \mc{1}{r|}{14.53} & \mc{1}{r}{71574} & \mc{1}{r|}{13.96} & \mc{1}{r}{227833} & \mc{1}{r|}{22.10} & \mc{1}{r}{\textbf{103}} & \mc{1}{r|}{8.89} & \mc{1}{r}{263} & \mc{1}{r}{8.73} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r}{26270} & \mc{1}{r|}{9.33} & \mc{1}{r}{17626} & \mc{1}{r|}{9.56} & \mc{1}{r}{121122} & \mc{1}{r|}{17.14} & \mc{1}{r}{\textbf{251}} & \mc{1}{r|}{7.55} & \mc{1}{r}{919} & \mc{1}{r}{7.83} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{861} & \mc{1}{r|}{3.13} & \mc{1}{r}{861} & \mc{1}{r|}{3.11} & \mc{1}{r}{860} & \mc{1}{r|}{2.97} & \mc{1}{r}{\textbf{780}} & \mc{1}{r|}{3.33} & \mc{1}{r}{781} & \mc{1}{r}{3.40} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r}{1103} & \mc{1}{r|}{0.51} & \mc{1}{r}{1100} & \mc{1}{r|}{0.64} & \mc{1}{r}{1098} & \mc{1}{r|}{0.53} & \mc{1}{r}{\textbf{853}} & \mc{1}{r|}{2.49} & \mc{1}{r}{901} & \mc{1}{r}{1.96} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{35442} & \mc{1}{r|}{3.83} & \mc{1}{r}{20572} & \mc{1}{r|}{4.10} & \mc{1}{r}{63621} & \mc{1}{r|}{6.93} & \mc{1}{r}{\textbf{282}} & \mc{1}{r|}{3.16} & \mc{1}{r}{377} & \mc{1}{r}{3.31} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r}{29419} & \mc{1}{r|}{98.37} & \mc{1}{r}{23107} & \mc{1}{r|}{127.25} & \mc{1}{r}{42270} & \mc{1}{r|}{118.01} & \mc{1}{r}{4319} & \mc{1}{r|}{153.87} & \mc{1}{r}{\textbf{4293}} & \mc{1}{r}{147.40} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{6052} & \mc{1}{r|}{1.49} & \mc{1}{r}{5511} & \mc{1}{r|}{1.54} & \mc{1}{r}{6348} & \mc{1}{r|}{1.39} & \mc{1}{r}{\textbf{516}} & \mc{1}{r|}{1.38} & \mc{1}{r}{544} & \mc{1}{r}{1.41} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/plain_struction_table.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccccc}

  \mc{1}{l|}{\mr{3}{*}{Graph}} & \mc{2}{c}{NonIncreasing} & \mc{2}{c}{Plain} & \mc{2}{c}{Plain} & \mc{2}{c}{Plain} & \mc{2}{c}{Plain} \\  

  \mc{1}{l|}{} & \mc{2}{c}{[no struction]} & \mc{2}{c}{orig. struction} & \mc{2}{c}{mod. struction} & \mc{2}{c}{ext. struction} & \mc{2}{c}{ext. red. struction} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{fe\_body} & \mc{1}{r}{15992} & \mc{1}{r|}{0.88} & \mc{1}{r}{44430} & \mc{1}{r|}{0.02} & \mc{1}{r}{44469} & \mc{1}{r|}{0.02} & \mc{1}{r}{\textbf{1437}} & \mc{1}{r|}{0.22} & \mc{1}{r}{1753} & \mc{1}{r}{0.32} \\  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{15269} & \mc{1}{r|}{0.41} & \mc{1}{r}{16386} & \mc{1}{r|}{0.01} & \mc{1}{r}{16386} & \mc{1}{r|}{0.01} & \mc{1}{r}{\textbf{5416}} & \mc{1}{r|}{0.50} & \mc{1}{r}{5448} & \mc{1}{r}{0.29} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r}{107265} & \mc{1}{r|}{14.53} & \mc{1}{r}{1087716} & \mc{1}{r|}{0.18} & \mc{1}{r}{1087716} & \mc{1}{r|}{0.18} & \mc{1}{r}{\textbf{387}} & \mc{1}{r|}{2.11} & \mc{1}{r}{2804} & \mc{1}{r}{2.04} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r}{26270} & \mc{1}{r|}{9.33} & \mc{1}{r}{684496} & \mc{1}{r|}{0.22} & \mc{1}{r}{684496} & \mc{1}{r|}{0.35} & \mc{1}{r}{\textbf{1995}} & \mc{1}{r|}{3.01} & \mc{1}{r}{9514} & \mc{1}{r}{2.47} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{\textbf{861}} & \mc{1}{r|}{3.13} & \mc{1}{r}{1462} & \mc{1}{r|}{0.01} & \mc{1}{r}{1458} & \mc{1}{r|}{0.00} & \mc{1}{r}{870} & \mc{1}{r|}{0.29} & \mc{1}{r}{870} & \mc{1}{r}{0.65} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r}{\textbf{1103}} & \mc{1}{r|}{0.51} & \mc{1}{r}{2653} & \mc{1}{r|}{0.03} & \mc{1}{r}{2653} & \mc{1}{r|}{0.02} & \mc{1}{r}{1801} & \mc{1}{r|}{2.64} & \mc{1}{r}{1798} & \mc{1}{r}{4.17} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{35442} & \mc{1}{r|}{3.83} & \mc{1}{r}{971421} & \mc{1}{r|}{0.52} & \mc{1}{r}{991000} & \mc{1}{r|}{0.44} & \mc{1}{r}{\textbf{771}} & \mc{1}{r|}{1.51} & \mc{1}{r}{3611} & \mc{1}{r}{1.56} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r}{29419} & \mc{1}{r|}{98.37} & \mc{1}{r}{4266942} & \mc{1}{r|}{7.69} & \mc{1}{r}{4283809} & \mc{1}{r|}{7.78} & \mc{1}{r}{\textbf{11947}} & \mc{1}{r|}{104.27} & \mc{1}{r}{12210} & \mc{1}{r}{145.88} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{6052} & \mc{1}{r|}{1.49} & \mc{1}{r}{299118} & \mc{1}{r|}{0.19} & \mc{1}{r}{299724} & \mc{1}{r|}{0.20} & \mc{1}{r}{2109} & \mc{1}{r|}{0.61} & \mc{1}{r}{\textbf{2061}} & \mc{1}{r}{0.58} \\  

\end{tabu}
\end{ThreePartTable}

==> tables/reduction_subset_table.tex <==
\begin{ThreePartTable}
\begin{tabu}{ccccccccc}

  \mc{1}{l|}{\mr{2}{*}{Graph}} & \mc{2}{c}{extended} & \mc{2}{c}{extended$_{\text{g}}$} & \mc{2}{c}{extended$_{\text{gn}}$} & \mc{2}{c}{extended$_{\text{gnc}}$} \\  

  \mc{1}{l|}{} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r|}{$t$} & \mc{1}{r}{$n$} & \mc{1}{r}{$t$} \\ 
  \hline  

  \mc{1}{l|}{fe\_body} & \mc{1}{r}{1167} & \mc{1}{r|}{0.82} & \mc{1}{r}{1177} & \mc{1}{r|}{0.20} & \mc{1}{r}{1162} & \mc{1}{r|}{\textbf{0.17}} & \mc{1}{r}{1162} & \mc{1}{r}{0.19} \\  

  \mc{1}{l|}{fe\_sphere} & \mc{1}{r}{3540} & \mc{1}{r|}{1.26} & \mc{1}{r}{3662} & \mc{1}{r|}{0.33} & \mc{1}{r}{2961} & \mc{1}{r|}{\textbf{0.31}} & \mc{1}{r}{3510} & \mc{1}{r}{0.30} \\  

  \mc{1}{l|}{buddha} & \mc{1}{r}{103} & \mc{1}{r|}{8.89} & \mc{1}{r}{86} & \mc{1}{r|}{2.12} & \mc{1}{r}{86} & \mc{1}{r|}{\textbf{1.90}} & \mc{1}{r}{86} & \mc{1}{r}{2.07} \\  

  \mc{1}{l|}{ecat} & \mc{1}{r}{251} & \mc{1}{r|}{7.55} & \mc{1}{r}{258} & \mc{1}{r|}{2.66} & \mc{1}{r}{274} & \mc{1}{r|}{\textbf{2.29}} & \mc{1}{r}{253} & \mc{1}{r}{2.92} \\  

  \mc{1}{l|}{georgia-AM3} & \mc{1}{r}{780} & \mc{1}{r|}{3.33} & \mc{1}{r}{796} & \mc{1}{r|}{0.33} & \mc{1}{r}{796} & \mc{1}{r|}{\textbf{0.29}} & \mc{1}{r}{796} & \mc{1}{r}{0.29} \\  

  \mc{1}{l|}{rhode-island-AM2} & \mc{1}{r}{853} & \mc{1}{r|}{2.49} & \mc{1}{r}{845} & \mc{1}{r|}{1.27} & \mc{1}{r}{845} & \mc{1}{r|}{\textbf{1.20}} & \mc{1}{r}{835} & \mc{1}{r}{1.46} \\  

  \mc{1}{l|}{roadNet-PA} & \mc{1}{r}{282} & \mc{1}{r|}{3.16} & \mc{1}{r}{282} & \mc{1}{r|}{1.11} & \mc{1}{r}{300} & \mc{1}{r|}{\textbf{1.07}} & \mc{1}{r}{302} & \mc{1}{r}{1.27} \\  

  \mc{1}{l|}{soc-LiveJournal1} & \mc{1}{r}{4319} & \mc{1}{r|}{153.87} & \mc{1}{r}{4319} & \mc{1}{r|}{\textbf{22.33}} & \mc{1}{r}{4319} & \mc{1}{r|}{22.72} & \mc{1}{r}{4293} & \mc{1}{r}{31.45} \\  

  \mc{1}{l|}{web-NotreDame} & \mc{1}{r}{516} & \mc{1}{r|}{1.38} & \mc{1}{r}{516} & \mc{1}{r|}{0.50} & \mc{1}{r}{516} & \mc{1}{r|}{\textbf{0.35}} & \mc{1}{r}{516} & \mc{1}{r}{0.38} \\  

\end{tabu}
\end{ThreePartTable}
